Algorithmic complexity of $\beta$-expansions and application to A/D conversion

We establish diverse relationships between the algorithmic (Kolmogorov) complexity of the prefixes of any binary expansion and $\beta$-expansions. These relationships allow to develop intuitions on the complexity behavior of $\beta$-expansions, and raise problems related to compressibility of binary sequences generated in the context of A/D conversion relying on $\beta$-expansions. Our last contribution is to solve these problems.

==> subfiles/appendices.tex <==
% !TEX root = ../main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX A %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\texorpdfstring{Definition of $\beta$-expansions by blocks}{}}

% Throughout the paper, we make use of the fact that $\delta_\beta$ is continuous on $\{0,1\}^\omega$, with respect to a specific distance $d$, that we introduce next.
% \begin{definition}\label{def:metric on discrete sequences}
% 	We define
% 	\begin{equation}
% 		\begin{array}{lccl}
% 			d : & \left(\{0,1\}^\omega\right)^2 & \to & \R\\
% 				& \xf,\yf & \mapsto &
% 			\displaystyle\frac{1}{\min \{i \in \N \, : \, \xf_i \neq \yf_i\}}.
% 		\end{array}
% 	\end{equation}
% \end{definition}
% \begin{lemma}
% 	$d$ is a metric.
% \end{lemma}
% \begin{proof}
% 	Let $\xf,\yf \in \{0,1\}^\omega$, and note that $d(\xf,\yf) \geq 0$, $d(\xf,\yf) = d(\yf,\xf)$, and $d(\xf,\yf) = 0 \Leftrightarrow \xf = \yf$. 
% 	Let $\xf,\yf,\zf \in \{0,1\}^\omega$. Then,
% 	\begin{enumerate}[label=(\alph*)]
% 		\item if $d(\xf,\yf) \leq d(\xf,\zf)$, then trivially $d(\xf,\yf) \leq d(\xf,\zf) + d(\zf,\yf)$,
% 		\item if $d(\xf,\yf) > d(\xf,\zf)$, then $d(\yf,\zf) = d(\xf,\yf)$, so $d(\xf,\yf) \leq d(\xf,\zf) + d(\yf,\zf)$.
% 	\end{enumerate}
% 	In all cases, we have $d(\xf,\yf) \leq d(\xf,\zf) + d(\zf,\yf)$. Therefore, $d$ is symmetric, positive separable, and satisfies the triangular inequality on $\N$, so $d$ is a metric.
% \end{proof}
% \begin{lemma}\label{lem:delta beta is continuous}
% 	Let $\beta \in (1,2]$. $\delta_\beta$ as a mapping from $\{0,1\}^\omega$ to $I_\beta$ is continuous.
% \end{lemma}
% \begin{proof}
% 	Fix $\beta \in (1,2]$, $\varepsilon > 0$, and $\xf,\yf \in \{0,1\}^\omega$ such that $d(\xf,\yf) \leq 1/j$, 
%     for some $j \in \N$. Then,
% \begin{align}
% 	\left|\delta_\beta\left(\xf\right) - \delta_\beta\left(\yf\right)\right| &= \left| \sum_{i=1}^\infty (\xf - \yf_i) \beta^{-i}\right|  \leq \sum_{i=j+1}^\infty\left| \xf - \yf_i\right|\beta^{-i} \leq
% 	2 \left| \sum_{i=j+1}^\infty \beta^{-i}\right| \leq \frac{2}{\beta-1}\beta^{-j}.
% \end{align}
% Therefore, a sufficient condition for $\left|\delta_\beta\left(\xf\right) - \delta_\beta\left(\yf\right)\right| \leq \varepsilon$ to hold is
% \begin{equation}
% 	d(\xf,\yf) = \frac{1}{j} \leq \frac{1}{\log_\beta\left( \frac{2}{\varepsilon (\beta-1)}\right)}.
% \end{equation}
% In summary, for all $\xf,\yf \in \{0,1\}^\omega$ satisfying $d(\xf,\yf) \leq \delta := \frac{1}{\log_\beta\left( \frac{2(\lceil \beta \rceil -1)}{\varepsilon (\beta-1)}\right)}$, one has $\left|\delta_\beta(\xf)-\delta_\beta(\yf)\right| \leq \varepsilon$, which establishes the continuity of $\delta_\beta$.
% \end{proof}
The two following results are about computing $\delta_\beta$ when the input is made up of blocks, which turns out to be useful. 
\begin{lemma}\label{lem:factorisation of beta expansion through concatenation}
	Let $n \in \N$, $(\ell_i)_{i \in \ints{0,n}}$, and $(x_i)_{i \in \ints{0,n}} \in \{0,1\}^m$ be a family of $n+1$ binary sequences of respective length $\ell_i$. We define $L_i := \sum_{j=0}^i \ell_j$, for $i \in \ints{0,n}$. Then, for all $\beta \in (1,2]$, it holds that
	\begin{equation}
		\delta_\beta\left(\coprod_{i=0}^n x_i \right) = \delta_\beta(x_0) + \sum_{i=1}^n \beta^{-L_{i-1}} \delta_\beta(x_i).
	\end{equation}
\end{lemma}
\begin{proof} The proof follows by the chain of arguments
	\begin{align}
		\delta_\beta\left(\coprod_{i=0}^n x_i \right) &= \sum_{j=1}^{L_n} \beta^{-j}\left[\coprod_{i=0}^n x_i\right]_j = \sum_{j=1}^{L_0} \beta^{-j}\left[\coprod_{i=0}^n x_i\right]_j + \sum_{j=L_0+1}^{L_n} \beta^{-j}\left[\coprod_{i=0}^n x_i\right]_j\\
		& = \sum_{j=1}^{\ell_0} \beta^{-j}\left[\coprod_{i=0}^n x_0\right]_j + \sum_{j=1}^n \sum_{k=L_{j-1}+1}^{L_j} \beta^{-k}\left[\coprod_{i=0}^n x_i\right]_k\\
		&= \sum_{j=1}^{\ell_0} \beta^{-j}x_0 + \sum_{j=1}^n \sum_{k=1}^{L_j - L_{j-1}} \beta^{-k - L_{j-1}}\left[\coprod_{i=0}^n x_i\right]_{k + L_{j-1}}\\
		&= \delta_\beta(x_0) + \sum_{j=1}^n \beta^{-L_{j-1}}\sum_{k=1}^{\ell_j} \beta^{-k} \left[x_j\right]_k\\
		&= \delta_\beta(x_0) + \sum_{i=1}^n \beta^{-L_{i-1}} \delta_\beta(x_i).
	\end{align}
\end{proof}
\begin{lemma}\label{lem:factorisation of beta expansion through concatenation two}
	Let $x \in \{0,1\}^\ast$ and $\xf \in \{0,1\}^\omega$. Then, for all $\beta \in (1,2]$, it holds that
	\begin{equation}
		\delta_\beta\left( x  \xf \right) = \delta_\beta(x) + \beta^{-|x|} \delta_\beta(\xf).
	\end{equation}
\end{lemma}
\begin{proof}
	The proof follows by the chain of arguments
	\begin{align}
		\delta_\beta\left( x  \xf \right) &=  \sum_{i=1}^\infty [x  \xf]_i\beta^{-i} = \sum_{i=1}^{|x|} [x  \xf]_i\beta^{-i} + \sum_{i=|x| + 1}^{\infty} [x  \xf]_i\beta^{-i}\\
		&= \sum_{i=1}^{|x|} x_i\beta^{-i} + \sum_{i=1}^{\infty} [x  \xf]_{i+|x|}\beta^{-(i+|x|)} =\delta_\beta(x) + \beta^{-|x|} \sum_{i=1}^{\infty} \xf_{i}\beta^{-i}\\
		& =\delta_\beta(x) + \beta^{-|x|} \delta_\beta(\xf).
	\end{align}
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\texorpdfstring{Simple relations for algorithmic complexity of binary and $\beta$-expansions}{Simple relations for algorithmic complexity of binary and -expansions}}
\label{app:greedy binary expansion is a minimizer of Kolmogorov complexity}

\subsection{Proof of Theorem \ref{thm:binary expansion minimizes kolmogorov complexity}}


\begin{lemma}\label{lem:condition prefix beta expansion of x}
	Let $\beta \in (1,2]$, and $s \in \ibet$. Then, for all $x \in \{0,1\}^\ast$, $x$ is a prefix of a $\beta$-expansion if and only if $s \in \delta_\beta(x) +\beta^{-|x|}\left[0,\frac{1}{\beta - 1}\right]$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2]$, and $s \in \ibet$. Suppose $s \in \delta_\beta(x) +\beta^{-|x|}\left[0,\frac{1}{\beta - 1}\right]$. Then, there exists $\xf \in \{0,1\}^\omega$ such that
	\begin{equation}
		s = \delta_\beta(x) +\beta^{-|x|}\delta_\beta(\xf) \overset{\ref{lem:factorisation of beta expansion through concatenation two}}{=} \delta_\beta(x  \xf),
	\end{equation}
	so $x$ is a prefix of the $\beta$-expansion $x  \xf$. Conversely, suppose that $x$ is a prefix of a $\beta$-expansion of $s$. Then, there exists $\xf \in \{0,1\}^\omega$ such that $x  \xf$ is a $\beta$-expansion of $s$, i.e.
	\begin{equation}
		s = \delta_\beta(x  \xf)  \overset{\ref{lem:factorisation of beta expansion through concatenation two}}{=} \delta_\beta(x) +\beta^{-|x|}\delta_\beta(\xf) \in \delta_\beta(x) + \beta^{-|x|}\left[0,\frac{1}{\beta - 1}\right].
	\end{equation}
\end{proof}


\begin{lemma}\label{lem:generalization bounding candidates greedy expansion}
	Let $\beta_1,\beta_2 \in (1,2), \ \beta_1 < \beta_2$, $n \in \N$ and $x \in \{0,1\}^n$. We denote by $A(x)$ the set of $\lceil n \log_2(\beta_1)\rceil$-prefixes of the greedy expansions of all real numbers for which there exists $\beta \in (\beta_1,\beta_2)$ such that one of the $\beta$-expansions has $n$-prefix $x$. Then,
	\begin{equation}
		\#\left(A(x)\right) \leq \frac{2}{\beta_1 - 1} + n(n+1)(\beta_2 - \beta_1)\beta_1^{n} + 2.
	\end{equation}
\end{lemma}
\begin{proof}
	Let $\beta_1,\beta_2 \in (1,2], \ \beta_1 < \beta_2$, $n \in \N$ and $x \in \{0,1\}^n$. Let $X(x) \subseteq \left[0, \frac{1}{\beta_1 - 1}\right)$ be the set of real numbers for which there exists $\beta \in (\beta_1,\beta_2)$ such that one of the $\beta$-expansions has prefix $x$. By Lemma \ref{lem:condition prefix beta expansion of x}, 
	\begin{equation}
		S(x) = \bigcup_{\beta \in [\beta_1,\beta_2]} \left(\delta_\beta(x) + \beta^{-n}\left[0,\frac{1}{\beta - 1}\right]\right).
	\end{equation}
	Note that $t \mapsto \delta_t(b)$, as a function from $(1,2]$ to $\R$, is continuous and decreasing, so $S(x)$ is a closed interval whose lower bound is $\delta_{\beta_2}(x)$ and $\delta_{\beta_1}(x) + \frac{\beta_1^{-n}}{\beta_1-1}$ is the upper bound, i.e.
	\begin{equation}
		S(x) = \left[\delta_{\beta_2}(x),\delta_{\beta_1}(x) + \frac{\beta_1^{-n}}{\beta_1 - 1}\right].
	\end{equation}
	Let $w \in \{0,1\}^{\lceil n \log_2(\beta_2)\rceil}$. One has that $y \in A(x)$ $\Leftrightarrow$ there exists a $s \in S(x)$ such that $y$ is a prefix of $\gf_2(s)$ $\overset{\ref{lem:condition prefix beta expansion of x}}{\Rightarrow}$ there exists $s \in X(x)$ such that $s \in \delta_2(y) + 2^{-|y|}\left[0,1\right]$ $\Leftrightarrow$ there exists $s \in S(x)$ such that $\delta_2(y) \in s + 2^{-|y|}\left[-1, 0\right]$ $\Leftrightarrow$ $\delta_2(y) \in S(x) + 2^{-|y|}\left[-1, 0\right] = \left[\delta_{\beta_2}(x)- 2^{-|y|},\delta_{\beta_1}(x) + \frac{\beta_1^{-n}}{\beta_1 - 1}\right]$. Therefore,
	\begin{equation}
		A(x) \subseteq \delta_2\left(\{0,1\}^{\lceil n \log_2(\beta_1)\rceil}\right) \cap \underset{=: R(x)}{\underbrace{\left[\delta_{\beta_2}(x)- 2^{-|y|},\delta_{\beta_1}(x) + \frac{\beta_1^{-n}}{\beta_1 - 1}\right]}}.
	\end{equation}
	As for any two different elements of $s,s' \in \delta_2\left(\{0,1\}^{\lceil n \log_2(\beta_1)\rceil}\right)$, $|s - s'| \geq d := 2^{-\lceil n \log_2(\beta_1)\rceil}$, one has
	\begin{align}
		\#(A(x)) &\leq \left\lceil \frac{|R(x)|}{d}\right\rceil \leq \frac{\left[\delta_{\beta_2}(x)- 2^{-\lceil n \log_2(\beta_1)\rceil},\delta_{\beta_1}(x) + \frac{\beta_1^{-n}}{\beta_1 - 1}\right]}{2^{-\lceil n \log_2(\beta_1)\rceil}} + 1\\
		&= \frac{2^{-\lceil n \log_2(\beta_1)\rceil} + \frac{\beta_1^{-n}}{\beta_1 - 1} + \delta_{\beta_1}(x) - \delta_{\beta_2}(x)}{2^{-\lceil n \log_2(\beta_1)\rceil}} + 1\\
		& = \frac{2^{-\lceil n \log_2(\beta_1)\rceil}\beta_1^{-n}}{\beta_1 - 1} + 2^{-\lceil n \log_2(\beta_1)\rceil} \left(\delta_{\beta_1}(x) - \delta_{\beta_2}(x)\right) + 2 \\
		&\leq \frac{2^{-n \log_2(\beta_1) + 1}\beta_1^{-n}}{\beta_1 - 1} + 2^{-n \log_2(\beta_1) + 1} \left(\delta_{\beta_1}(x) - \delta_{\beta_2}(x)\right) + 2\\
		 &\leq \frac{2}{\beta_1 -1} + 2\beta_1^n \left(\delta_{\beta_1}(x) - \delta_{\beta_2}(x)\right) + 2\\
		 &\leq \frac{2}{\beta_1 -1} + 2\beta_1^n \frac{n(n+1)}{2} (\beta_2-\beta_1) + 2\\
		 &= \frac{2}{\beta_1 -1} + \beta_1^n n(n+1) (\beta_2-\beta_1) + 2.
	\end{align}
\end{proof}

\begin{theorem}\label{lemma:generalized app beta expansions are more complex than the binary expansion}
	For all $s \in [0,1]$ and all $\beta \in (1,2)$, there exists $c > 0$ such that
\begin{equation}
	K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] \leq K[\xf|n] + F(K[u_n]) + c, \ \ \forall n \in \N, \ \ \forall \xf \in \Sigma_\beta(s),
\end{equation}
where $u_n := \gf_2(\beta-1)_{1: n}$, and $F: t \mapsto t + 2\log_2(t)$.
\end{theorem}
\begin{proof}
The main arguments of this proof follow closely that of \cite[Theorem 3]{staiger2002kolmogorov}. Let $s \in [0,1]$, $\beta \in (1,2)$, $\xf \in \Sigma_\beta(s)$ and $n \in \N$, large enough to ensure that $u_n := \gf_2(\beta - 1)_{1: n}$ is not made only of $0$'s. Let $\beta_1 - 1 \in (0,1)\cap \Q$ to be the real number having the same greedy binary expansion as $\beta - 1$, but truncated after $\lceil n \log_2(\beta)\rceil$ bits, i.e. $\beta_1 - 1 := \delta_2(u_n)$.
We also define $\beta_2 := \beta_1 + 2^{-\lceil \log_2(\beta)\rceil}$. By Lemma \ref{lem:condition prefix beta expansion of x}, 
\begin{equation}
	1 \overset{(a)}{<} \beta_1 \leq \beta \leq \beta_2 \leq 2.
\end{equation}
where (a) follows from the fact that $u_n$ is not made only of $0$'s.

By Lemma \ref{lem:generalization bounding candidates greedy expansion}, the sole knowledge of $\xf_{1: n}$ allows to immediatly conclude that $\gf_2(s)_{1: \lceil n \log_2(\beta) \rceil}$ belongs to a set $A(\xf_{1: n}) \subseteq \{0,1\}^{\lceil n \log_2(\beta_1) \rceil}$, which cardinality is bounded above by $\frac{2}{\beta_1 - 1} + n(n+1)(\beta_2 - \beta_1)\beta_1^{n} + 2$, and which can be computed by using $u_n$ only. As defined above, $\beta_2 - \beta_1 = 2^{-\lceil \log_2(\beta)\rceil} \leq \beta^{-n}$, hence $n(n+1)(\beta_2 - \beta_1)\beta_1^n \leq n(n+1) (\beta_1/\beta)^n$. As $\beta_1/\beta < 1$, $\left(n(n+1) (\beta_1/\beta)^n\right)_{n \in \N}$ is a bounded sequence. Overall, there exists a constant $N > 0$, independant of $n$, such that $\#(A(\xf_{1: n})) \leq N$.

Let $z_n \in \N$ be the index of $\gf_2(s)_{1: \lceil n \log_2(\beta) \rceil}$ in the lexicographical enumeration of $A(\xf_{1: n})$. Then, one can build an effective algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$, such that on input $\langle \langle\xf_{1: n}, u_n \rangle,  z_n \rangle$, $\varphi$ computes $A(\xf_{1: n})$, finds the $z_n$-th element $y$ of $A(\xf_{1: n})$ and outputs $y$.
 By the preceding discussion, it is clear that $\varphi(\langle \langle \xf_{1: n},  u_n\rangle,  z_n  \rangle) = \gf_2(s)_{1: \lceil n \log_2(\beta) \rceil}$. By Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists $C,C' > 0$ such that 
 \begin{align}\label{eq:first bounding of kolmogorov complexity of greedy binary expansion}
	K[y] &\overset{\ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}}{\leq} K[\langle \langle\xf_{1: n}, z_n \rangle,  u_n \rangle ] + C\\
	&\overset{(\ref{eq:simple inequality on concatenation of sequences})}{\leq} K[\langle \xf_{1: n}, z_n \rangle] + F\left(K[u_n]\right) + C_+ + C\\
	&\overset{(\ref{eq:simple inequality on concatenation of sequences})}{\leq} K[\xf_{1: n}] + F\left(K[z_n]\right) + F\left(K[u_n]\right) + 2C_+ + C\\
	&\overset{(\ref{eq:algorithmic complexity is bounded by the length})}{\leq} K[\xf_{1: n}] + F\left(|z_n|+ C_{||}\right) + F\left(K[u_n]\right) + 2C_+ + C\\
	&\overset{\ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}}{\leq} K[\xf_{1: n}] + F\left(|z_n|+ C_{||}\right) + F\left(K[u_n] + C'\right)  + 2C_+ + C\\
	&\overset{(a)}{\leq} K[\xf_{1: n}] + F\left(|z_n|\right) + F\left(K[u_n]\right) + C_{||} + 2C_+ + C + C',\label{eq:ineq algorithmic complexity w appendix}
 \end{align}
 where $(a)$ is by $F$ being subadditive.
 Recall from above that $\#(A(\xf_{1:n})) \leq N$. As $z_n$ is an index for $A(\xf_{1:n})$, then $z_n \leq N$, and we set $C_0 :=  F(N)$, so that 
 \begin{equation}
 K[y] \overset{(\ref{eq:ineq algorithmic complexity w appendix})}{\leq} K[\xf_{1: n}] + F\left(K[u_n]\right) + C_{||} + 2C_+ + C + C' + C_0.
 \end{equation}
We set $c := C_{||} + 2C_+ + C + C' + C_0$. By identification of $y$ with $\gf_2(s)_{1: \lceil n \log_2(\beta_1) \rceil}$, one has 
 \begin{equation}\label{eq:almost the end of the proof}
		K[\gf_2(s)|\lceil n \log_2(\beta_1) \rceil] \leq K[\xf|n] + F(K[u_n]) + c.
 \end{equation}
 Note that as $\beta_1 := \delta_2(u_n)$, $|\beta - \beta_1| \leq 2^{-\lceil n \log_2(\beta)\rceil} \leq \beta^{-n}$, so
 \begin{align}
	\left|\lceil n \log_2(\beta) \rceil - \lceil n \log_2(\beta_1) \rceil\right| & \leq n (\log_2(\beta) - \log_2(\beta_1)) + 2\\
	& = n (\log_2(\beta_1 + \beta^{-n}) - \log_2(\beta_1)) + 2\\
	& = n (\log_2(1 + \beta_1^{-1}\beta^{-n})) + 2 \\
	&\leq n \beta_1^{-1}\beta^{-n} + 2\\
	&\overset{(a)}{\leq} \frac{\beta_1^{-1}}{\log(\beta)}\beta^{-\frac{1}{\log(\beta)}} + 2 =: D,
 \end{align}
 where is a consequence of a study of the maximum of the functiono $t \mapsto t\beta^{-t}$. By application of Lemma \ref{lem:kolmogorov complexity of closed sequences}, there exists $D' > 0$ such that
 \begin{equation}\label{eq:comparable kolmogorov complexities for approximations}
	K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] \leq K[\gf_2(s)|\lceil n \log_2(\beta_1) \rceil] + D'.
 \end{equation}
By (\ref{eq:almost the end of the proof}) and (\ref{eq:comparable kolmogorov complexities for approximations}), one gets
\begin{equation}
	K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] \leq K[\xf|n] + F(K[u_n]) + c + D',
\end{equation}
thereby finishing the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:upper bound kolmogorov complexity beta expansions}}

\textit{To appear.}

\section{Miscellaneous results}

% \begin{lemma} \label{lem:log x delta is decreasing}
% 	Let $\beta \in (1,2)$, and $\delta \in \left(0, \frac{2 - \beta}{\beta}\right)$. Then, 
% 	\begin{equation}
% 		\begin{array}{lrcl}
% 			g : & (1,\beta] & \to & \R\\
% 			& t & \mapsto & -\log_t\left( \frac{\delta}{2-t}\right)
% 		\end{array}
% 	\end{equation}
% 	is decreasing.
% \end{lemma}
% \begin{proof}
% 	Let $t \in (1,\beta]$. Then,
% 	\begin{align}
% 		g'(t) &= \frac{\log(\delta)}{t\log(t)^2} - \frac{\frac{1}{2-t} \log(t) - \frac{1}{t}\log(2-t)}{\log(t)^2}\\
% 		&= \frac{1}{\log(t)^2} \left( \frac{-1}{2-t} + \frac{1}{t}(\log(\delta) - \log(2-t))\right). \label{eq:expression of g prime x}
% 	\end{align}
% 	As $\delta \leq \frac{2 -\beta}{\beta} < 2 -\beta \leq 2 - t$, one has $\log(\delta) - \log(2-t) < 0$. From (\ref{eq:expression of g prime x}), it follows that
% 	\begin{equation}
% 		g'(t) < 0,
% 	\end{equation}
% 	thereby finishing the proof.
% \end{proof}

% \begin{lemma}\label{lem:delta beta lipschitz}
% 	For $\beta \in (1,2]$ $\delta_\beta$ be defined according to (\ref{eq:definition of delta beta}). Let $x \in \{0,1\}^\ast$. Then, 
% 	\begin{equation}
% 		\begin{array}{lrcl}
% 			h : & (1,2] & \to & \R\\
% 			& \beta & \mapsto & \delta_\beta(x)
% 		\end{array}
% 	\end{equation}
% 	is $\frac{|x|(|x|+1)}{2}$-Lipschitz.
% \end{lemma}
% \begin{proof}
% 	Let $\beta_1, \beta_2 \in (1,2)$, and $x \in \{0,1\}^\ast$. Without loss of generality, we assume that $\beta_1 < \beta_2$. 
% 	\begin{align}
% 		|\delta_{\beta_1}(x) - \delta_{\beta_2}(x)| = \left|\sum_{i=1}^{|x|} x_i \beta_1^{-i} - \sum_{i=1}^{|x|} x_i \beta_2^{-i}\right| = \left|\sum_{i=1}^{|x|} x_i \left(\beta_1^{-i} -  \beta_2^{-i}\right)\right|
% 		\overset{(a)}{\leq} \sum_{i=1}^{|x|}  \left|\beta_1^{-i} - \beta_2^{-i}\right|, \label{eq:weak eq bounding delta beta variations}
% 	\end{align}
% 	where (a) is by $x_i \leq 1$.
% 	Note that for all $\beta \in (1,2)$, $\left|\frac{\partial \beta^{-i}}{\partial \beta}\right| =\left| -i \beta^{-(i+1)}\right| \leq i$. Then, by using the mean value theorem, one gets $\left|\beta_1^{-i} - \beta_2^{-i}\right| \leq i |\beta_1 - \beta_2|$. By (\ref{eq:weak eq bounding delta beta variations}),
% 	\begin{equation}
% 		|\delta_{\beta_1}(x) - \delta_{\beta_2}(x)| \leq \sum_{i=1}^{|x|} i |\beta_1 - \beta_2| = \frac{|x|(|x|+1)}{2} |\beta_1 - \beta_2|,
% 	\end{equation}
% 	thereby finishing the proof.
% \end{proof}
% \begin{lemma}\label{eq:condition on n 0 for xi i to be lower bounded}
%     Let $\beta \in (1,2)$, $C \in (0,1)$, $L,N \in \N$, $q_i := 1 + \delta_2(\gf_2(\beta-1)_{1: L + Ni})$, and $\xi_i := \frac{1}{q_i^{i+1}} \prod_{j=0}^{i} q_j$, for all $i \in \N_0$. If 
%     \begin{equation}\label{eq:condition on n_0 general}
%         L \geq \frac{1}{2}\log_2(-\log(C)),
%     \end{equation} then 
%     \begin{equation}
%         \xi_i \geq C, \ \text{for all} \ i \in \N_0.
%     \end{equation}
% \end{lemma}
% \begin{proof}
    
% Let $\beta \in (1,2)$, $L,N \in \N$, $q_i := 1 + \delta_2(\gf_2(\beta-1)_{1: L + Ni})$, and $\xi_i := \frac{1}{q_i^i} \prod_{j=0}^{i-1} q_j$, for all $i \in \N_0$. Note that
% \begin{equation}
%    \log( \xi_i) = \log\left(\frac{1}{q_i^{i+1}}\prod_{j=0}^{i} q_j\right) = \sum_{j=0}^{i} \log\left( \frac{q_j}{q_i}\right). 
% \end{equation}
% We will show that if $n_0$ satisfies (\ref{eq:condition on n_0 general}), then $\log(\xi_i) \geq \log(C)$ for all $i \in \N$. A numerical approximation allows to show that 
% \begin{equation}\label{eq:minoration de log 1 + x}
%     \log(1 + t) \geq 2t, \ \text{for all} \ t \in [-0.75, 0].
% \end{equation}
% Now, let $\xf := \gf_2(\beta-1)_{L+1:\infty}$. Note that by Lemma \ref{lem:factorisation of beta expansion through concatenation}, 
% \begin{align}
%     q_j &= 1 + \delta_2(\gf_2(\beta-1)_{1: L + Nj} = 1 + \delta_2(\gf_2(\beta-1)_{1: L}) + 2^{-L} \delta_2(\xf_{1: Nj})\\
%     &= q_0 + 2^{-L} \delta_2(\xf_{1: Nj}),
% \end{align}
% for all $j \in \N$. Fix  $i \in \N$.
% \begin{align}
%     \log(\xi_i) &= \sum_{j=0}^{i} \log\left( \frac{q_j}{q_i}\right) = \sum_{j=0}^{i} \log\left( \frac{q_0 + 2^{-L} \delta_2(\xf_{1: Nj})}{q_0 + 2^{-L} \delta_2(\xf_{1: Ni})}\right)\\
%     &=\sum_{j=0}^{i} \log\left( \frac{1 + \frac{1}{2^{L}q_0} \delta_2(\xf_{1: Nj})}{1 + \frac{1}{2^{L}q_0} \delta_2(\xf_{1: Ni})}\right) \\
%     &=\sum_{j=0}^{i} \log\left( \frac{1 + \frac{1}{2^{L}q_0} (\delta_2(\xf_{1: Nj})- \delta_2(\xf_{1: Ni}) + \delta_2(\xf_{1: Ni}))}{1 + \frac{1}{2^{L}q_0} \delta_2(\xf_{1: Ni})}\right)\\
%     &=\sum_{j=0}^{i} \log\left(1 +  \frac{\delta_2(\xf_{1: j}) - \delta_2(\xf_{1: Ni})}{2^{L}q_0 \left( 1 + \frac{1}{2^{L}q_0} \delta_2(\xf_{1: Ni})\right)}\right)\\
%     &=\sum_{j=0}^{i} \log\left(1 +  \frac{\delta_2(\xf_{1: Nj}) - \delta_2(\xf_{1: Ni})}{2^{L}q_0 +  \delta_2(\xf_{1: Ni})}\right). \label{eq:other form xi i}
% \end{align}
% Note that, for all $i,j \in \N$, $j \leq i$ implies that
% \begin{equation}
%     0 \geq \frac{\delta_2(\xf_{1: Nj}) - \delta_2(\xf_{1: i})}{2^{L}q_0 +  \delta_2(\xf_{1: Ni})} \geq \frac{-2^{-L-Nj}}{2^{L}q_0 + \delta_2(\xf_{1: Ni})} \overset{(a)}{\geq} -\frac{2^{-L-Nj}}{2^{L}q_0} \overset{(b)}{\geq} - \frac{1}{2^{2L}} \overset{(c)}{\geq} - 0.75, \label{eq:simplification of the xi i terms}
% \end{equation}
% where (a) is by $\delta_2(\xf_{1: Ni}) \geq 0$, (b) follows from $q_0 \geq 1$ and $2^{-Nj} \leq 1$, and (c) is a consequence of $L \geq 1$. Therefore,
% \begin{align}
%     \log(\xi_i) &\overset{(\ref{eq:other form xi i})}{=} \sum_{j=0}^{i} \log\left(1 +  \frac{\delta_2(\xf_{1: Nj}) - \delta_2(\xf_{1: Ni})}{2^{L}q_0 +  \delta_2(\xf_{1: Li})}\right) \overset{(\ref{eq:minoration de log 1 + x})}{\geq} 2 \sum_{j=0}^{i} \frac{\delta_2(\xf_{1: Nj}) - \delta_2(\xf_{1: Ni})}{2^{L}q_0 +  \delta_2(\xf_{1: Ni})} \overset{(\ref{eq:simplification of the xi i terms})}{\geq} -2^{-2L}. \nonumber
% \end{align}
% It immediately follows that $L \geq \frac{1}{2}\log_2(-\log(C))$ implies $\xi_i \geq C$.
% \end{proof}

\begin{lemma}
	\cite[Example 2.1.5]{li2008introduction} There exists $C_+>0$, such that
	\begin{align}\label{eq:simple inequality on concatenation of sequences}
		K[ x x'] &\leq K[x] + F(K[x']) + C_+, \ \ \text{for all} \ x,x' \in \{0,1\}^\ast,
	\end{align}
	and
	\begin{align}\label{eq:simple inequality on pairing of sequences}
		K[ \langle x, x'\rangle] &\leq K[x] + F(K[x']) + C_+, \ \ \text{for all} \ x,x' \in \{0,1\}^\ast,
	\end{align}
	where $F:t\mapsto t + 2\log_2(t)$.
\end{lemma}
\begin{lemma}\cite[Theorem 2.1.2]{li2008introduction} There exists $C_{||} > 0$, such that 
	\begin{equation}\label{eq:algorithmic complexity is bounded by the length}
		K[x] \leq |x| + C_{||}, \ \ \text{for all} \ x \in \{0,1\}^\ast.
	\end{equation}
\end{lemma}
\begin{lemma}
	Let $N \in \N$, $\xf \in \{0,1\}^\omega$, $(u_n)_{n \in \N}$ a sequence of integers. Then, 
	\begin{equation}
		K[\xf|N n] \leq u_n, \ \forall n \in \N \Rightarrow \exists C > 0 \ s.t. \ K[\xf|n] \leq u_{\lfloor n/N \rfloor } + C, \ \forall n \in \N.
	\end{equation}
\end{lemma}
\begin{proof}
	Let $N \in \N$, $\xf \in \{0,1\}^\omega$, $(u_n)_{n \in \N}$ a sequence of integers, and suppose that $K[\xf|N n] \leq u_n, \ \forall n \in \N$. Fix $n \in \N$. Then, $k := \lfloor n/N \rfloor$ satisfies $n = kN + (n - kN)$, where $n - kN \leq N$. Then,
	\begin{align}
		K[\xf|n] &= K[\xf_{1: n}] = K[\xf_{1: kN}  \xf_{1: (n- kN)}] \\
		&\overset{(\ref{eq:simple inequality on concatenation of sequences})}{\leq} K[\xf_{1: kN}] + K[\xf_{1: (n- kN)}] + 2 \log_2 (K[\xf_{1: (n- kN)}]) + C_+\\
		&\overset{(a)}{\leq} K[\xf_{1: kN}] + N + C_{||} + 2 \log_2 (N + C_{||}) + C_{+}\\
		&\overset{(b)}{\leq} u_k + N + C_{||} + 2 \log_2 (N + C_{||}) + C_{+}\\
		&= u_{\lfloor n/N \rfloor} + N + C_{||} + 2 \log_2 (N + C_{||}) + C_{+},
	\end{align}
	where (a) follows from (\ref{eq:algorithmic complexity is bounded by the length}) and $n - kN \leq N$, and (b) is by $K[\xf|N k] \leq u_k$. We set $C:= N + C_{||} + 2 \log_2 (N + C_{||}) + C_{+}$, thereby finishing the proof.
\end{proof}
\begin{lemma}\label{lem:kolmogorov complexity of closed sequences}
	Let $\xf \in \{0,1\}^\omega$, $(i_n)_{n \in \N}$ and $(j_n)$ be two increasing sequences of natural numbers. Suppose that there exists $M > 0$ such that $|i_n-j_n| \leq M$, for all $n \in \N$. Then, there exists $C>0$, such that
	\begin{equation}
		K[\xf|i_n] \leq K[\xf|j_n] + C, \ \text{for all} \ n \in \N.
	\end{equation}
\end{lemma}
\begin{proof}
	Let $\xf \in \{0,1\}^\omega$, $(i_n)_{n \in \N}$ and $(j_n)$ be two increasing sequences of natural numbers. Suppose that there exists $M > 0$ such that $ |i_n-j_n| \leq M$, for all $n \in \N$. Fix $n \in \N$, and let $x:= 10^{j_n + M-i_n}$. Then, one can build an effective algorithm $\phi: \{0,1\}^\ast \to \{0,1\}^\ast$, which on input $\xf_{1: j_n + M}  x$, which uses $x$ to delete the $j_n + M - i_n$ last bits of $\xf_{1: j_n + M}$, and outputs the resulting sequence. Then, $\phi(\xf_{1: j_n + M}  x) = \phi(\xf_{1: i_n})$. By Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists $c_\phi > 0$ such that
	\begin{align}
		K[\xf|i_n] &= K[\xf_{1: i_n}] \leq K[\xf_{1: j_n}  x] + c_\phi\\
		&\overset{(\ref{eq:simple inequality on concatenation of sequences})}{\leq} K[\xf_{1: j_n}] + K[x] + 2\log(K[x]) +c_{\phi} + C_{+}\\
		&\overset{(\ref{eq:algorithmic complexity is bounded by the length})}{\leq} K[\xf_{1: j_n}] + |x| + C_{||} + 2 \log_2 (|x| + C_{||}) + c_\phi + C_{+}\\
		&\overset{(a)}{\leq} K[\xf_{1: j_n}] + 2M + C_{||} + 2 \log_2 (2M + C_{||}) + c_\phi + C_{+},
	\end{align}
	where (a) is by $|x| = j_n + M - i_n$ and $i_n - M \leq j_n$. We set $C:= 2M + C_{||} + 2 \log_2 (2M + C_{||}) + c_\phi+ C_{+}$, thereby finishing the proof.
\end{proof}


==> subfiles/expected_complexity_beta_expansions.tex <==
% !TEX root = main.tex

\section{\texorpdfstring{Expected Kolmogorov complexity of $\beta$-expansions generated by the Daubechies algorithm}{}}

ENLEVER CETTE SECTION POUR HELMUT, ET FAIRE LA SECTION SUR L'ALGORITHME. POINT.

Bon ALORS: on se rassure.

Let $(\Omega,\AM, \mu)$ be a probability space. 
\begin{definition}
    A $\mu$-test is a measurable function $f : \Omega \to \R$ such that 
    \begin{equation}
        \mu\left\{ \omega \in \Omega : f(\omega) > k \right\} \leq 2^{-k}.
    \end{equation}
\end{definition}
\begin{definition}
    A unit $\mu$-integrable function is a measurable function $f : \Omega \to \R$ such that 
    \begin{equation}
        \int_\Omega f d\mu \leq 1.
    \end{equation}
\end{definition}
\begin{theorem}
    Let $f$ be unit $\mu$-integrable. Then, $\log f$ is a $\mu$-test.
\end{theorem}
\begin{proof}
    Let $f$ be unit $\mu$-integrable. Define, for $k \in \N$,
    \begin{equation}
        A_k := \left\{ \omega \in \Omega :\log f(\omega) > k \right\}.
    \end{equation}
    Suppose that $\log f$ is not a $\mu$-test, i.e., that there exists $k \in \N$ such that $\mu(A_k) > 2^{-k}$. Then,
    \begin{align}
        \int_\Omega f d\mu \geq \int_{A_k} fd\mu > 2^k \mu(A_k) > 1,
    \end{align}
    which is a contradiction.
\end{proof}
\noindent From now on $\Omega = \{0,1\}^\N$. Let $F : x \mapsto x + \log_2(x)$.
\begin{definition}
    Let $A \in \Omega$ and $f_{0|A} : \Omega \to \R$ be defined by 
    \begin{equation}
        f_{0|A}(\omega) := \sup_{n \in \N} \left\{ \log \frac{1}{\mu(\omega_{1:n}\Omega)} - F\circ C[\omega_{1:n}|A] \right\},
    \end{equation}
    for all $\omega \in \Omega$.
\end{definition}
\begin{theorem}
    For all $A \in \Omega$, $f_{0|A}$ is a $\mu$-test.
\end{theorem}
\begin{proof}
    We prove that $2^{f_{0|A}}$ is unit $\mu$-integrable. First, define 
    \begin{equation}
        h_n(\omega) =  \log \frac{1}{\mu(\omega_{1:n}\Omega)} - F \circ C [\omega_{1:n}|A].
    \end{equation}
    Then,
    \begin{align}
        \sum_{n\in \N} \int_\Omega 2^{h_n} d\mu & = \sum_{n \in \N} \int_{\omega \in \Omega} \frac{1}{\mu(\omega_{1:n}\Omega)} 2^{- F \circ C [\omega_{1:n}|A]} d\mu(\omega)\\
        & = \sum_{n \in \N} \sum_{x \in \{0,1\}^n} \frac{1}{\mu(x\Omega)} 2^{- F \circ C [x|A]} \mu(x \Omega)\\
        & = \sum_{n \in \N} \sum_{x \in \{0,1\}^n} 2^{- F \circ C [x|A]} = \sum_{x \in \{0,1\}^\ast} 2^{- F \circ C [x|A]}.
    \end{align}
    For each $x \in \{0,1\}^\ast$, define $x_A \in \{0,1\}^\ast$ to be the canonical string associated to $x$ relatively to $A$, i.e. the lexicographically maximal string satisfying $|x_A| = C(x|A)$. Note that the set $\{ \bar x_A : x \in \{0,1\}^\ast\}$ is prefix-free, and hence by Kraft inequality,
    \begin{equation}
        \sum_{x \in \{0,1\}^\ast} 2^{-\len{\bar x_A}} \leq 1.
    \end{equation}
    Since $\len{\bar x_A} = F \circ C[x|A]$ we get 
    \begin{equation}
        \sum_{n\in \N} \int_\Omega 2^{h_n} = \sum_{x \in \{0,1\}^\ast} 2^{- F \circ C [x|A]} = \sum_{x \in \{0,1\}^\ast} 2^{-\len{\bar x_A}} \leq 1.
    \end{equation}
    We conclude by noting that 
    \begin{align}
        \int_\Omega 2^{f_{0|A}} d\mu = \int_\Omega  2^{\sup_{n\in \N} h_n} d\mu \overset{(a)}{=}  \int_\Omega \sup_{n\in \N} 2^{h_n} d\mu
        \leq \int_\Omega \sum_{n\in \N} 2^{h_n} d\mu
        \overset{(b)}{=} \sum_{n\in \N} \int_\Omega 2^{h_n} d\mu
        \leq 1,
    \end{align}
    where (a) is follows from the fact that $x \mapsto 2^x$ is continuous, and (a) is by the Lebesgue sum-integral inversion theorem.
\end{proof}


In this section, we study the expected Kolmogorov complexity of the $\beta$-expansions generated by Algorithm DAUBECHIES. Recall that on input $s \in I_\beta$, the physical device $T$ satisfies the following input-output relationship
\begin{equation}
    T(s) = \begin{cases}
        0, \ \text{if} \ s \in [0, t - \varepsilon) =: E_T^{(0)},\\
        \text{Randomly} \ 0 \ \text{or} \ 1, \ \text{if} \ s \in [t - \varepsilon, t + \varepsilon] =: S_T,\\
        1, \ \text{if} \ s \in (t + \varepsilon, 1/(\beta-1)] =: E_T^{(1)}.
    \end{cases}
\end{equation}
Note that the sequence $(r_i)_{i \in \{0, \ldots, n\}}$ defined in lines LINES of Algorithm DAUBECHIES is defined by the following recursive relationship
\begin{align}
    r_0 &= s,\\
    r_{i+1} &= \beta r_i - T(r_i) =: K_{\beta,T}(r_i), \ \forall i \in \{0,\ldots, n-1\}.
\end{align}
Therefore, the output of Algorithm DAUBECHIES $\mathcal A_\beta(s,n,T)$ on input $s \in [0,1]$ and $n \in \N$, is expressed as
\begin{equation}
    \mathcal A_\beta(s,n,T) = \coprod_{i=0}^{n-1} T\left(K_{\beta,T}^i(s)\right).
\end{equation}
In order to formalize better the problem, we can define $T(s)$ formally as a random variable on $\{0,1\}$, i.e., as a function $T(s) : \{0,1\} \to \{0,1\}$ satisfying
\begin{equation}
    T(s)(x) := \begin{cases}
        0, \ \text{if} \ s \in  E_T^{(0)},\\
        x, \ \text{if} \ s \in  S_T,\\
        1, \ \text{if} \ s \in  E_T^{(1)},
    \end{cases}
    \ \forall x \in \{0,1\}.
\end{equation}
Since the generation of the sequence $(r_i)_{i \in \N}$ might rely on an arbitrarily large number of Bernoulli experiments, we define an extension $\tilde T(s)$ of $T(s)$, that will be useful to consider Algorithm DAUBECHIES as a random variable. Namely, we define $\tilde T(s) : \{0,1\}^\N \to \{0,1\}$ by 
\begin{equation}
    \tilde T(s)(\xf) := \begin{cases}
        0, \ \text{if} \ s \in  E_T^{(0)},\\
        \xf_1, \ \text{if} \ s \in  S_T,\\
        1, \ \text{if} \ s \in  E_T^{(1)},
    \end{cases}
    \ \forall \xf \in \{0,1\}^\N.
\end{equation}
Thanks to the formulation above, we can see Algorithm DAUBECHIES as first generating an infinite sequence $\xf \in \{0,1\}^\N$ out of infinitely many Bernoulli experiments, and then reading successively the outcomes of this experiment, i.e., at each time step, the algorithm reads $\xf_1$, and then discards it, such that the sequence $\xf$ is transformed into the sequence $\yf := \xf_2\xf_3\ldots$. This is usually denoted by $\yf = \sigma(\xf)$, where $\sigma : \{0,1\}^\N \to \{0,1\}^\N$ is called the left-shift. Then, in the next time step, the algorithm will read $\yf_1 = \xf_2$ to generate the next bit of the $\beta$-expansion of $s$.  Note that when $s \notin S$, then the generated bit does not depend on the Bernoulli experiments, as it is generated deterministically. Hence, the Algorithm DAUBECHIES does not need to discard $\xf_1$, and wait until the next time step for which $s \in S$ to discard it. Accordingly, at each time step, the function $\sigma_s : \{0,1\}^\N \to \{0,1\}^\N$ defined by 
\begin{equation}
    \sigma_s(\xf) := \begin{cases}
        \xf \ \text{if} \ s \notin S,\\
        \sigma(\xf), \ \text{if} \ s \in S,
    \end{cases} \ \forall s \in I_\beta, \ \xf \in \{0,1\}^\N,
\end{equation}
is applied to the infinite sequence $\xf$ of Bernoulli experiments. We are now ready to state formally the definition of the Algorithm DAUBECHIS as a random variable. First, we model $K_{\beta,T}(s)$ as a random variable on $\{0,1\}^\N$, i.e., as a function $K_{\beta,T}(s) : \{0,1\}^\N \to I_\beta \times \{0,1\}^\N$.  defined by 
\begin{equation}
    K_{\beta,T}(s)(\xf) := (\beta s - \tilde T(s)(\xf_1), \sigma_s(\xf)),
    \ \forall \xf \in \{0,1\}^\N.
\end{equation}
In order to simplify the notations, we might consider $\tilde T$ as a function from $I_\beta \times \{0,1\}^\N$ into $\{0,1\}$ and $K_{\beta,T}$ as a function from $I_\beta \times \{0,1\}^\N$ into itself, by making the confusion between $T(s)(\xf)$ and $T(s,\xf)$, and the confusion between $K_{\beta,T}(s)(\xf)$ and $K_{\beta,T}(s,\xf)$. This simpler formalism allows to define the output of the Algorithm DAUBECHIES as a random variable as well, i.e., as a function $\mathcal A_\beta(s,n,T) : \{0,1\}^\N \to \{0,1\}^n$, by 
\begin{equation}
    \mathcal A_\beta(s,n,T)(\xf) = \coprod_{i=0}^{n-1} \tilde T\left(K_{\beta,T}^i(s,\xf)\right), \ \forall \xf \in \{0,1\}^\N.
\end{equation}
We repeat that Algorithm DAUBECHIES can generate different outputs of the same input $s \in [0,1]$. Namely, for $s \in [0,1]$ and $n \in \N$, we denote by $\Sigma_\beta(s,n,T) \subseteq \{0,1\}^n$ the set of possible outputs of Algorithm DAUBECHIES on input $(s,n)$. Note that 
\begin{equation}
    \Sigma_\beta(s,n,T) = \left\{ \mathcal A_\beta(s,n,T)(\xf) : \xf \in \{0,1\}^\N\right\} = \mathcal A_\beta(s,n,T)\left( \{0,1\}^\N\right).
\end{equation} 
We let also $\NN_\beta(s,n,T) :=  \# \left(\Sigma_\beta(s,n,T) \right)$. For the specific case of $T$ satisfying $E_T^{(0)} = [0, \beta^{-1})$ and $S_T = [\beta^{-1}, (\beta(\beta-1))^{-1}]$, $\NN_\beta(s,n,T)$ is a well-studied quantity usually called the \textit{growth rate for $\beta$-expansions}, as it counts how many $\beta$-expansions the number $s$ has. We now leverage the formalism introduced above to establish lower bounds on the expected Kolmogorov complexity of the $\beta$-expansions it generates. Recall that for a fixed number $\beta \in (1,2)$, we have defined the equivalence relationship $\sim_\beta$ over $\{0,1\}^\ast$ by 
\begin{equation}
    x \sim_\beta y \iff n := |x| = |y| \ \text{and} \ \sum_{i=1}^n x_i \beta^{-i} = \sum_{i=1}^n y_i \beta^{-i}, \ \forall x,y \in \{0,1\}^\ast.
\end{equation}
Moreover, we have defined the equivalence class $[x]_\beta := \{y \in \{0,1\}^\ast : x \sim_\beta y\}$, for all $x \in \{0,1\}^\ast$, which, seen as a multivalued function $[\cdot]_\beta : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$, is proven to be computable in the proof of Corollary \ref{cor:M is computable for algebraic beta}.We define 
\begin{equation}
    \tilde\NN_\beta(s,n,T) := \# \left(\Sigma_\beta(s,n,T) / \sim_\beta\right).
\end{equation}
Note that if $\beta$ is not algebraic, then $[x]_\beta = \{x\}$ for every $x \in \{0,1\}^n$, hence $\tilde\NN_\beta(s,n,T) = \NN_\beta(s,n,T)$. We now construct a multivalued function $f_{\beta, 1 \to all} : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ that are computable relatively to $\beta$, such that
\begin{equation}
    \langle \Sigma_\beta(s,n,T) \rangle \in f_{\beta, 1 \to all}\left(x\right). 
\end{equation}
To build $f_{\beta, 1 \to all}$, we first follow the same intuitions that lead to the construction of $f_{\beta \to 2}$ and $f_{2 \to \beta}$ in the PREVIOUS SECTIONS. Namely, the knowledge of $x \in \Sigma_\beta(s,n,T)$ allows to infer that
\begin{equation}
    s \in I(x) := \left[\sum_{i=1}^{n} x_i \beta^{-i},  \sum_{i=1}^{n} x_i \beta^{-i}+ \frac{\beta^{-n}}{\beta-1} \right],
\end{equation}
and further deduce that 
\begin{equation}
    \sum_{i=1}^n y_i \beta^{-i} \in J(x) := \left[\sum_{i=1}^{n} x_i \beta^{-i} - \frac{\beta^{-n}}{\beta-1},  \sum_{i=1}^{n} x_i \beta^{-i}+ \frac{\beta^{-n}}{\beta-1} \right],
\end{equation}
for all $y \in \Sigma_\beta(s,n,T)$. Hence, by defining $g_\beta : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ as 
\begin{equation}
    g_\beta(x) := \left\{ y \in \{0,1\}^n : n = |x|,  \sum_{i=1}^n y_i \beta^{-i} \in J(x)\right\},
\end{equation}
for all $x \in \{0,1\}^\ast$, we get 
\begin{equation}
    \Sigma_\beta(s,n,T) \subseteq g_\beta(x), \ \forall x \in \Sigma_\beta(s,n,T).
\end{equation}
Now, for $x \in \{0,1\}^\ast$, define $\tilde g_\beta(x) := g_\beta(x)/ \sim_\beta$, and $\tilde \NN_g(x) := \# \tilde g_\beta(x)$. Note that the function defined by
\begin{equation}
    \begin{array}{rccc}
        \varphi_\beta : & \{0,1\}^n / \sim_\beta & \to & I_\beta\\
        & [x]_\beta & \mapsto & \sum_{i=1}^n x_i \beta^{-i}
    \end{array}
\end{equation}
is injective into $I_\beta$. We define an ordering $\prec$ on $\{0,1\}^n / \sim_\beta$ by 
\begin{equation}
    u \prec v \iff \varphi_\beta(u) < \varphi_\beta(v), \ \forall u,v \in \{0,1\}^n / \sim_\beta.
\end{equation}
For $x \in \{0,1\}^\ast$, we enumerate the elements of $\tilde g_\beta(x)$ as follows. We let $u_1(x), \ldots, u_{k}(x)$ such that $\{u_1(x), \ldots, u_k(x)\} = \tilde g_\beta(x)$ and $i < j \Rightarrow u_i(x) \prec u_j(x)$, for all $i,j \in \{1, \ldots, k\}$. We can then express $\Sigma_\beta(s,n,T)$ simply in function of the elements of $\tilde g_\beta(x)$. 
\begin{lemma}
    Let $\beta \in (1,2)$, $s \in [0,1]$, $n \in \N$, $T$ be a physical device and $x \in \Sigma_\beta(s,n,T)$. Then, there exists $i,j \in \{1, \ldots, \tilde \NN_g(x)\}$, $i \leq j$, such that 
    \begin{equation}
        \Sigma_\beta(s,n,T) = \bigcup_{\ell=i}^ju_\ell(x).
    \end{equation}
\end{lemma}
\begin{proof}
    Let $\beta \in (1,2)$, $s \in [0,1]$, $n \in \N$, $T$ be a physical device and $x \in \Sigma_\beta(s,n,T)$. The proof is in two parts: we first prove that EH NON IL EST PAS VRAI CE THEOREME BOLOSS.
\end{proof}


For a fixed $s \in [0,1]$, $n \in \N$ and $\xf \in \{0,1\}^\N$, recall that the sequence $(r_i)_{i \in \N}$ results from iterations of the function $K_{\beta,T}$, and define
\begin{equation}
    h_\beta(s,n,\xf,T) := \# \{r_i \in S : i \in \{1,\ldots,n  \} \}.
\end{equation}
In fact, $h_\beta(s,n,\xf,T)$ counts the number of times that Algorithm DAUBECHIES had to read the first bit of the infinite sequence of Bernoulli experiments in order to generate its first bit, i.e., the Algorithm had to read exactly the $h_\beta(s,n,\xf,T)$ first bits of the infinite sequence $\xf \in \{0,1\}^\N$ in order to generate its output. Note that the output of the Algorithm does not depend on the bits of $\xf$ located after the position $h_\beta(s,n,\xf,T)$, hence, for every $x \in \Sigma_\beta(s,n,T)$, there exists a sequence $\xf \in \{0,1\}^\N$ such that 
\begin{equation}
    \mathcal A_\beta(s,n,T)\left(\xf_{1:h_\beta(s,n,\xf,T)} \{0,1\}^\N\right) = \{x\}.
\end{equation}
Accordingly, we define 
\begin{equation}
    \noise_\beta(s,n,T,x) := \left\{u \in \{0,1\}^{\leq n} : \mathcal A_\beta(s,n,T)\left(u \{0,1\}^\N\right) = \{x\}\right\},
\end{equation}
for all $x \in \Sigma_\beta(s,n,T)$. We first construct two multivalued functions $f_{\beta, 1 \to all}, f_{\beta, 1+all \to \noise} : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ that are computable relatively to $\beta$, such that
\begin{equation}
    \langle \Sigma_\beta(s,n,T) \rangle \in f_{\beta, 1 \to all}\left(x\right), 
\end{equation}
and
\begin{equation}
    \langle \noise_\beta(s,n,T,x) \rangle \in f_{\beta , 1+all \to \noise}\left(\langle x,\langle \Sigma_\beta(s,n,T) \rangle \rangle \right),
\end{equation}
for all $s \in [0,1]$, $n \in \N$, and $x \in \Sigma_\beta(s,n,T)$. 



This implicitely defines a multivalued function $f_{\beta, 1 \to \noise} : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ by 
\begin{equation}
    f_{\beta, 1 \to \noise}(x) := f_{\beta , 1+all \to \noise}\left(\langle x, f_{\beta, 1 \to all}\left(x\right) \rangle \right), \ \forall x \in \{0,1\}^\ast.
\end{equation}




We denote by  the se
Note also that, in the above equation, the sequence $\xf_{1:h_\beta(s,n,\xf,T)}$ is uniquely determined by $x$.



Hence, the generation of the $\beta$-expansion can be hence seen as a nondeterministic process, where the nondeterministic part occurs only when the variable $r$ in Algorithm 4 belongs to the interval $[t - \varepsilon, t + \varepsilon]$. Indeed, when $r \in [t - \varepsilon, t + \varepsilon]$, $T$ delivers a random value, that can be seen as introducing noise. Given a real number $s \in [0,1]$, we let Algorithm 4 run for infinitely many time step, i.e. $n = \infty$. Denote by $i_1, i_2, \ldots $ the time steps for which the variable $r \in [t - \varepsilon, t + \varepsilon]$, and denote by $\xf \in \{0,1\}^\N$ be the sequence generated by the Algorithm, which is a $\beta$-expansion of $s$. The sequence $\xf$ is then generated deterministically, except for those elements $\xf_{i_1}, \xf_{i_2}, \ldots$ that have been generated randomly. We will show that, indeed, the sequence $\xf_{i_1}\xf_{i_2}\ldots $ can be seen as a noise, because the difference between the algorithmic complexity of $\xf$ and the algorithmic complexity of the $\beta$-expansion $\yf$ of $s$ that would be generated with a perfect threshold $t$ is lower bounded by the algorithmic complexity of $\xf_{i_1}\xf_{i_2}\ldots$. This is formally expressed as 
\begin{equation}
    \underline{\Delta}_\beta(\xf) \geq \log_\beta(2) \liminf_{n \to \infty} \frac{K[\xf_{i_1} \ldots \xf_{i_n}]}{n}\cdot
\end{equation}
OKKK: ALORS C'EST LE GROS BORDEL, LA FONCTION F 2 to BETA ETAIT PAS CALCULABLE !!
Accordingly, we define a function that converts a nondeterministic $\beta$-expansion of $s$ into the corresponding deterministic $\beta$-expansion and the noise introduced.
\begin{definition}\label{def:multivalued function converting from nondeterministic beta to deterministic beta + noise}
    OK JE POURRAIS D'ABORD DESIGNER LA FONCTION SEULEMENT POUR LE NOISE, PUIS LA COMBINER AVEC CELLE POUR L'EXPANSION BINAIRE
    Bon, cette fonction, elle prend comme input 2 entiers en plut de $x$. Ces entiers donnent la position exacte du premier et du dernier cluster de $\beta$-expansions de $s$. Ensuite, on peut donc extraire toutes les $\beta$-expansions de $s$. Là, on peut dessiner un arbre des beta-expansions et placer notre beta expansion dans cet arbre, et extraire chaque bit qui correspond à un branching de l'arbre. Formellement,
    Let $f^\beta_{ND\to D} : \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ be the multivalued function defined as 
\begin{align}\label{eq:main:def:multivalued function converting from base beta to base 2 + noise}
    f^\beta_{ND\to D}(\langle x, k, \ell \rangle) &:= x_{i_1, \ldots, i_h},
\end{align}
for all $x \in \{0,1\}^{n\log_\beta(2)}$ for some $n \in \N$, and $f^\beta_{ND\to D}(x) = \epsilon$ for $x \in \{0,1\}^m$ where $m \neq n \log_\beta(2)$ for all $n \in \N$.
\end{definition} 
PROUVER LE RESULTAT POUR $s \in \Q$??




\subsection{Formalisation of the ergodic problem}
Suppose that on input $s \in I_\beta$, the physical device $T$ delivers a bit $0$ or $1$, according to a Bernoulli probability distribution parametrized by the input $s$. We denote this parameter by $p(s)$. A example of $p(s)$ would be the following figure. For $n \in \N$ and $s \in I_\beta$, we denote by $\mathcal A_p(s,n) \in \{0,1\}^n$ the random variable that models the output of Algorithm 4 on input $s \in I_\beta$ and $n \in \N$, depending on $p$. Moreover, we define $\mathcal A_p(s) \in \{0,1\}^\N$ the be the random variable that models the output of Algorithm 4, it we would let it run infinitely long. More formally, this is expressed as follows. Then,
\begin{equation}
    \begin{array}{rccc}
        T_p : & I_\beta \times [0,1]^\N & \to & \{0,1\}\\
                       & r, \tff & \mapsto & \displaystyle  
                       \begin{cases}
                        0 \text{ if } \tff_1 \leq p(r)\\
                        1 \text{ if } \tff_1 > p(r).
                       \end{cases},
    \end{array}
\end{equation}
and the following equation of evolution
\begin{equation}
    \begin{array}{rccc}
        \mathcal K_p : & I_\beta \times [0,1]^\N & \to & I_\beta \times [0,1]^\N\\
                       & r, \tff &\displaystyle \mapsto &  \left(\beta r - T_p(r,\tff_1), \sigma \tff\right)
    \end{array}
\end{equation}
This translates to 
\begin{equation}
    \mathcal A_p(s, \tff) := \coprod_{i=1}^\infty T_p\left( \mathcal K_p^{i-1}(s, \tff)\right) =: \coprod_{i=1}^\infty a_i(s, \tff).
\end{equation}
Define $\supp p := \overline{\{s \in I_\beta : p(s) \in (0,1)\}}$, and for $s, \tff$, let $(I_i(s,\tff))_{i \in \N}$ be the increasing sequence of natural numbers satisfying 
\begin{equation}
    \{I_i(s,\tff) : i \in \N\} = \{ j \in \N : a_j(s,\tff) \in \supp p\}.
\end{equation}
Then, we can define the sequence of elements that where generated by a random process as 
\begin{equation}
    \mathcal R_p(s, \tff) := \coprod_{i=1}^\infty a_{I_i(s,\tff)}(s, \tff) := \coprod_{i=1}^\infty r_i(s, \tff).
\end{equation}

% Given a fixed number $s \in I_\beta$, we write $\mathcal A_s(\tff) := \mathcal A(s,\tff)$. Then, for $s \in I_\beta$, 
$A(s,\tff)$ is a random variable of distribution
\begin{equation}
    \mathcal A_{\#} \left(\lambda_\beta \otimes\lambda^\N\right),
\end{equation}
where $\lambda^\N$ is the infinite product of the Lebesgue measure, such that 
\begin{equation}
    \lambda^\N(C_1\times C_2 \times \ldots \times C_n \times [0,1]^\N) = \prod_{i=1}^n \lambda(C_i),
\end{equation}
for all $C_1, \ldots, C_n \subseteq [0,1]$ Borel sets. Then, for all $n \in \N$, 
\begin{equation}
    \mathbb E[K[\mathcal A_p(s, n)]] = \int_{\{0,1\}^\N}  K[\xf_{1:n}] d\mathcal A_{\#}\left(\lambda_\beta \otimes\lambda^\N\right).
\end{equation}



\subsection{Ergodic properties of the Daubechies algorithm: piecewise-constant case}

\subsection{Study for the piecewiese-constant case}

\subsection{A conjecture for the general case}



==> subfiles/proof_rational_case.tex <==
%! TEX root = ./main.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\texorpdfstring{Proof of the main result: case $\beta \in \Q$}{}}

\label{sec:new beta map}

We can use the dynamical system realization of the chunk-by-chunk greedy map described in (\ref{eq:greedy map chunks as dynamical system}) to generate chunks of a specific $\beta$-expansion of a given $s \in [0,1]$ by reading increasingly long prefixes of its greedy binary expansion. The generated $\beta$-expansion will then be proven to satisfy (\ref{eq:inequality to be proven}). The convertion prefix-to-chunk appears to be an important tool to control the behavior of the dynamical system, so that it indeed generates a $\beta$-expansion. Let $s \in [0,1]$ and $N \in \N$. When presented with increasingly long prefixes of $\gf_2(s)$ of respective lengths $\Sigma_i \in \N$, the dynamical system converts $\gf_2(s)_{1: \Sigma_i}$ to $\xf_{1: Ni}$, for $i \in \N$, where $\xf \in \Sigma_\beta(s)$. We will choose the $\Sigma_i$ to be such that $\limi{i} \frac{\Sigma_i}{Ni} = \log_2(\beta)$, which leads to (\ref{eq:inequality to be proven}) for $\beta \in \Q$. Specifically, we shall see that the dynamical system is realized by an effective algorithm. Figure \ref{fig:principle conversion greedy binary to beta exp} illustrates this process.
\begin{figure}[H]
	\centering
	\tikzmath{\x=3;}
	\tikzmath{\y1=0.25;}
	\tikzmath{\y2=0.5;}
	\tikzmath{\S=0.93;}
	\begin{tikzpicture}[scale = 0.8]
		\node[anchor = west] at (0,0.1){{\small $\gf_2(s) = 01001|0001|111|1001|000|1101|010|0000|001|1000|011|\ldots$}};
		\node[anchor = west] at (0,-\x){{\small$\xf = \underset{N}{000100}|\underset{N}{101000}|\underset{N}{001000}|101000|100000|101000|100000|100000|100000|010001|000010|\ldots$}};
		\draw[thick, ->] (2,-1.7) -- (2.9*\S-1, -\x + \y2);
		\draw[thick, ->] (4*\S,-1) -- (4.6*\S-0.7, -\x + \y2);
		\draw[thick, ->] (5*\S,-0.4) -- (6.1*\S-0.8, -\x + \y2);
		\draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-1.5) -- (3.1,-1.5) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_1$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-0.8) -- (4.2,-0.8) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_2$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-0.22) -- (5,-0.22) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_3$};
  	\path (5.5,-1.2) -- node[auto=false]{\ldots} (6.5,-1.2);
	\end{tikzpicture}
	\caption{Conversion of the greedy binary expansion $\gf_2(s)$ to a $\beta$-expansion $\xf$ of similar algorithmic complexity.}
	\label{fig:principle conversion greedy binary to beta exp}
\end{figure}

The chunks of the $\beta$-expansion $\xf$ are generated by the following iterative process. Suppose that at step $i \in \N_0$, $\xf_{1:Ni}$ has been generated from $\gf_2(s)_{1:\Sigma_i}$. Now, we read a next chunk of $\gf_2(s)$, of size $\Sigma_{i+1}-\Sigma_i$, so that we have at our disposal $\xf_{1:Ni}$ and $\gf_2(s)_{1:\Sigma_{i+1}}$, and we generate a chunk of $\xf$ of size $N$ by choosing the lexicographically maximal binary sequence $x \in \{0,1\}^N$ that satisfies 
\begin{equation}\label{eq:reducing the error between x beta and greedy binary}
	\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \frac{\beta^{-N(i+1)}}{\beta - 1} \leq \delta_\beta(\xf_{1:Ni}x) \leq \delta_2(\gf_2(s)_{1:\Sigma_{i+1}}),
\end{equation}
and take $\xf_{1:N(i+1)} := \xf_{1:Ni} x$. Using Lemma \ref{lem:factorisation of beta expansion through concatenation two}, one can rewrite (\ref{eq:reducing the error between x beta and greedy binary}) as
\begin{equation}\label{eq:first step towards x greedy exp of R i}
	\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \frac{\beta^{-N(i+1)}}{\beta - 1} \leq \delta_\beta(\xf_{1:Ni}) + \beta^{-Ni} \delta_\beta(x) \leq \delta_2(\gf_2(s)_{1:\Sigma_{i+1}}).
\end{equation}
Using again Lemma \ref{lem:factorisation of beta expansion through concatenation two}, we have
\begin{equation}\label{eq:factorisation binary expansion}
	\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) = \delta_2\left(\gf_2(s)_{1:\Sigma_{i}}\right) + 2^{-\Sigma_i}\delta_2\left(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}\right).
\end{equation}
By defining $R_0 = 0$, $\Sigma_0 = 0$,
\begin{equation}\label{eq:R i definition}
	R_i := \beta^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) - \delta_\beta(\xf_{1:Ni})\right), \ \text{for} \ i \in \N,
	\tag{\text{$\mathcal{R}$}}
\end{equation}
and
\begin{equation}\label{eq:s i to generate beta expansion}
	s_i := \frac{\beta^{Ni}}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}), \ \text{for} \ i \in \N_0,
	\tag{\text{$\mathcal{S}$}}
\end{equation}
(\ref{eq:first step towards x greedy exp of R i}) is equivalent to 
\begin{equation}\label{eq:greedy exp for x}
	R_i + s_i - \frac{\beta^{-N}}{\beta-1} \leq \delta_\beta(x) \leq R_i + s_i.
\end{equation}
$x \in \{0,1\}^N$ is then the lexicographically maximal sequence satisfying (\ref{eq:greedy exp for x}), which exactly corresponds to the first $N$ bits of the greedy $\beta$-expansion of $R_i+s_i$, i.e.
\begin{equation}
	x := d_\beta^N(R_i + s_i).
\end{equation}
Therefore, $\xf$ is iteratively defined as 
\begin{equation}
	\xf = \coprod_{i=0}^\infty \grpref\left(R_i + s_i\right).
\end{equation}
This exatcly matches (\ref{eq:inferring chunks of greedy expansion from R i E beta}), and
hence, the successive values taken by the variable $R_i$ correspond to the evolution of the dynamical system (\ref{eq:greedy map chunks as dynamical system}) given by
\begin{equation}
	\tag{\text{$E^N_\beta$}}
	R_{i+1} = G_\beta^N(R_i + s_i),
\end{equation}
when presented with input $\ssf =s_0s_1\ldots$ defined by (\ref{eq:s i to generate beta expansion}). 
However, one must pay attention to the fact that if $R_i + s_i \notin I_\beta$, then (\ref{eq:greedy map chunks as dynamical system}) is not well-defined as $G_\beta$ is defined on $I_\beta$ only. Using the interpretation in terms of a dynamical system, we establish conditions on $N,\Sigma_i$ so that, given $\beta$, (\ref{eq:greedy map chunks as dynamical system}) is well-defined, then we prove that the above procedure produces a valid $\beta$-expansion, and finally we study the algorithmic complexity of the delivered $\beta$-expansion.







% \begin{figure}[H]
% 	\centering
% 	\includegraphics[width=0.9\textwidth]{images/conversion_greedy_binary_to_beta_low_complex.png}
% 	% \caption{Principle of conversion from the greedy binary expansion $g_2(s)$ to a $\beta$-expansion $\xf_\beta(s)$ with similar algorithmic complexity.}
% 	% \label{fig:principle conversion greedy binary to beta exp}
% \end{figure}

% Before formally introducing the dynamical system, we show that the greedy map $G_\beta$ can be interpreted as a bit-shifting and a bit-extraction device. This vantage point is helpful in understanding the operational aspects of the dynamical system. Let $s \in [0,1]$ and denote its greedy expansion by $\xf$. Then, one has 
% \begin{equation}
% 	G_\beta(s) = G_\beta\left(\sum_{i=1}^\infty \xf_i \beta^{-i}\right) = \beta \left(\sum_{i=1}^\infty \xf_i \beta^{-i}\right) - \xf_1 = \sum_{i=1}^\infty \xf_{i+1} \beta^{-i}.
% \end{equation}
% which shows that application of $G_\beta$ simply shifts the sequence $x$ by one position to the left. It now follows directly that iterating $G_\beta$ $n$ times effects an left-shift by $n$ positions according to 
% \begin{equation}\label{eq:n iterations of greedy map is same as shifting n bits}
% 	G^n_\beta(s) = \sum_{i=1}^\infty \xf_{i+n} \beta^{-i}.
% \end{equation}
% Moreover, we can also interpret the greedy map as a bit-extraction device, namely by noting that
% \begin{equation}
% 	s - \frac{1}{\beta} G_\beta(s) = \sum_{i=1}^\infty \xf_i \beta^{-i} - \frac{1}{\beta}\sum_{i=1}^\infty \xf_{i+1} \beta^{-i} = \frac{\xf_1}{\beta}.
% \end{equation}

% Likewise, the first $n$ bits of the greedy $\beta$-expansion of $s$ can be extracted as
% \begin{equation}\label{eq:n iterations of greedy map is same as reading the first n bits}
% 	s - \frac{1}{\beta^n} G^n_\beta(s) = \sum_{i=1}^\infty \xf_i \beta^{-i} - \frac{1}{\beta^n}\sum_{i=1}^\infty \xf_{i+n} \beta^{-i} = \sum_{i=1}^n\xf_i \beta^{-i} = \delta_\beta(\xf_{1: n}).
% \end{equation}



% We will later prove that $\dom \beta$ is not empty for every $\beta \in (1,2)$.
% Accordingly, we define
% \begin{equation}\label{eq:definition of the low complex beta expansion}
% 	\xf_\beta(s)_{1:Ni} := \DD_\Theta(s_{0:i-1}), \ \ \text{for all} \ i \in \N_0,
% \end{equation}
% with $s_i$ satisfying (\ref{eq:s i to generate beta expansion}).

% We turn to the description of the ideas underlying the conception of the dynamical system just introduced. We suppose that $S_0 = s \in [0,1]$. 
% \begin{enumerate}
% 	\item We first give an interpretation of the sequence $S_i$. By iteration of (\ref{eq:definition of K beta}), one gets $S_i = G_2^{\sum_{j=0}^{i-1} M_j}(S_0)= G_2^{\Sigma_{i}}(s)$, for all $i \in \N$. As $G_2$ performs bitshifting in the greedy binary expansion, $S_i$ encodes the greedy binary expansion of $s$, with the first $\Sigma_{i} = \sum_{j=0}^{i-1} M_j$ bits removed. In Figure \ref{fig:principle conversion greedy binary to beta exp}, $S_i$ acts as a pointer indicating the starting locations of the chunks of size $M_{i}$ of the greedy binary expansion of $s$.
% 	\item We now give an interpretation of the sequence $S'_i$. Recall that $S'_i = S_{i} - \frac{1}{2^{M_{i}}}G_2^{M_{i}}(S_{i})$. As $s \mapsto s - \frac{1}{2^n}G^n_2(s)$ extracts the first $n$ bits of the greedy binary expansion of $s$, we deduce that $S'_i = S_{i} - \frac{1}{2^{M_{i}}}G_2^{M_{i}}(S_{i})$ encodes the first $M_i$ bits of the greedy binary expansion of $S_i$. Hence, $S'_i$ encodes the chunks of greedy binary expansion of $s$, with respective lengths $M_i$, and respective starting locations $\Sigma_i$.
% 	\item We move to the interpretation interpretation of the sequences $R_i$ and $R'_i$. $R_i$ is designed so that
% 	\begin{equation}
% 		R_i = \beta^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_i}) - \delta_\beta(X_i)\right),
% 	\end{equation}
% 	and can be interpreted as the approximation error between the $Ni$-prefix of $\xf_\beta(s)$ and the approximation of $s$ by the $\Sigma_i$-truncation of its greedy binary expansion. Further, $R'_i$ is designed so that
% 	\begin{equation}
% 		R'_i = \beta^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \delta_\beta(X_i)\right),
% 	\end{equation}
% 	and can be interpreted as the approximation error between the $Ni$-prefix of $\xf_\beta(s)$ and the approximation of $s$ by the $\Sigma_{i+1}$-truncation of its greedy binary expansion. The goal of the dynamical system is to reduce this approximation error by adding a chunk of size $N$ to the $Ni$-prefix of $\xf_\beta(s)$.
	
% 	The goal of the dynamical system is to constantly aim at $\delta_2(\gf_2(s)_{1:\Sigma_i})$ by adding bits to $X_i$, which is corresponds exactly to a controlled dynamical system in control theory. On Figure A is represented the block diagram of this controlled system.
% \end{enumerate}

% We now show that, indeed, (\ref{eq:definition of K beta}) is well-defined under suitable choices of $N$ and $\Sigma_i$. 
% Note that (\ref{eq:definition of K beta}) is well-defined is equivalent to say that (\ref{eq:reducing the error between x beta and greedy binary}) is satisfied, which, by the above discussion, implies that $\DD_\Theta(\ssf)$ is a $\beta$-expansion of $s$. We will prove this statement formally in the next subsection.

\subsection{The dynamical system is well-defined}



For (\ref{eq:greedy map chunks as dynamical system}) to be well-defined, we must have $R_i + s_i \in I_\beta$ for all $i \in \N_0$. We define
\begin{equation}
	\dom E_\beta^N := \left\{ \ssf \in I_\beta^\omega : R_i + s_i \in I_\beta, \ \forall i \in \N_0  \right\}.
\end{equation}
We will use the following result on the greedy map $G_\beta$, inspired from a note\footnote{On page 317: ``Notice that for each $x \in [0, \lfloor \beta\rfloor/(\beta-1)]$ there exists an integer $n_0 = n_0(x)$ such that for all $n \geq n_0$ one has $T_\beta^n(x) \in [0,1)$.''} in \cite[Section 1]{dajani2002greedy}, which states for all $t \in I_\beta$ and large enough $N \in \N$, $G_\beta^N(t) \in [0,1]$. This result will allow to tune $N$ so that $0 \leq R_i \leq 1$, and we will then tune the $\Sigma_i$ so that $0 \leq s_i \leq \frac{\beta}{2(\beta - 1)} - 1$. Altogether, this indeed yields $0 \leq R_i + s_i \leq \frac{\beta}{2} \frac{1}{\beta-1} < \frac{1}{\beta-1}$. We start with the result on the greedy map.
\begin{lemma}\label{ineq:greedy beta expansion}
	Let $\beta \in (1,2)$, $r \in I_\beta$, and set $N_\beta(r) =
		-\log_\beta\left(\frac{1-(\beta-1)r}{2 - \beta}\right)$. Then, for $n \in \N$, it holds that $n > N_\beta(r)$ if and only if
	\begin{equation}
		G^n_\beta(r) \in [0,1).
	\end{equation}
\end{lemma}
\begin{proof} Fix $\beta \in (1,2)$. The proof is divided two regimes for $r \in I_\beta$. First, note that if $r \in [0,1)$, then
	\begin{equation}
		G_\beta(r) \overset{(\ref{eq:greedy map})}{=} \begin{cases}
		\beta r, \ \text{if} \ r < \frac{1}{\beta},\\
		\beta r - 1, \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} \geq \begin{cases}
		\beta \times 0, \ \text{if} \ r < \frac{1}{\beta},\\
		\beta \times \frac{1}{\beta} -1, \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} = 0.
	\end{equation}
	and
	\begin{equation}
		G_\beta(r) \overset{(\ref{eq:greedy map})}{=} \begin{cases}
		\beta r, \ \text{if} \ r < \frac{1}{\beta},\\
		\beta r - 1, \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} < \begin{cases}
		\beta \times \frac{1}{\beta}, \ \text{if} \ r < \frac{1}{\beta},\\
		\beta \times 1 -1, \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} \leq 1.
	\end{equation}
	Therefore, $G_\beta([0,1)) \subseteq [0,1)$. Now, fix $x \in I_\beta \backslash [0,1) = \left[1,\frac{1}{\beta-1}\right]$, and take $m \in \N$ to satisfy $G^m_\beta(r) \geq 1$. As $G_\beta([0,1)) \subseteq [0,1)$, we must have for all $i \leq m$, that $G^i_\beta(r) \geq 1 \geq \frac{1}{\beta}$. Then, one gets
	\begin{equation}\label{eq:value of m to satisfy non greedy condition}
		1 \leq G^m_\beta(r) \overset{(\ref{eq:greedy map})}{=} (t \mapsto \beta t - 1)^m(r) = \beta^m r - \sum_{i=0}^{m-1} \beta^i = \beta^m r - \frac{\beta^m-1}{\beta-1} \cdot
	\end{equation}
	This is satisfied if and only if
	\begin{equation}
		m \leq -\log_\beta\left(\frac{1-(\beta-1)r}{2 - \beta}\right).
	\end{equation}
\end{proof}
\noindent We now move to the statement allowing to control $R_i$.
\begin{lemma}\label{eq:J beta is in dom E beta N}
	Let $\beta \in (1,2)$. If $N \geq \log_\beta(2)$ then $J_\beta^\omega \subset \dom E_\beta^N$, with 
	\begin{equation}\label{eq:definition J beta}
		J_\beta := \left[0, \frac{\beta}{2(\beta - 1)} - 1 \right] \neq \varnothing.
	\end{equation}
\end{lemma}
\begin{proof}
	Fix $\beta \in (1,2)$. We start by showing that $J_\beta$ is nonempty.
	The function $f : (1,2] \to \R$ defined as $f(\beta) = \frac{\beta/2}{\beta-1}$ for all $\beta \in (1,2]$ satisifies $f'(\beta) = -\frac{1}{2(\beta-1)^2} < 0$ for all $\beta \in (1,2]$ and $f(2) = 1$. Hence, $f$ is decreasing on $(1,2]$ and $f(2) = 1$, so $ \frac{\beta}{2(\beta - 1)} - 1 = f(\beta) - 1 > 0$ for all $\beta \in (1,2)$, yielding $J_\beta \neq \varnothing$.

	Now, let $\ssf = s_0s_1s_2\ldots \in J_\beta^\omega$. We suppose that $N \geq \log_\beta(2)$, and prove by induction
	\begin{equation}\label{eq:condition Ri si}
		R_i + s_i \in I'_\beta := \left[0, \frac{\beta/2}{\beta-1}\right] \subset \left[0, \frac{1}{\beta-1}\right] = I_\beta, \ \text{for all}\ i \in \N_0.
	\end{equation}
	We start by showing that $R_0 + s_0 \in I'_\beta$. Indeed, from the definition of $E_\beta^N$, $R_0 = 0$. Moreover, as $s_0 \in J_\beta$, one has
	\begin{equation}
		R_0 + s_0 = s_0 \in J_\beta \subset I'_\beta.
	\end{equation}
	We continue by proving that if $R_{i-1} + s_{i-1} \in I'_\beta$, then $R_{i} + s_i \in I'_\beta$, for all $i \in \N$. More precisely, we show that if $R_{i-1} + s_{i-1} \in I'_\beta$, then $R_i \in [0,1]$, which combined with $s_i \in J_\beta$ yields $R_i + s_i \in I'_\beta$, for all $i \in \N$. Fix $i \in \N$ and suppose that $R_{i-1} + s_{i-1}\in I'_\beta$. It follows from (\ref{eq:greedy map chunks as dynamical system}) that
	\begin{equation}\label{eq:relation R i+1 R i s i}
		R_i = G_\beta^N\left(R_{i-1}+s_{i-1}\right).
	\end{equation}
	By Lemma \ref{ineq:greedy beta expansion}, 
	\begin{equation}
		G_\beta^n\left(R_{i-1} + s_{i-1}\right) \in [0,1]
	\end{equation}
	for all
	\begin{equation}\label{eq:condition on n for convergence of greedy expansion}
		n \geq - \log_\beta\left( \frac{1 - (\beta - 1)(R_{i-1} + s_{i-1})}{2- \beta} \right).
	\end{equation}
	From $R_{i-1} + s_{i-1} \leq \frac{\beta/2}{\beta-1}$, one calculates
	\begin{align}
		- \log_\beta\left( \frac{1 - (\beta - 1)(R_{i-1}+s_{i-1})}{2- \beta} \right) \leq - \log_\beta\left( \frac{1 - (\beta - 1)\frac{\beta/2}{\beta-1}}{2- \beta} \right)
		 = \log_\beta(2)
		 \leq N.
	\end{align}
	Then, $N$ satisfies (\ref{eq:condition on n for convergence of greedy expansion}), so
	\begin{equation}\label{eq:R i is in 0 1}
		R_{i} \overset{(\ref{eq:relation R i+1 R i s i})}{=} G^N_\beta(R_{i-1} + s_{i-1}) \osetlem{\ref{ineq:greedy beta expansion}}{\in} [0,1].
	\end{equation}
	By virtue of inductive reasonning, we conclude that $R_i + s_i \in I'_\beta$ for all $i \in \N_0$, so $\ssf \in \dom E_\beta^N$.
\end{proof}
\noindent We finally tune $\Sigma_i$ so that $\ssf \in J_\beta^\omega$.
\begin{lemma}\label{lem:s is in J beta}
	Let $\beta \in (1,2)$, $s \in [0,1]$, $N \in \N$, $(\Sigma_i)_{i \in \N_0}$, and $\ssf = s_0s_1\ldots$ be defined according to (\ref{eq:s i to generate beta expansion}). Then, if $\Sigma_0 = 0$ and
	\begin{equation}\label{eq:conditions on sigma i to work}
		\Sigma_i \geq Ni\log_2(\beta)+\log_2\left(\frac{\beta -1}{2 - \beta}\right) + 1, \ \text{for all} \ i \in \N,
	\end{equation}
	we have $\ssf \in J_\beta^\omega$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2)$, $s \in [0,1]$, $N \in \N$, $(\Sigma_i)_{i \in \N_0}$ satisfying $\Sigma_0 = 0$ and (\ref{eq:conditions on sigma i to work}), and $\ssf = s_0s_1\ldots$ be defined by (\ref{eq:s i to generate beta expansion}). For $i \in \N_0$,
	\begin{equation}
		0 \leq s_i \overset{(\ref{eq:s i to generate beta expansion})}{=} \frac{\beta^{Ni}}{2^{\Sigma_i}} \delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) \leq \frac{\beta^{Ni}}{2^{\Sigma_i}} \leq \frac{\beta/2}{\beta-1} - 1,
	\end{equation}
	where (a) follows from $\delta_2 : \{0,1\}^\omega \to [0,1]$, and (b) is by (\ref{eq:conditions on sigma i to work}).
\end{proof}
We wrap up the last three results in a Theorem that states precise values for $N$ and $(\Sigma_i)_{i \in \N_0}$ so that $\ssf \in \dom E_\beta^N$.
\begin{theorem}\label{thm:condition on the input sequences so that s is in dom E}
	Let $s \in [0,1]$, $\beta \in (1,2)$, $\Sigma_0 = 0$ and
	\begin{equation}\label{eq:final value parameters}\tag{\text{$\mathcal{P}$}}
		\begin{array}{rl}
			N &:= \lceil \log_\beta(2) \rceil,\\
			\Sigma_i &:= \lceil Ni\log_2(\beta)\rceil + \left\lceil \log_2\left(\frac{\beta -1}{2 - \beta}\right) + 1 \right\rceil, \ \text{for all} \ i \in \N.
		\end{array}
	\end{equation}
	Then, for all $\ssf = s_0s_1\ldots$ defined according to (\ref{eq:s i to generate beta expansion}), $\ssf \in \dom E_\beta^N$.
\end{theorem}
\begin{proof}
	$N = \lceil \log_\beta(2) \rceil \geq \log_\beta(2)$, so by Lemma \ref{eq:J beta is in dom E beta N}, $J_\beta^\omega \subset \dom E_\beta^N$. Moreover, $\Sigma_i := \lceil Ni\log_2(\beta)\rceil + \left\lceil \log_2\left(\frac{\beta -1}{2 - \beta}\right) + 1 \right\rceil \geq Ni\log_2(\beta)+\log_2\left(\frac{\beta -1}{2 - \beta}\right) + 1$, for all $i \in \N$, Lemma \ref{lem:s is in J beta} implies that $\ssf \in J_\beta^\omega$.
\end{proof}
We now proceed to formally prove that the dynamical system indeed generates a $\beta$-expansion.

\subsection{\texorpdfstring{The dynamical system produces a valid $\beta$-expansion}{}}

\label{sec:control of X and Z}

In this section, we show that for $\beta \in (1,2)$ and $s \in [0,1]$, if we define $N$ and $(\Sigma_i)_{i \in \N}$ according to (\ref{eq:final value parameters}), and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion}), then $E_\beta^N(\ssf)$ is a $\beta$-expansion of $s$.

\begin{theorem}\label{thm:convergence rational dynamical system to beta expansion}
	Let $\beta \in (1,2)$, $(N,(\Sigma_i)_{i \in \N})$ be defined according to $(\ref{eq:final value parameters})$ and set $\Sigma_0 = 0$. Let $s \in [0,1]$ and define $\ssf = s_0s_1\ldots$ according to (\ref{eq:s i to generate beta expansion}). Then,
	\begin{equation}
		E_\beta^N(\ssf) \in \Sigma_\beta(s).
	\end{equation}
\end{theorem}
\begin{proof}
	Let $\beta \in (1,2)$, $(N,(\Sigma_i)_{i \in \N})$ be defined according to $(\ref{eq:final value parameters})$ and set $\Sigma_0 = 0$. Let $s \in [0,1]$ and define $\ssf = s_0s_1\ldots$ according to (\ref{eq:s i to generate beta expansion}). By Theorem \ref{thm:convergence rational dynamical system to beta expansion}, $E_\beta^N(\ssf)$ is well-defined. To prove that $E_\beta^N(\ssf) \in \Sigma_\beta(s)$, by (\ref{eq:definition beta expansion}) we need to show that $\delta_\beta(E_\beta^N(\ssf)) = s$. We will successively show 
	\begin{equation}\label{eq:prefixes of d theta converge to d theta}
		\limi{n} \delta_\beta(E_\beta^N(s_0s_1\ldots s_{n-1})) = \delta_\beta(E_\beta^N(\ssf))
	\end{equation}
	and
	\begin{equation}\label{eq:prefixes of d theta converge to s}
		\limi{n} \delta_\beta(E_\beta^N(s_0s_1\ldots s_{n-1})) = s,
	\end{equation}
	which combination leads to $\delta_\beta(E_\beta^N(\ssf)) = s$. We start by proving (\ref{eq:prefixes of d theta converge to d theta}). Let $n \in \N$. Note that
	\begin{align}
		E_\beta^N(\ssf)_{1:Nn} &\overset{(\ref{eq:inferring chunks of greedy expansion from R i E beta})}{=} \left[\coprod_{i=0}^\infty d_\beta^N\left(R_i + s_i\right)\right]_{1:Nn}\\
		&= \coprod_{i=0}^{n-1} d_\beta^N\left(R_i + s_i\right)\\
		&\overset{(\ref{eq:inferring prefix of chunks of greedy expansion from R i E beta})}{=} E_\beta^N(s_0s_1 \ldots s_{n-1}) \label{eq:d theta prefix is a prefix of d theta}
	\end{align}
	It follows that
	\begin{align}
		\delta_\beta(E_\beta^N(\ssf)) &= \delta_\beta(E_\beta^N(\ssf)_{1:Nn} E_\beta^N(\ssf)_{Nn+1:\infty})\\
		&\osetlem{\ref{lem:factorisation of beta expansion through concatenation two}}{=} \delta_\beta(E_\beta^N(\ssf)_{1:Nn}) + \beta^{-Nn} \delta_\beta(E_\beta^N(\ssf)_{Nn+1:\infty})\\
		&\overset{(a)}{\in} \delta_\beta(E_\beta^N(\ssf)_{1:Nn}) + \beta^{-Nn} I_\beta\\
		&\overset{(\ref{eq:d theta prefix is a prefix of d theta})}{=} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1}))  + \beta^{-Nn}I_\beta,
	\end{align}
	where (a) is by $\delta_\beta(\xf) \in I_\beta$, for all $\xf \in \{0,1\}^\omega$. Hence, 
	\begin{equation}
		0 \leq \limi{n} \left(\delta_\beta(E_\beta^N(\ssf)) - \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1}))\right) \leq \limi{n} \frac{\beta^{-Nn}}{\beta-1} = 0,
	\end{equation}
	yielding (\ref{eq:prefixes of d theta converge to d theta}). We move to the proof of (\ref{eq:prefixes of d theta converge to s}), which immediately follows from (\ref{eq:R i definition beta r}). Fix $n \in \N$. The dynamical system has been defined so that if (\ref{eq:s i to generate beta expansion}) holds, then 
	\begin{equation}
		R_n \overset{(\ref{eq:R i definition})}{=} \beta^{Nn}\left(\delta_2(\gf_2(s)_{\Sigma_i:\Sigma_{i+1}}) - \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1}))\right). 
	\end{equation}
	As (\ref{eq:final value parameters}) holds, Theorem \ref{thm:condition on the input sequences so that s is in dom E} implies that $\sf \in \dom E\beta^N$, i.e. $R_n + s_n \in I_\beta$. In particular, we have $0 \leq R_n \leq \frac{1}{\beta-1}$, so that
	\begin{equation}
		0 \leq \frac{R_i}{\beta^{Ni}} \overset{(\ref{eq:R i definition})}{=} \delta_2(\gf_2(s)_{\Sigma_i:\Sigma_{i+1}}) - \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1}))  \overset{(\ref{eq:R i definition})}{=} \frac{R_i}{\beta^{Ni}} \leq \frac{1}{(\beta-1) \beta^{Ni}} \underset{n \to \infty}{\to} 0.
	\end{equation}
	Therefore,
	\begin{equation}
		\limi{n} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) = \limi{n} \delta_2(\gf_2(s)_{\Sigma_i:\Sigma_{i+1}}) = s.
	\end{equation}
	This ends the proof.
	% Let $n \in \N$. 
	% \allowdisplaybreaks
	% \begin{align}
	% 	\delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) &\overset{(\ref{eq:inferring prefix of chunks of greedy expansion from R i E beta})}{=} \delta_\beta\left(\coprod_{i=0}^{n-1} d^N_\beta\left(R_i +  s_i\right)\right)\\
	% 	&\osetlem{\ref{lem:factorisation of beta expansion through concatenation}}{=}\sum_{i=0}^{n-1} \beta^{-Ni}\delta_\beta\left(d^N_\beta\left(R_i +  s_i\right)\right)\\
	% 	&\overset{(\ref{eq:definition multiple digit map})}{=}\sum_{i=0}^{n-1} \beta^{-Ni}\delta_\beta\left(\gf_\beta\left(R_i +  s_i\right)_{1:N}\right)\\
	% 	&\overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left( R_i +  s_i - \frac{1}{\beta^N}G^N_\beta\left(R_i +  s_i\right) \right)\\
	% 	&\overset{(\ref{eq:greedy map chunks as dynamical system})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left(R_i +s_i - \frac{1}{\beta^N}R_{i+1}\right)\\
	% 	&\overset{(\ref{eq:s i to generate beta expansion})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left(R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \frac{1}{\beta^N}R_{i+1}\right)\\
	% 	&= \sum_{i=0}^{n-1} \beta^{-Ni} R_i + \sum_{i=0}^{n-1} \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \sum_{i=0}^{n-1} \beta^{-N(i+1)} R_{i+1}\\
	% 	&= R_0 - \beta^{Nn}R_n + \sum_{i=0}^{n-1} \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}})\\
	% 	&\osetlem{\ref{lem:factorisation of beta expansion through concatenation}}{=} R_0 - \beta^{Nn}R_n + \delta_2(\gf_2(s)_{1:\Sigma_n}). \label{eq:intermediate equation delta beta x n}
	% \end{align}
	% From the definition of $E_\beta^N$, $R_0 = 0$. Moreover, as $(N, (\Sigma_i)_{i \in \N})$ satisfy (\ref{eq:final value parameters}), by (\ref{eq:R i is in 0 1}) one has $R_n \in [0,1]$. Therefore,
	% \begin{equation}
	% 	0 \geq \limi{n} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) - \delta_2(\gf_2(s)_{1:\Sigma_n}) \geq \limi{n} -\beta^{-Nn} = 0.
	% \end{equation}
	% As $\limi{n} \Sigma_n = \infty$, we then have
	% \begin{equation}
	% 	\limi{n} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) = \limi{n}\delta_2(\gf_2(s)_{1:\Sigma_n}) = s, 
	% \end{equation}
	% thereby finishing the proof.
\end{proof}

\subsection{\texorpdfstring{Algorithmic complexity of the $\beta$-expansion generated by the dynamical system}{}}


We have established that for $\beta \in (1,2)$, and $s \in [0,1]$, $E_\beta^N(\ssf)$ constitutes a valid $\beta$-expansion, assuming that (\ref{eq:final value parameters}) and (\ref{eq:s i to generate beta expansion}) hold. It remains to show that the algorithmic complexity of the prefixes of $E_\beta^N(\ssf)$ can be inferred from the algorithmic complexity of the prefixes of the greedy expansion $\gf_2(s)$. However, we can establish such a statement for $\beta \in \Q$ only. Indeed, the equations of the dynamical system that generate $E_\beta^N(\ssf)$ involve using the function $G_\beta$, which in full generality cannot be cast into an effective algorithm by virtue of requiring infinite precision. Instead, we would need another dynamical system which copes with approximations of $\beta$ only. We will develop this dynamical system in the next section. In this paragraph, we conclude the proof of (\ref{eq:inequality to be proven}), which establishes a relationship between the algorithmic complexity of the respective prefixes of $E_\beta^N(\ssf)$ and $\gf_2(s)$, respectively, for $\beta \in (1,2) \cap \Q$ only.

\begin{lemma}\label{lem:weak inequality binary beta expansion Kolmogorov rational}
	Let $\beta \in (1,2)\cap \Q$, $s \in [0,1]$ and $(N,(\Sigma_{i \in \N}))$ be defined according to (\ref{eq:final value parameters}). Then, there exists $\xf \in \Sigma_\beta(s)$, such that
	\begin{equation}
		K[\xf|N n] \leq K[\gf_2(s)|\Sigma_n] + c_\beta, \ \ \text{for all} \ n \in \N.
	\end{equation}
	where $c_\beta > 0$ depends only on $\beta$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2)\cap \Q$, $s \in [0,1]$, $(N,(\Sigma_{i \in \N}))$ satisfying (\ref{eq:final value parameters}), and $\ssf = s_0s_1\ldots$ defined according to (\ref{eq:s i to generate beta expansion}). By Theorem \ref{thm:convergence rational dynamical system to beta expansion}, $E_\beta^N(s_0s_1\ldots s_{n-1})$ is an $Nn$-prefix of $E_\beta^N(\ssf) \in \Sigma_\beta(s)$, for $n \in \N$. Since $\beta \in \Q$, (\ref{eq:greedy map chunks as dynamical system}) can be run on a digital computer because it requires only finite precision, and hence $E_\beta^N$ can be cast into the effective algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$ summarized in Algorithm \ref{alg:conversion binary expansion to beta expansion}. Note that $\varphi(\gf_2(s)_{1:\Sigma_n}) = E_\beta^N(s_0s_1\ldots s_{n-1}) = E_\beta^N(\ssf)_{1:Nn}$, for $n \in \N$. Therefore, by Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity} there exists $c_\varphi > 0$ such that
	\begin{equation}
		K[\xf|N n] \leq K[\gf_2(s)|\Sigma_n] + c_\varphi, \ \ \text{for all} \ n \in \N.
	\end{equation}
	$\varphi$ depends only on $E_\beta^N$, which itself depends only on $\beta$ as $N = \lceil \log_\beta(2) \rceil$. Hence, $c_\varphi$ depends only on $\beta$.
	\begin{algorithm}[H]
		\caption{$\beta$-expansion from a binary expansion}\label{alg:conversion binary expansion to beta expansion}
		\begin{algorithmic}[1]
			\Require $n \in \N$, $x \in \{0,1\}^\ast$
			\State Check that $|x| \geq \Sigma_n$, if not raise an error.
			\For{$i = 0, \ldots, n-1$}
			\State $s_i \gets \frac{\beta^{Ni}}{2^{\Sigma_i}}\delta_2(x_{\Sigma_i+1:\Sigma_{i+1}})$
			\EndFor
			\State \Return $E_\beta^N(s_0s_1\ldots s_{n-1})$
		\end{algorithmic}
	\end{algorithm}
\end{proof}

\begin{corollary}
	Let $\beta \in (1,2)\cap \Q$, $s \in [0,1]$. Then, there exists $\xf \in \Sigma_\beta(s)$, and $c_\beta > 0$ depending only on $\beta$, such that
	\begin{equation}\label{eq:algorithmic complexity of beta expansion lower than binary expansion}
		K[\xf|n] \leq K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] + c_\beta, \ \text{for all} \ n \in \N.
	\end{equation}
\end{corollary}
\begin{proof}
	Let $\beta \in (1,2)\cap \Q$, $s \in [0,1]$, and $(N,(\Sigma_{i \in \N}))$ be defined according to (\ref{eq:final value parameters}). By Lemma (\ref{lem:weak inequality binary beta expansion Kolmogorov rational}), there exists $\xf \in \Sigma_\beta(s)$, such that 
	\begin{equation}
		K[\xf|N n] \leq K[\gf_2(s)|\Sigma_n] + C_\beta, \ \ \text{for all} \ n \in \N.
	\end{equation}
	where $C_\beta > 0$ depends only on $\beta$. By (\ref{eq:simple inequality on concatenation of sequences}), there exists $c_N>0$, depending only on $N$, such that
\begin{equation}\label{eq:before ultimate equation proof kolmogorov}
	K[\xf)|n]  \leq K[\gf_2(s)|\Sigma_{\lfloor n/N\rfloor}] + C_\beta + c_N, \ \ \text{for all} \ n \in \N.
\end{equation}
Moreover, by setting $M = 3 + \left| \log_2\left(\frac{\beta - 1}{2 - \beta}\right)\right|$, (\ref{eq:final value parameters}) yields
\begin{equation}
	\lceil n \log_2(\beta) \rceil - M \leq\Sigma_{\lfloor n/N\rfloor} \leq \lceil n \log_2(\beta) \rceil + M, \ \text{ for all } \ n \in \N.
\end{equation}
Then, by Lemma \ref{lem:kolmogorov complexity of closed sequences}, there exists $c_M > 0$, depending only on $M$, such that
\begin{equation}\label{eq:before ultimate equation proof kolmogorov 2}
	K[\gf_2(s)|\Sigma_{\lfloor n/N\rfloor}] \leq K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] + c_M, \ \text{for all} \ n \in \N.
\end{equation}
By combining (\ref{eq:before ultimate equation proof kolmogorov}) and (\ref{eq:before ultimate equation proof kolmogorov 2}), one has
\begin{equation}
	K[\xf|n] \leq K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] + C_\beta + c_N + c_M, \ \text{for all} \ n \in \N.
\end{equation}
As $N$ and $M$ depend only on $\beta$, $c_N$ and $c_M$ depend only on $\beta$ as well. We then finish the proof by letting $c_\beta := C_\beta + c_N + C_M$.
\end{proof}
We have established a simple relation between the algorithmic complexity of the prefixes of a certain $\beta$-expansion and the algorithmic complexity of the prefixes of the greedy binary expansion, for $\beta\in \Q$. The proof was effected through the study of a dynamical system that delivers the $\beta$-expansion. In the next section, we slightly modify the dynamical system $E_\beta^N$ to establish a similar relation, that holds for general $\beta \in (1,2)$.

==> subfiles/proof_real_case.tex <==
%! TEX root = ./main.tex

\section{\texorpdfstring{Proof of the main result: case $\beta \in \R$}{}}



For $\beta \in (1,2) \backslash \Q$, one cannot cast (\ref{eq:greedy map chunks as dynamical system}) into an effective algorithm, because it uses comparisons with $\beta$ in its computations, which might require infinite precision. Here, we instead define a dynamical system that only manipulates finite-precision approximations of $\beta$. Inspired from the considerations which applied for the simpler case $\beta \in \Q \cap (1,2)$, we introduce a dynamical system which generates chunks of a $\beta$-expansion of a given $s \in [0,1]$ by reading increasingly long prefixes of both the greedy binary expansion of $s$ and $\beta - 1$. For computable $\beta \in (1,2)$, the generated $\beta$-expansion will then be proven to satisfy (\ref{eq:inequality to be proven}). Let $s \in [0,1]$ and $N\in \N$. When presented with increasingly long prefixes of $\gf_2(s)$ of respective lengths $\Sigma_i \in \N$, and increasingly long prefixes of $\gf_2(\beta)$ of respective lengths $\Lambda_i \in \N$, the dynamical system converts $\langle \gf_2(s)_{1: \Sigma_i}, \gf_2(\betaun)_{1: \Lambda_i}\rangle$ to $\xf_{1: Ni}$, for $i \in \N$, where $\xf \in \Sigma_\beta(s)$. We will choose the $\Sigma_i$ and $\Lambda_i$ to be such that $\limi{i} \frac{\Sigma_i}{Ni} = \log_2(\beta)$ and $\limi{i} \frac{\Lambda_i}{Ni} = 1$, which, in turn, leads to (\ref{eq:inequality to be proven}) for $\beta$ computable. Specifically, we shall see that the dynamical system is realized by an effective algorithm. Figure \ref{fig:principle conversion greedy binary to beta exp beta r} illustrates this process. 
\begin{figure}[H]
	\centering
	\tikzmath{\x=3;}
	\tikzmath{\y1=0.25;}
	\tikzmath{\y2=0.5;}
	\tikzmath{\S=0.93;}
	\begin{tikzpicture}[scale = 0.8]
		\node[anchor = west] at (9.35,0.1){{\small $\gf_2(\betaun) = 01001|0001|111|1001|000|1101|\ldots$}};
		\node[anchor = west] at (0,0.1){{\small $\gf_2(s) = 01001|0001|111|1001|000|1101|\ldots$}};
		\node[anchor = west] at (5.7,-\x){{\small$\xf = \underset{N}{000100}|\underset{N}{101000}|\underset{N}{001000}|101000|\ldots$}};
		\draw[thick, ->] (2.8,-1.7) -- (2.9*\S+4.1, -\x + \y2-0.1);
		\draw[thick, ->] (4*\S,-1) -- (4.6*\S+4.5, -\x + \y2);
		\draw[thick, ->] (5*\S,-0.4) -- (6.1*\S+4.5, -\x + \y2);
		\draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-1.5) -- (3.1,-1.5) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_1$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-0.8) -- (4.2,-0.8) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_2$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (1.9,-0.22) -- (5,-0.22) node[midway, yshift = -0.9em]{\scriptsize$\Sigma_3$};
  
  \draw[thick, ->] (12,-0.34) -- (2.9*\S+5, -\x + \y2);
		\draw[thick, ->] (12,-0.92) -- (4.6*\S+5, -\x + \y2);
		\draw[thick, ->] (5*\S+7.6,-1.64) -- (6.1*\S+5.5, -\x + \y2);
		\draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (11.9,-0.22) -- (13.1,-0.22) node[midway, yshift = -0.9em]{\scriptsize$\Lambda_1$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (11.9,-0.8) -- (14.2,-0.8) node[midway, yshift = -0.9em]{\scriptsize$\Lambda_2$};
  \draw [decorate,decoration={brace,amplitude=5pt,mirror}]
  (11.9,-1.5) -- (15,-1.5) node[midway, yshift = -0.9em]{\scriptsize$\Lambda_3$};
	\end{tikzpicture}
	\caption{Conversion of the greedy binary expansions $\gf_2(s)$ and $\gf_2(\beta \hspace{-0.5mm} - \hspace{-0.5mm} 1)$ to a $\beta$-expansion $\xf$ of similar algorithmic complexity.}
	\label{fig:principle conversion greedy binary to beta exp beta r}
\end{figure}

The chunks of the $\beta$-expansion $\xf$ are generated by the following iterative process. Suppose that at step $i \in \N_0$, the first $i$ chunks of $\xf$ of size $N$ have been generated from has been generated from $\gf_2(s)_{1:\Sigma_i}$ and $\gf_2(\betaun)_{1:\Lambda_i}$ Now, we read the next chunk of $\gf_2(s)$, of size $\Sigma_{i+1}-\Sigma_i$, and the next chunk of $\gf_2(\betaun)$, of size $\Lambda_{i+1}-\Lambda_i$. We define 
\begin{equation}\label{eq:beta i to generate beta expansion beta r}
	\tag{\text{$\mathcal B$}}
	\beta_{i+1} := 1+\delta_2(\gf_2(\betaun)_{1:\Lambda_{i+1}}),
\end{equation}
and we generate a chunk $\xf$ of size $N$ by choosing the lexicographically maximal binary sequence $x \in \{0,1\}^N$ that satisfies 
\begin{equation}\label{eq:reducing the error between x beta and greedy binary beta r}
	\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \beta_{i+1}^{-N(i+1)} \leq \delta_{\beta_{i+1}}(\xf_{1:Ni}x) \leq \delta_2(\gf_2(s)_{1:\Sigma_{i+1}}),
\end{equation}
and take $\xf_{1:N(i+1)} := \xf_{1:Ni} x$. Using Lemma \ref{lem:factorisation of beta expansion through concatenation}, one can rewrite (\ref{eq:reducing the error between x beta and greedy binary beta r}) as
\begin{equation}\label{eq:first step towards x greedy exp of R i beta r}
	\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \frac{\beta_{i+1}^{-N(i+1)}}{\beta_{i+1} - 1} \leq \delta_{\beta_{i+1}}(\xf_{1:Ni}) + \beta^{-Ni} \delta_{\beta_{i+1}}(x) \leq \delta_2(\gf_2(s)_{1:\Sigma_{i+1}}).
\end{equation}
By defining $R_0 = 0$, $\Sigma_0 = 0$,
\begin{equation}\label{eq:R i definition beta r}
		R_i := \beta_{i+1}^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) - \delta_{\beta_{i}}(\xf_{1:Ni})\right), \ \text{for} \ i \in \N,
	\tag{\text{$\mathcal{R'}$}}
\end{equation}
\begin{equation}\label{eq:s i to generate beta expansion beta r}
	s_i := \frac{\beta_{i+1}^{Ni}}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}), \ \text{for} \ i \in \N_0,
	\tag{\text{$\mathcal{S'}$}}
\end{equation}
and
\begin{equation}\label{eq:epsilon i to generate beta expansion beta r}
	\varepsilon_i := \beta_{i+1}^{Ni} \left(\delta_{\beta_{i}}(\xf_{1:Ni}) - \delta_{\beta_{i+1}}(\xf_{1:Ni})\right), \ \text{for} \ i \in \N_0, \tag{\text{$\varepsilon$}}
\end{equation}
(\ref{eq:first step towards x greedy exp of R i}) is equivalent to 
\begin{equation}\label{eq:greedy exp for x beta r}
	R_i + s_i + \varepsilon_i - \frac{\beta_{i+1}^{-N}}{\beta_{i+1}-1} \leq \delta_{\beta_{i+1}}(x) \leq R_i + s_i + \varepsilon_i.
\end{equation}
$x \in \{0,1\}^N$ is then seen to be the lexicographically maximal sequence satisfying (\ref{eq:greedy exp for x}), which exactly corresponds to the first $N$ bits of the greedy $\beta$-expansion of $R_i + s_i + \varepsilon$, i.e.
\begin{equation}\label{eq:def x n i x n i + 1}
	x := d_{\beta_{i+1}}^N(R_i + s_i + \varepsilon_i).
\end{equation}
Therefore, $\xf$ is iteratively defined as 
\begin{equation}
	\xf = \coprod_{i=0}^\infty d_{\beta_{i+1}}^N\left(R_i + s_i+\varepsilon_i\right).
\end{equation}
This does not match (\ref{eq:inferring chunks of greedy expansion from R i E beta}), and
hence, as opposed to the simpler the case $\beta \in \Q$, we cannot conclude on the relation between $R_{i+1}$ and $R_i$. Instead, we establish the relation as follows. For $i \in \N_0$, we have
\allowdisplaybreaks
\begin{align}
	R_{i+1} &\overset{(\ref{eq:R i definition beta r})}{=}\beta_{i+2}^{N(i+1)}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i+1}}) - \delta_{\beta_{i+1}}(\xf_{1:N(i+1)})\right)\\
	& \osetlem{\ref{lem:factorisation of beta expansion through concatenation two}}{=} \beta_{i+2}^{N(i+1)}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) + \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \delta_{\beta_{i+1}}(\xf_{1:Ni}) \right.\nonumber\\
	&  \hspace{2.3cm}\left. - \frac{1}{\beta_{i+1}^{Ni}}\delta_{\beta_{i+1}}(\xf_{Ni+1:N(i+1)}) \right)\\
	& = \beta_{i+2}^{N(i+1)}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) + \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \delta_{\beta_{i+1}}(\xf_{1:Ni}) \right.\nonumber\\
	&  \hspace{2.3cm} \left. - \delta_{\beta_i}(\xf_{1:Ni}) + \delta_{\beta_i}(\xf_{1:Ni}) - \frac{1}{\beta_{i+1}^{Ni}}\delta_{\beta_{i+1}}(\xf_{Ni+1:N(i+1)}) \right)\\
	& = \frac{\beta_{i+2}^{N(i+1)}}{\beta_{i+1}^{Ni}}\left(\beta_{i+1}^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) - \delta_{\beta_i}(\xf_{1:Ni})\right) + \frac{\beta_{i+1}^{Ni}}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}})  \right.\nonumber\\
	&  \hspace{2.3cm} \left. + \beta_{i+1}^{Ni}\left(\delta_{\beta_i}(\xf_{1:Ni}) - \delta_{\beta_{i+1}}(\xf_{1:Ni})\right)  - \delta_{\beta_{i+1}}(\xf_{Ni+1:N(i+1)}) \right)\\
	& \overset{\substack{(\ref{eq:R i definition beta r})\\ (\ref{eq:s i to generate beta expansion beta r})\\ (\ref{eq:epsilon i to generate beta expansion beta r})}}{=} \frac{\beta_{i+2}^{N(i+1)}}{\beta_{i+1}^{Ni}}\left(R_i + s_i + \varepsilon_i  - \delta_{\beta_{i+1}}\left(\xf_{Ni+1:N(i+1)}\right) \right)\\
	& \overset{(\ref{eq:def x n i x n i + 1})}{=} \frac{\beta_{i+2}^{N(i+1)}}{\beta_{i+1}^{Ni}}\left(R_i + s_i + \varepsilon_i  - \delta_{\beta_{i+1}}\left(d_{\beta_{i+1}}^N\left(R_i + s_i + \varepsilon_i\right)\right) \right)\\
	&\overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=} \frac{\beta_{i+2}^{N(i+1)}}{\beta_{i+1}^{Ni}} \frac{1}{\beta_{i+1}^{N}} G^N_{\beta_{i+1}}\left( R_i + s_i + \varepsilon_i\right).
\end{align}
We conclude on the relation
\begin{equation}
	R_{i+1} = \left(\frac{\beta_{i+2}}{\beta_{i+1}}\right)^{N(i+1)} G^N_{\beta_{i+1}}\left( R_i + s_i + \varepsilon_i\right).
\end{equation}
Note that in the above equation, $\varepsilon_i$ depends on $\xf_{1:Ni}$. The dynamical system hence needs to record the successive values taken by $\xf_{1:Ni}$. For that purpose, we add an extra variable, denoted by $X_i$, such that $X_i = \xf_{1:Ni}$. The dynamical system will hence be defined by a system of equations instead of just one equation.
\begin{equation}\label{eq:R i X i + 1 definition of E N}
	\begin{array}{rr}
		R_{i+1} =& \left(\frac{\beta_{i+2}}{\beta_{i+1}}\right)^{N(i+1)} G^N_{\beta_{i+1}}\left( R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right),\\
	X_{i+1} =& X_i \, d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right).
	\end{array}
	\tag{\text{$\mathcal E_N$}}
\end{equation}
where $\varepsilon_N(x, t_1, t_2 , i) := t_2^{Ni}\left(\delta_{t_1}(x) - \delta_{t_2}(x)\right)$, for all $x \in \{0,1\}^\ast$, $t_1,t_2 \in (1,2)$ and $i \in \N_0$.
Similarly as for $E_\beta^N$, when presented with inputs $\ssf = s_0s_1\ldots \in  I_\beta^\omega$ and $\betaf = \beta_0\beta_1\ldots \in  (1,2)^\omega$, we can see $\EE_N$ as a mapping $ \bigcup_{n \in \N_0} \left(I_\beta^n \times (1,2)^n\right) \to \{0,1\}^n$ by $\EE_N(\epsilon, \epsilon) := \epsilon$ and
\begin{equation}\label{eq:inferring prefix of chunks of greedy expansion from R i E beta i}
	\EE_N(s_0s_1\ldots s_{n-1}, \beta_0\beta_1\ldots \beta_n) := X_{n-1} = \coprod_{i=0}^{n-1} d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right), 
\end{equation}
for all $n \in \N$, and as a mapping $I_\beta^\omega \times (1,2)^\omega \to \{0,1\}^\omega$ through
\begin{equation}\label{eq:inferring chunks of greedy expansion from R i E beta i}
	\EE_N(\ssf, \betaf) := \limi{n} X_n = \coprod_{i=0}^{\infty} d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right).
\end{equation}
One must pay attention to the fact that if $R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \notin I_{\beta_{i+1}}$, then (\ref{eq:R i X i + 1 definition of E N}) is not well-defined as $G_{\beta_{i+1}}$ is defined on $I_{\beta_{i+1}}$ only. Using the interpretation in terms of a dynamical system, we establish conditions on $N,\Sigma_i, \Lambda_i$ so that, given $\beta$, (\ref{eq:R i X i + 1 definition of E N}) is well-defined, then prove that the above procedure produces a valid $\beta$-expansion, and finally study the algorithmic complexity of the delivered $\beta$-expansion.

\subsection{The dynamical system is well-defined}

For (\ref{eq:R i X i + 1 definition of E N}) to be well-defined, we must have $R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I_{\beta_{i+1}}$ for all $i \in \N_0$. Note that $\beta_i \leq \beta$ implies $I_{\beta} \subset I_{\beta_{i+1}}$, for all $i \in \N_0$. Therefore, in this case, this is sufficient to impose $R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I_{\beta}$ for all $i \in \N_0$. We define
\begin{equation}
	\dom \EE_N(\beta) := \left\{ \ssf \in I_\beta^\omega, \betaf \in (1,\beta]^\omega : R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I_{\beta}, \ \forall i \in \N_0  \right\}.
\end{equation}
The structure of the proof is almost identical to the proof of the well-definition of (\ref{eq:greedy map chunks as dynamical system}) for the simpler case $\beta \in \Q$. Concretely, we set $K_\beta := \frac{1}{3}J_\beta$, where $J_\beta \neq \varnothing$ is defined by (\ref{eq:definition J beta}), for $\beta \in (1,2)$, such that $I'_\beta := [0,1] + 3K_\beta = [0, \frac{\beta/2}{\beta-1}] \subset [0, \frac{1}{\beta-1}] = I_\beta$. We will prove, under certain conditions on $N$, $\Sigma_i$ and $\Lambda_i$, that $R_i \in [0,1] + K_\beta$, $s_i \in K_{\beta}$ and $\varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in K_{\beta}$, resulting in
\begin{equation}
	\underset{\in [0,1]+K_\beta}{\underbrace{R_i}} + \underset{\in K_\beta}{\underbrace{s_i}} + \underset{\in K_\beta}{\underbrace{\varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)}} \in [0,1] + 3K_\beta \subset I_\beta.
\end{equation}
We start by proving that under some conditions on $N$, $\ssf$ and $\betaf$, $\EE_N$ is well-defined. For $\beta \in (1,2)$, we define $\lowbeta := 1 + \frac{\beta-1}{10} > 1$ and introduce the set $A_\beta = \left[\lowbeta, \beta \right] \subset (1,\beta)$, displayed on Figure \ref{fig:set A beta}, that will turn out very useful in the upcoming discussion.
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[scale = 5]
		\draw (0,0) -- (2,0);
		\draw (0,-0.02) -- (0,0.02);
		\draw (1,-0.02) -- (1,0.02);
		\draw (2,-0.02) -- (2,0.02);
		\draw[blue] (1.06,-0.02) -- (1.06,0.02);
		\draw[blue] (1.6,-0.02) -- (1.6,0.02);
		\draw[blue, thick] (1.06,0) -- (1.6,0);
		\node[below] at (0,-0.015){$0$};
		\node[below] at (1,-0.015){$1$};
		\node[below] at (2,-0.015){$2$};
		\node[above] at (1.12,-0.012){\tiny $1 + \frac{\beta-1}{10}$};
		\node[above] at (1.6,-0.008){\tiny $\beta$};
		\node[below] at (1.3,-0.008){\footnotesize $A_\beta$};
	\end{tikzpicture}
	\caption{Example of $A_\beta$ for $\beta = 1.6$.}
	\label{fig:set A beta}
\end{figure}
We first make explicit a subset of $I_\beta^\omega \times (1, 2)^\omega$ taht is included in $\dom \EE_N(\beta)$.
\begin{lemma}\label{eq:J beta is in dom E beta N beta r}
	Let $\beta \in (1,2)$. If 
	\begin{equation}\label{eq:condition on N}
		\tag{$\mathcal N$}
		N \geq \log_{\lowbeta}(2) + \log_{\lowbeta}\left( \frac{2- {\lowbeta}}{2 - \beta} \right),
	\end{equation}
	then
	\begin{equation}
		K_\beta^\omega \times \mathcal U_N(\beta) \subset \dom \EE_N(\beta),
	\end{equation}
	where $\mathcal U_N(\beta) := A_\beta^\omega \cap \mathcal V_N(\beta) \cap \mathcal W_N(\beta)$, with
	\begin{equation}\label{eq:definition V beta N}
		\mathcal V_N(\beta) := \left\{ \betaf \in (1,2]^\omega : \varepsilon_N(x, \beta_i, \beta_{i+1} , i) \in K_{\beta}, \ \text{for all} \ x \in \{0,1\}^{Ni}, \ i \in \N_0 \right\},
	\end{equation}
	and
	\begin{equation}\label{eq:definition W beta N}
		\mathcal W_N(\beta) := \left\{ \betaf \in (1,2]^\omega : \left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} \in [0,1] + K_{\beta}, \ i \in \N_0 \right\}.
	\end{equation}
\end{lemma}
\begin{proof} 
	Let $\beta \in (1,2)$, $N \geq \log_\beta(2)$, $\ssf = s_0s_1s_2\ldots \in K_\beta^\omega$ and $\betaf =\beta_0\beta_1\ldots \in \mathcal U_N(\beta)$. We prove by induction that
	\begin{equation}\label{eq:condition Ri si beta i}
		R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I'_\beta = [0,1] + 3K_\beta \subset I_\beta, \ \text{for all}\ i \in \N_0.
	\end{equation}
	We start by showing that $R_0 + s_0 + \varepsilon_N(X_0, \beta_0, \beta_{1} , 0) \in I'_\beta$. Indeed, from the definition of $\EE_N$, $R_0 = 0$. Moreover, as $s_0 \in K_\beta$ and $\betaf \in \mathcal V_N(\beta)$, one has
	\begin{equation}
		R_0 + s_0 + \varepsilon_N(X_0, \beta_0, \beta_{0+1} , 0) = s_0 + \varepsilon_N(X_0, \beta_0, \beta_{1} , 0) \in K_\beta + K_\beta \subset I'_\beta.
	\end{equation}
	We continue by proving that if $S_{i-1} := R_{i-1} + s_{i-1} + \varepsilon_N(X_{i-1}, \beta_{i-1}, \beta_{i} , i-1)  \in I'_\beta$, then $S_i := R_{i} + s_i+ \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I'_\beta$, for all $i \in \N$. Fix $i \in \N$ and suppose that $S_{i-1}\in I'_\beta$. It follows from (\ref{eq:R i X i + 1 definition of E N}) that
	\begin{equation}\label{eq:relation R i+1 R i s i beta i}
		R_i = \left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} G_{\beta_{i+1}}^N\left(S_{i-1}\right).
	\end{equation}
	By Lemma \ref{ineq:greedy beta expansion}, 
	\begin{equation}
		G_{\beta_{i+1}}^n\left(S_{i-1}\right) \in [0,1]
	\end{equation}
	for all
	\begin{equation}\label{eq:condition on n for convergence of greedy expansion beta r}
		n \geq - \log_{\beta_{i+1}}\left( \frac{1 - ({\beta_{i+1}} - 1)S_{i-1}}{2- {\beta_{i+1}}} \right).
	\end{equation}
	From $S_{i-1} \in I'_\beta = \left[0, \frac{\beta/2}{\beta-1}\right]$, one calculates
	\begin{align}
		- \log_{\beta_{i+1}}\left( \frac{1 - ({\beta_{i+1}} - 1)S_{i-1}}{2- {\beta_{i+1}}} \right) &\leq - \log_{\beta_{i+1}}\left( \frac{1 - ({\beta_{i+1}} - 1)\frac{\beta/2}{\beta-1}}{2- {\beta_{i+1}}} \right)\overset{(a)}{\leq} - \log_{\beta_{i+1}}\left( \frac{1 - \beta/2}{2- {\beta_{i+1}}} \right)\nonumber\\
		& = \log_{\beta_{i+1}}(2) + \log_{\beta_{i+1}}\left( \frac{2- {\beta_{i+1}}}{2 - \beta} \right)\\
		&\overset{(b)}{\leq} \log_{\lowbeta}(2) + \log_{\lowbeta}\left( \frac{2- {\lowbeta}}{2 - \beta} \right)\\
		& \leq N,
	\end{align}
	where (a) and (b) use that $\beta_{i+1} \in A_\beta = [\lowbeta, \beta]$
	Then, $N$ satisfies (\ref{eq:condition on n for convergence of greedy expansion beta r}), so
	\allowdisplaybreaks
	\begin{align}\label{eq:R i is in 0 1 beta r}
		R_{i} &\overset{(\ref{eq:relation R i+1 R i s i beta i})}{=} \left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} G^N_\beta(R_{i-1} + s_{i-1} + \varepsilon_N(X_{i-1}, \beta_{i-1}, \beta_{i} , i-1))\\
		& \osetlem{\ref{ineq:greedy beta expansion}}{\in} \left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni}[0,1] \overset{(a)}{=} [0,1] + K_\beta,
	\end{align}
	where (a) follows from $\betaf \in \mathcal W_N(\beta)$, which implies $\left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} \in [0,1] + K_\beta$. Moreover, $s_i \in K_\beta$ and $\betaf \in \mathcal V_N(\beta)$, so we have $\varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in K_\beta$. It follows that $R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in [0,1] + 3 K_\beta = I'_\beta$. By virtue of inductive reasonning, we conclude that $R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i) \in I'_\beta$ for all $i \in \N_0$, so $(\ssf,\betaf) \in \dom \EE_N$.
\end{proof}
We now identify explicit subsets of $\mathcal V_N(\beta)$ and $\mathcal W_N(\beta)$. We start by making explicit a subset $\mathcal V'_N(\beta) \subset \mathcal V_N(\beta)$. For $\beta \in (1,2)$, define $C_\beta := \max K_\beta$.

\begin{definition} Let $\beta \in (1,2)$ and $N \in \N$. We say that $\betaf \in (1,\beta)^\omega$ converges $N$-fast towards $\beta$ if 
	\begin{equation}\label{eq:C N fast converging}
		|\beta - \beta_i| \leq \frac{\min\{1,C_\beta\}}{e\beta^{Ni}N^2i^2}, \ \text{for all} \ i \in \N.
	\end{equation}
We denote by $\mathcal Z_N(\beta)$ the set of nondecreasing sequences $\betaf \in (1,\beta)^\omega$ that converge $N$-fast towards $\beta$.
\end{definition}
\begin{lemma}\label{lem:beta C N converging implies bounded error}
	For $\beta \in (1,2)$ and $N \in \N$, $\mathcal Z_N(\beta)\subset \mathcal V_N(\beta) \cap W_N(\beta)$. 
\end{lemma}
\begin{proof} Let $\beta \in (1,2)$, $N \in \N$ and $\betaf \in \mathcal Z_N(\beta)$. We first show that $\mathcal Z_N(\beta) \subset \mathcal V_N(\beta)$, and then move to the proof of $\mathcal Z_N(\beta) \subset \mathcal W_N(\beta)$. Fix $i \in \N_0$ and $x \in \{0,1\}^{Ni}$. We will show that $\betaf \in \mathcal V_N(\beta)$ by proving that $\varepsilon_N(x, \beta_i, \beta_{i+1} , i) \in K_\beta =: [0, C_\beta]$. First note that $\varepsilon_N(\epsilon, \beta_0, \beta_{1} , 0) = 0 \in K_\beta$, so the case $i = 0$ is dealt with. Suppose in the following that $i \geq 1$. As $\betaf$ is nondecreasing, $\beta_i \leq \beta_{i+1}$ so $\delta_{\beta_i}(x) \geq \delta_{\beta_{i+1}}(x)$, and hence $0 \leq \beta_{i+1}^{Ni}\left(\delta_{\beta_i}(x) - \delta_{\beta_{i+1}}(x)\right) = \varepsilon_N(x, \beta_i, \beta_{i+1} , i)$. Let us now prove that $\varepsilon_N(x, \beta_i, \beta_{i+1} , i) \leq C_\beta$.
	\begin{align}
		\delta_{\beta_i}(x) - \delta_{\beta_{i+1}}(x) &= \sum_{j=1}^{Ni} x_j \beta_i^{-j} - \sum_{j=1}^{Ni} x_j \beta_{i+1}^{-j} = \sum_{j=1}^{Ni} x_j \left(\beta_i^{-j} -  \beta_{i+1}^{-j}\right)\\
		&\leq \sum_{j=1}^{Ni} x_j  \left(\beta_i^{-j} - \beta_{i+1}^{-j}\right) \overset{(a)}{\leq} \sum_{j=1}^{Ni}  \left(\beta_i^{-j} - \beta_{i+1}^{-j}\right), \label{eq:weak eq bounding delta beta variations}
	\end{align}
	where (a) is by $x_i \leq 1$.
	Note that for all $\beta \in [1,2)$, $\left|\frac{\partial \beta^{-j}}{\partial \beta}\right| = -j \beta^{-(j+1)} \geq -j$, for all $j \in \N$. Then, by using the mean value theorem, one gets $\beta_{i}^{-j} - \beta_{i+1}^{-j} \leq j (\beta_i - \beta_{i+1})$ for all $j \in \N$. By (\ref{eq:weak eq bounding delta beta variations}),
	\begin{align}
		\beta_{i+1}^{Ni}\left(\delta_{\beta_i}(x) - \delta_{\beta_{i+1}}(x)\right) &\leq \beta_{i+1}^{Ni} \sum_{j=1}^{Ni} j (\beta_i - \beta_{i+1}) = \beta_{i+1}^{Ni} \frac{Ni(Ni+1)}{2} (\beta_i - \beta_{i+1})\\
		&\leq \beta_{i+1}^{Ni} N^2i^2 (\beta_i - \beta_{i+1}) \overset{(a)}{\leq} \beta_{i+1}^{Ni} N^2i^2 (\beta - \beta_{i+1}) \overset{(\ref{eq:C N fast converging})}{\leq} C_\beta,
	\end{align}
	where (a) follows from $\betaf$ being nondecreasing. This finishes the proof that $\mathcal Z_N(\beta) \subset \mathcal V_N(\beta)$. We now prove that $\mathcal Z_N(\beta) \subset \mathcal W_N(\beta)$. Fix $i \in \N_0$ and $x \in \{0,1\}^{Ni}$. We will show that $\betaf \in \mathcal W_N(\beta)$ by proving that $\left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} \in [0,1] + K_\beta =: [0, 1+ C_\beta]$. First note that $\left(\frac{\beta_{1}}{\beta_{0}}\right)^{0} = 1 \in [0, 1+ C_\beta]$, so the case $i = 0$ is dealt with. Suppose in the following that $i \geq 1$. (\ref{eq:C N fast converging}) implies that, in particular,
	\begin{equation}\label{eq:weak N fast convergence}
		|\beta - \beta_i| \leq \frac{\min\{1,C_\beta\}}{eNi}\cdot
	\end{equation}
	Then,
	\begin{align}
		\left(\frac{\beta_{i+1}}{\beta_{i}}\right)^{Ni} &= \left(1 + \frac{\beta_{i+1} - \beta_i }{\beta_{i}}\right)^{Ni} \overset{(a)}{<}  \left(1 + |\beta - \beta_i|\right)^{Ni}  \overset{(b)}{\leq} 1 + eNi |\beta - \beta_i| \overset{(\ref{eq:weak N fast convergence})}{\leq} 1 + C_\beta,
	\end{align}
	where (a) is by $\beta_i > 1$ and $\beta_{i+1} \leq \beta$, and (b) follows from the study of the sign of $(1+t)^n - (1 + ent)$ for $x \in [0,1]$ and $n \in \N$. This concludes the proof of $\mathcal Z_N(\beta) \subset \mathcal W_N(\beta)$.
\end{proof}
We now establish explicit conditions on $\Lambda_i$ so that $\betaf$ converges $N$-fast towards $\beta$.

\begin{lemma}\label{lem:condition on L for beta C N converging}
	Let $\beta \in (1,2)$, $N,L > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$. Suppose that 
	\begin{equation}\label{eq:condition on L}
		\tag{\text{$\mathcal L_1$}}
		L \geq 1 -\log_2\left(\min\{1,C_\beta\} (1-\log_2(\beta)^2)\right).
	\end{equation}
	Then, $\betaf$ is nondecreasing and converges $N$-fast towards $\beta$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2)$, $N,L > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$. $\betaf$ is obviously nondecreasing. Moreover,
	\begin{equation}
		|\beta - \beta_i| = |\beta - 1 - \delta_2(\gf_2(\betaun)_{\Lambda_{i}})| \leq \frac{1}{2^{\Lambda_{i}}}.
	\end{equation}
	We will prove that
	\begin{equation} \label{eq:condition lambda i for C N fast}
		\frac{1}{2^{\Lambda_{i}}} \leq \frac{\min\{1,C_\beta\}}{e\beta^{Ni}N^2i^2}, \ \text{for all} \ i \in \N_0,
	\end{equation}
	which will alow us to conclude that $\betaf$ converges $N$-fast. 
	\begin{align}
		\frac{1}{2^{\Lambda_{i}}} = \frac{1}{2^{Ni+L}} &\overset{(\ref{eq:condition on L})}{\leq} \frac{1}{2^{Ni} 2^{1 - \log_2(\min\{1,C_\beta\}(1-\log_2(\beta)^2))}}\\ 
		&= \frac{\min\{1,C_\beta\} (1-\log_2(\beta))^2}{2\times2^{Ni}eN}\\
		&= \frac{eN^2(1-\log_2(\beta))^2\beta^{Ni}i^2}{2\times 2^{Ni}}\frac{\min\{1,C_\beta\}}{\beta^{Ni}eN^2i^2}\cdot
	\end{align}
	The function $f : t \mapsto \frac{\beta^{Nt}t^2}{2^{Nt}}$ attains its maximum in $t_0 = \frac{2\ln(2)}{N(1-\log_2(\beta))}$, of a value of
	\begin{equation}
		f(t_0) = \frac{4\ln(2)^2}{2^{2\ln(2)} N^2 (1-\log_2(\beta))^2}.
	\end{equation}
	Therefore,
	\begin{align}
			\frac{1}{2^{\Lambda_{i}}} &\leq \frac{e \times 4\ln(2)^2}{2 \times 2^{2\ln(2)}}\frac{\min\{1,C_\beta\}}{\beta^{Ni}eN^2i^2}\cdot
	\end{align}
	The proof is concluded by remarking that $\frac{e \times 4\ln(2)^2}{2 \times 2^{2\ln(2)}} \simeq 0.999 \leq 1$.
	% (\ref{eq:condition lambda i for C N fast}) is equivalent to
	% \begin{equation}
	% 	Ni + L = \Lambda_i \geq Ni \log_2(\beta) + 2 \log_2(i) + \log_2(eN^2) - \log_2(\min\{1,C_\beta\}), \ \text{for all} \ i \in \N_0,
	% \end{equation}
	% which holds if
	% \begin{equation}
	% 	L \geq \max_{i\in\N_0} \left\{ Ni(\log_2(\beta) - 1) + 2\log_2(i)\right\} - \log_2(C_\beta) .
	% \end{equation}
	% The function $f : t \mapsto Nt (\log_2(\beta) - 1) + 2 \log_2(t)$ 
\end{proof}
\noindent We further establish explicit conditions on $\Lambda_i$ so that $\betaf \in A_\beta^\omega$.
\begin{lemma}\label{lem:condition on L for beta in A beta}
	Let $\beta \in (1,2)$, $N,L > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$. Suppose that 
	\begin{equation}\label{eq:condition on L 2}
		\tag{\text{$\mathcal L_2$}}
		L \geq - \log_2\left(\frac{9}{10}(\beta-1)\right).
	\end{equation}
	Then, $\betaf \in A_\beta^\omega$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2)$, $N,L > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$.  Suppose that (\ref{eq:condition on L 2}) holds. Note that $\betaf$ is nondecreasing and satisfies $\beta_i \leq \beta$ for all $i \in \N_0$. Then, we only have to prove that $\beta_0 \geq \lowbeta$. Then,
	\begin{align}
		\beta_0 = 1 + \delta_2(\gf_2(\betaun)_{\Lambda_0}) &\geq 1 + \beta - 1 - 2^{-L} \geq \beta - 2^{\log_2\left(\frac{9}{10}(\beta-1)\right)} = 1 + \frac{\beta-1}{10} = \lowbeta . 
	\end{align}
\end{proof}

We finally conclude with concrete conditions on both the $\Sigma_i$ and $\Lambda_i$ so that the dynamical system is well-defined.

% \begin{theorem}
% 	Let $\beta \in (1,2)$, $N,L,C > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$. Suppose that (\ref{eq:condition on L}) holds and that $C \in J_\beta$. Then, 
% 	\begin{equation}
% 		\beta_{i+1}^{Ni}\left(\delta_{\beta_i}(\xf_{1:i}) - \delta_{\beta_{i+1}}(\xf_{1:i})\right) \in J_{\beta_{i+1}}, \ \text{for all} \ i \in \N_0.
% 	\end{equation}
% \end{theorem}
% \begin{proof}
% 	Let $\beta \in (1,2)$, $N,L,C > 0$, and define $\Lambda_i := Ni + L$ for all $i \in \N_0$, and define $\betaf = \beta_0\beta_1\ldots$ by $\beta_i := 1 + \delta_2(\gf_2(\betaun)_{\Lambda_i})$ for all $i \in \N_0$. Suppose that (\ref{eq:condition on L}) holds and that $C \in J_\beta$. Since (\ref{eq:condition on L}), by Lemma \ref{lem:condition on L for beta C N converging} $\betaf$ is nondecreasing and converges $(C,N)$-fast. By Lemma \ref{lem:beta C N converging implies bounded error}, we deduce that 
% 	\begin{equation}
% 		0 \leq \beta_{i+1}^{Ni}\left(\delta_{\beta_i}(\xf_{1:i}) - \delta_{\beta_{i+1}}(\xf_{1:i})\right)\leq C.
% 	\end{equation}
% 	Since $C \in J_\beta$, it follows that $\beta_{i+1}^{Ni}\left(\delta_{\beta_i}(\xf_{1:i}) - \delta_{\beta_{i+1}}(\xf_{1:i})\right) \in J_\beta$. We conclude the proof by noticing that $J_\beta = \cap_{i \in \N_0} J_{\beta_{i+1}}$.
% \end{proof}

% As a conclusion of this section, we derive the following statement.
\begin{theorem}\label{thm:final conditions P1 P2}
	Let $s \in [0,1]$, $\beta \in (1,2)$, and
	\begin{equation}\label{eq:final value parameters beta r 1}\tag{\text{$\mathcal{P}_1$}}
		\begin{array}{rl}
			N &:= \left\lceil\log_{\lowbeta}(2) + \log_{\lowbeta}\left( \frac{2- {\lowbeta}}{2 - \beta} \right)\right\rceil,\\
			L &:= \left\lceil 1-\log_2\left(\frac{9}{10}\min\{1,C_\beta\}(\beta-1) (1-\log_2(\beta)^2)\right)\right\rceil\\
			\Lambda_i &:= Ni + L, \ \text{for all} \ i \in \N_0. 
		\end{array}
	\end{equation}
	We then define $\betaf = \beta_0\beta_1\ldots \in A_\beta$ according to (\ref{eq:beta i to generate beta expansion beta r}), $\Sigma_0 =0$, and
	\begin{equation}\label{eq:final value parameters beta r 2}\tag{\text{$\mathcal{P}_2$}}
		\Sigma_i := \lceil Ni\log_2(\beta_{i+1})\rceil - \left\lfloor \log_2\left(C_\beta\right) \right\rfloor, \ \text{for all} \ i \in \N.
	\end{equation}
	Finally, let $\ssf = s_0s_1\ldots$ be defined according to (\ref{eq:s i to generate beta expansion beta r}). Then, $(\ssf,\betaf) \in \dom \EE_N$.
\end{theorem}
\begin{proof}
	Let $\beta,s,N,L,\Lambda_i,\betaf, \Sigma_i$ and $\ssf$ be defined as above. We prove that $\betaf \in \mathcal U_N(\beta)$ and $\ssf \in K_\beta^\omega$, which allows to conclude by Lemma \ref{eq:J beta is in dom E beta N beta r}. We first show that $\betaf \in \mathcal U_N(\beta)$. Note that $L$ satisfies both (\ref{eq:condition on L}) and (\ref{eq:condition on L 2}), hence by Lemmata \ref{lem:condition on L for beta C N converging} and \ref{lem:condition on L for beta in A beta}, $\betaf \in A^\omega_\beta \cap \mathcal Z_N(\beta)$, which by Lemma \ref{lem:beta C N converging implies bounded error} implies $\betaf \subset A^\omega_\beta \cap \mathcal V_N(\beta)\cap \mathcal W_N(\beta)= \mathcal U_N(\beta)$. Now, show that $\ssf \in K_\beta^\omega$. Let $i \in \N_0$.
	\begin{align}
		s_i = \frac{\beta_{i+1}^{Ni}}{2^{\Sigma_i}} \delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) \overset{(\ref{eq:final value parameters beta r 2})}{\leq} C_\beta \delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) \overset{(a)}{\leq} C_\beta,
	\end{align}
	where (a) follows from $\delta_2(\cdot) \leq 1$. Hence, $s_i \in [0,C_\beta] = K_\beta$. Lemma \ref{eq:J beta is in dom E beta N beta r} yields $(\ssf, \betaf) \in K_\beta \times \UU_N(\beta) \subset \dom \EE_N(\beta)$.
\end{proof}

We now formally establish that the dynamical system generates a $\beta$-expansion.

\subsection{\texorpdfstring{The dynamical system produces a valid $\beta$-expansion}{}}


In this section, we show that for $\beta \in (1,2)$ and $s \in [0,1]$, if we define $N$, $L$ and $(\Lambda_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 1}), $\betaf = \beta_0\beta_1\ldots$ according to (\ref{eq:beta i to generate beta expansion beta r}), $(\Sigma_i)_{i \in \N_0}$  and (\ref{eq:final value parameters beta r 2}),  and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion beta r}), then $\EE_N(\ssf, \betaf)$ is a $\beta$-expansion of $s$.

\begin{theorem}\label{thm:convergence rational dynamical system to beta expansion beta r}
	Let $\beta \in (1,2)$ and $s \in [0,1]$. Define $N$, $L$ and $(\Lambda_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 1}), $\betaf = \beta_0\beta_1\ldots$ according to (\ref{eq:beta i to generate beta expansion beta r}), $(\Sigma_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 2}),  and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion beta r}). Then,
	\begin{equation}
		\EE_N(\ssf,\betaf) \in \Sigma_\beta(s).
	\end{equation}
\end{theorem}
\begin{proof}
	Let $\beta \in (1,2)$ and $s \in [0,1]$. Define $N$, $L$ and $(\Lambda_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 1}), $\betaf = \beta_0\beta_1\ldots$ according to (\ref{eq:beta i to generate beta expansion beta r}), $(\Sigma_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 2}),  and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion beta r}). By Theorem \ref{thm:convergence rational dynamical system to beta expansion beta r}, $\EE_N(\ssf,\betaf)$ is well-defined. To prove that $\EE_N(\ssf,\betaf) \in \Sigma_\beta(s)$, by (\ref{eq:definition beta expansion}) we need to show that $\delta_\beta(\EE_N(\ssf,\betaf)) = s$. We let 
	\begin{align}
		x^{(n)} &:= \EE_N(s_0s_1\ldots s_n,\beta_0\beta_1\ldots \beta_n), \ \text{for} \ n \in \N,\\
		\xf &= \EE_N(\ssf,\betaf),
	\end{align}
	and we successively show 
	\begin{equation}\label{eq:prefixes of d theta converge to d theta beta r}
		\limi{n} \delta_\beta\left(x^{(n)}\right) = \delta_\beta(\xf),
	\end{equation}
	\begin{equation}\label{eq:delta beta and delta beta n converge}
		\limi{n} \delta_\beta\left(x^{(n)}\right) = \limi{n} \delta_{\beta_n}\left(x^{(n)}\right),
	\end{equation}
	and
	\begin{equation}\label{eq:prefixes of d theta converge to s beta r}
		\limi{n} \delta_{\beta_n}\left(x^{(n)}\right) = s,
	\end{equation}
	which combination leads to $\delta_\beta(\xf) = s$. We start by proving (\ref{eq:prefixes of d theta converge to d theta}). Let $n \in \N$. Note that
	\begin{align}
		\xf_{1:Nn} &\overset{(\ref{eq:inferring chunks of greedy expansion from R i E beta i})}{=} \left[\coprod_{i=0}^{\infty} d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right)\right]_{1:Nn}\\
		&= \coprod_{i=0}^{n-1} d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right)\\
		&\overset{(\ref{eq:inferring prefix of chunks of greedy expansion from R i E beta i})}{=} \delta_\beta\left(x^{(n)}\right).\label{eq:d theta prefix is a prefix of d theta beta r}
	\end{align}
	It follows that
	\begin{align}
		\delta_\beta(\xf) &= \delta_\beta(\xf_{1:Nn} \xf_{Nn+1:\infty})\\
		&\osetlem{\ref{lem:factorisation of beta expansion through concatenation two}}{=} \delta_\beta(\xf_{1:Nn}) + \beta^{-Nn} \delta_\beta(\xf_{Nn+1:\infty})\\
		&\overset{(a)}{\in} \delta_\beta(\xf_{1:Nn}) + \beta^{-Nn} I_\beta\\
		&\overset{(\ref{eq:d theta prefix is a prefix of d theta beta r})}{=} \delta_\beta\left(x^{(n)}\right)  + \beta^{-Nn}I_\beta,
	\end{align}
	where (a) is by $\delta_\beta(\yf) \in I_\beta$, for all $\yf \in \{0,1\}^\omega$. Hence, 
	\begin{equation}
		0 \leq \limi{n} \left(\delta_\beta(\xf) - \delta_\beta\left(x^{(n)}\right)\right) \leq \limi{n} \frac{\beta^{-Nn}}{\beta-1} = 0,
	\end{equation}
	yielding (\ref{eq:prefixes of d theta converge to d theta beta r}). We now move to the proof of (\ref{eq:delta beta and delta beta n converge}). Let $n \in \N$.
	\begin{align}
		\left|\delta_{\beta}\left(x^{(n)}\right) - \delta_{\beta_n}\left(x^{(n)}\right)\right| & \leq \sum_{i=1}^{Nn} x^{(n)}_i |\beta^{-i} - \beta_n^{-i}|\\
		& \overset{(a)}{\leq} \sum_{i=1}^{Nn} x^{(n)}_i i |\beta - \beta_n|\\
		& \leq \frac{Nn(Nn+1)}{2} |\beta - \beta_n|\\
		& \leq N^2n^2 |\beta - \beta_n|\\
		& \overset{(b)}{\leq} \frac{C_\beta}{\beta_n^{Nn}} \underset{n \to \infty}{\to} 0,
	\end{align}
	where (a) follows froms the arguments exposed just after (\ref{eq:weak eq bounding delta beta variations}) and (b) is a consequence of $\betaf \in \mathcal V'_N(\beta)$.
	
	We finally prove (\ref{eq:prefixes of d theta converge to s beta r}). Fix $n \in \N$ The dynamical system has been defined so that (\ref{eq:s i to generate beta expansion beta r}) holds, then
	\begin{equation}
		R_i \overset{(\ref{eq:R i definition beta r})}{=} \beta_{i+1}^{Ni}\left(\delta_2(\gf_2(s)_{1:\Sigma_{i}}) - \delta_{\beta_{i}}(\xf_{1:Ni})\right).
	\end{equation}
	As (\ref{eq:final value parameters beta r 1}) and (\ref{eq:final value parameters beta r 2}) hold, then by Theorem (\ref{thm:final conditions P1 P2}) $(\ssf, \betaf) \in \dom \EE_N$, i.e.,
	\begin{equation}R_n + s_n + \varepsilon_N(X_n, \beta_{n+1}, \beta_n, n) \in I_\beta.\end{equation}
	In particular, $0 \leq R_n \leq \frac{1}{\beta-1}$.
	\begin{equation}
		0 \leq \frac{R_i}{\beta^{Ni}} \overset{(\ref{eq:R i definition})}{=} \delta_2(\gf_2(s)_{\Sigma_i:\Sigma_{i+1}}) - \delta_\beta(x^{(n)})  \overset{(\ref{eq:R i definition})}{=} \frac{R_i}{\beta_n^{Ni}} \leq \frac{1}{(\beta-1) \beta_n^{Ni}} \overset{(a)}{\leq} \frac{1}{(\beta-1) \lowbeta^{Ni}}\underset{n \to \infty}{\to} 0,
	\end{equation}
	where (a) follows from $\betaf \in A_\beta^\omega$. Therefore,
	\begin{equation}
		\limi{n} \delta_{\beta_n}(x^{(n)}) = \limi{n} \delta_2(\gf_2(s)_{\Sigma_i:\Sigma_{i+1}}) = s.
	\end{equation}
	This ends the proof.
	% \allowdisplaybreaks
	% \begin{align}
		
	% 	\frac{R_n}{\beta_{n+1}} = 
	% \end{align}
	% \begin{align}
	% 	\delta_\beta(\EE_N(s_0s_1\ldots s_n,\beta_0\beta_1\ldots \beta_n)) &\overset{(\ref{eq:inferring prefix of chunks of greedy expansion from R i E beta i})}{=} \delta_\beta\left(\coprod_{i=0}^{n-1} d_{\beta_{i+1}}^N\left(R_i +  s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right)\right)\\
	% 	&\osetlem{\ref{lem:factorisation of beta expansion through concatenation}}{=}\sum_{i=0}^{n-1} \beta^{-Ni}\delta_\beta\left( d_{\beta_{i+1}}^N\left(R_i + s_i + \varepsilon_N(X_i, \beta_i, \beta_{i+1} , i)\right)\right)\\
	% 	&\overset{(\ref{eq:definition multiple digit map})}{=}\sum_{i=0}^{n-1} \beta^{-Ni}\delta_\beta\left(\gf_\beta\left(R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}} s_i\right)_{1:N}\right)\\
	% 	&\overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left( R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}} s_i - \frac{1}{\beta^N}G^N_\beta\left(R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}} s_i\right) \right)\\
	% 	&\overset{(\ref{eq:greedy map chunks as dynamical system})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left(R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}}s_i - \frac{1}{\beta^N}R_{i+1}\right)\\
	% 	&\overset{(\ref{eq:s i to generate beta expansion})}{=} \sum_{i=0}^{n-1} \beta^{-Ni} \left(R_i + \frac{\beta^{Ni}}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \frac{1}{\beta^N}R_{i+1}\right)\\
	% 	&= \sum_{i=0}^{n-1} \beta^{-Ni} R_i + \sum_{i=0}^{n-1} \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}}) - \sum_{i=0}^{n-1} \beta^{-N(i+1)} R_{i+1}\\
	% 	&= R_0 - \beta^{Nn}R_n + \sum_{i=0}^{n-1} \frac{1}{2^{\Sigma_i}}\delta_2(\gf_2(s)_{\Sigma_i+1:\Sigma_{i+1}})\\
	% 	&\osetlem{\ref{lem:factorisation of beta expansion through concatenation}}{=} R_0 - \beta^{Nn}R_n + \delta_2(\gf_2(s)_{1:\Sigma_n}). \label{eq:intermediate equation delta beta x n}
	% \end{align}
	% From the definition of $E_\beta^N$, $R_0 = 0$. Moreover, as $(N, (\Sigma_i)_{i \in \N})$ satisfy (\ref{eq:final value parameters}), by (\ref{eq:R i is in 0 1}) one has $R_n \in [0,1]$. Therefore,
	% \begin{equation}
	% 	0 \geq \limi{n} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) - \delta_2(\gf_2(s)_{1:\Sigma_n}) \geq \limi{n} -\beta^{-Nn} = 0.
	% \end{equation}
	% As $\limi{n} \Sigma_n = \infty$, we then have
	% \begin{equation}
	% 	\limi{n} \delta_\beta(E_\beta^N(s_0s_1 \ldots s_{n-1})) = \limi{n}\delta_2(\gf_2(s)_{1:\Sigma_n}) = s, 
	% \end{equation}
	% thereby finishing the proof.
\end{proof}

% \begin{theorem}\label{thm:generalized convergence rational dynamical system to beta expansion}
% 	Let $\beta \in (1,2)$, and suppose that $\DD_\beta$ satisfies $(\mathbf{H}')$. Then,
% 	\begin{equation}
% 		\xf_\beta(s) \in \Sigma_\beta(s), \ \forall s \in [0,1].
% 	\end{equation}
% \end{theorem}
% \begin{proof}
% 	Let $\beta \in (1,2)$, suppose that $\DD_\beta$ satisfies $(\mathbf{H}')$, and let $s \in [0,1]$. To prove that $\xf_\beta(s) \in \Sigma_\beta(s)$, we need to show that $\delta_\beta(\xf_\beta(s)) = s$. Consider the sequence $(X_n)_{n \in \N}$ generated by $\DD_\beta(s)$. $\limi{n} X_n = \xf_\beta(s)$, where the limit is defined according to distance $d$ introduced in Definition \ref{def:metric on discrete sequences}. As by Lemma \ref{lem:delta beta is continuous}, $\delta_\beta$ is continuous as a mapping from $\left(\{0,1\}^\omega, d\right)$ to $(\R,|\cdot|)$, $\left(\delta_\beta(X_n)\right)_{\N_2}$ therefore converges to $\delta_\beta(\xf_\beta(s))$. Further, fix $n \in \N$ and note that
% 	\begin{align}
% 		|\delta_\beta(X_n) - \delta_{q_{n-1}}(X_n)| &= \left|\sum_{i=1}^{|X_n|} [X_n]_i \left(\beta^{-i} - q_{n-1}^{-i}\right)\right| \leq \left|\sum_{i=1}^{|X_n|} \left(\beta^{-i} - q_{n-1}^{-i}\right)\right| \\
% 		&\leq \left|\sum_{i=1}^{\infty} \left(\beta^{-i} - q_{n-1}^{-i}\right)\right| \leq \frac{1}{\beta-1} - \frac{1}{q_{n-1}-1} \underset{n \to \infty}{\to} 0.
% 	\end{align}
% 	Then, $\limi{n}\delta_\beta(X_n) = \limi{n} \delta_{q_{n-1}}(X_n)$. We now show that  $\left(\delta_{q_{n-1}}(X_n)\right)_{\N_2}$ converges to $s$, which allows us to conclude that $ s = \limi{n}\delta_\beta(X_n) = \delta_\beta(\xf_\beta(s))$, and hence that $\delta_\beta(\xf_\beta(s)) \in \Sigma_\beta(s)$. Fix $n \in \N$. First note that $X_{n+1} = X_n  \gf_{q_{n}}(R'_{n})_{1: N}$. By repeating this argument, one has 
% 	\begin{equation}\label{eq:generalized B_n as concatenation of greedy Z i}
% 		X_{n+1} = X_0  \coprod_{i=0}^{n} \gf_{q_i}(R'_i)_{1: N} = \coprod_{i=0}^{n} \gf_{q_i}(R'_i)_{1: N}.
% 	\end{equation}
% 	Further, for $i \in \{1,\ldots,n\}$,
% 	\begin{align}
% 		R_{i+1} - q_i^N R_i &= q_i^N(1-\xi_i^N)R_i + \xi_i^N G_{q_i}^N(R'_i) - q_i^N R_i\\
% 		&\overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=}q_i^N(1-\xi_i^N)R_i + \xi_i^N q_i^N\left(R'_i - \delta_{q_i}(\gf_{q_i}(R'_i))_{1: N}\right)- q_i^N R_i\\
% 		&=  \xi_i^N q_i^N\left(\frac{q_i^{Ni}}{2^{\Sigma_i}} S'_{i} + q_{i}^{Ni} \left(\delta_{q_{i-1}}(X_i) - \delta_{q_i}(X_i)\right) - \delta_{q_i}(\gf_{q_i}(R'_i))_{1: N}\right)\\
% 		&=  \chi_i^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}(X_i) - q_i^{-Ni}\delta_{q_i}(\gf_{q_i}(R'_i))_{1: N}\right)\\
% 		&\overset{(\ref{eq:generalized B_n as concatenation of greedy Z i})}{=}  \chi_i^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}\left(\coprod_{j=0}^{i-1} \gf_{q_j}(R'_j)_{1: N}\right)  - q_i^{-Ni}\delta_{q_i}(\gf_{q_i}(R'_i))_{1: N}\right)\nonumber \\
% 		&\overset{\ref{lem:factorisation of beta expansion through concatenation}}{=}  \chi_i^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}\left(\coprod_{j=0}^i \gf_{q_j}(R'_j)_{1: N}\right)\right)\\
% 		&\overset{(\ref{eq:generalized B_n as concatenation of greedy Z i})}{=}  \chi_i^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}\left(X_{i+1}\right)\right), \label{eq:X i + 1 X i relationship}
% 	\end{align}
% and
% \begin{align}
% 	R_1 - q_0^NR_0 &= q_0^N(1-\xi_0^N)R_0 + \xi_0^N G_{q_0}^N(R'_0) - q_0^N R_0 = \xi_0^N G_{q_0}^N(R'_0) = G_{q_0}^N(R'_0) \\
% 	& \overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=} q_0^N\left( R'_0 - \delta_{q_0}(\gf_{q_0}(R'_0)_{1: N}) \right) \overset{(\ref{eq:generalized B_n as concatenation of greedy Z i})}{=} q_0^N\left( \frac{1}{2^{\Sigma_0}}S'_0 - \delta_{q_0}(B_1) \right)\label{eq:X 1 X 0 relationship}.
% \end{align}
% Moreover, note that
% \begin{align}
% 	& \sum_{i=0}^n \left( \prod_{j=i+1}^{n+1} q_j^N\right) \left(R_{i+1} - q_i^N R_i \right) =\sum_{i=0}^n \left(R_{i+1}\prod_{j=i+1}^{n+1} q_j^N - R_i\prod_{j=i}^{n+1} q_j^N \right)\\
% 	&=\sum_{i=1}^{n+1} \left(R_i\prod_{j=i}^{n+1} q_j^N\right) -\sum_{i=0}^n \left( R_i\prod_{j=i}^{n+1} q_j^N \right) 
% 	= R_{n+1} \prod_{j=n+1}^{n+1} q_j^N - R_0 \prod_{j=0}^{n+1} q_j^N\\
% 	&=R_{n+1}q_{n+1}^N - R_0 \chi_{n+1} \overset{(\ref{eq:definition of the generalized dynamical system})}{=} R_{n+1}q_{n+1}^N. \label{eq:relation X n + 1 with sum of X n s}
% \end{align}
% Then, 
% \begin{align}
% 	R_{n+1} &\overset{(\ref{eq:relation X n + 1 with sum of X n s})}{=} \frac{1}{q_{n+1}^N} \sum_{i=0}^n \left( \prod_{j=i+1}^{n+1} q_j^N\right) \left(R_{i+1} - q_i^N R_i \right) =  \sum_{i=0}^n \left( \prod_{j=i+1}^{n} q_j^N\right) \left(R_{i+1} - q_i^N R_i \right)\\
% 	& = \sum_{i=1}^n \left( \prod_{j=i+1}^{n} q_j^N\right) \left(R_{i+1} - q_i^N R_i \right) + \left( \prod_{j=1}^{n} q_j^N\right) \left(R_{1} - q_0^N R_0 \right)\\
% 	&\overset{(\ref{eq:X i + 1 X i relationship})}{=} \sum_{i=1}^n \left( \prod_{j=i+1}^{n} q_j^N\right) \chi_i^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}\left(X_{i+1}\right)\right) + \left( \prod_{j=1}^{n} q_j^N\right) \left(R_{1} - q_0^N R_0 \right) \nonumber\\
% 	&\overset{(\ref{eq:X 1 X 0 relationship})}{=} \sum_{i=1}^n  \chi_n^N \left(\frac{1}{2^{\Sigma_i}} S'_{i} + \delta_{q_{i-1}}(X_i) - \delta_{q_i}\left(X_{i+1}\right)\right) + \left( \prod_{j=1}^{n} q_j^N\right) q_0^N\left( \frac{1}{2^{\Sigma_0}}S'_0 - \delta_{q_0}(B_1)\right) \nonumber\\
% 	&= \chi_n^N  \left(\sum_{i=0}^n \frac{1}{2^{\Sigma_i}} S'_{i} + \sum_{i=1}^n \delta_{q_{i-1}}(X_i) - \sum_{i=0}^n\delta_{q_i}\left(X_{i+1}\right)\right)\\
% 	&= \chi_n^N  \left(\sum_{i=0}^n \frac{1}{2^{\Sigma_i}} S'_{i} - \delta_{q_n}\left(X_{n+1}\right)\right). \label{eq:intermediate result X n +1}
% \end{align}
% Remark that, for $i \in \{0,\ldots,n\}$,
% \begin{align}
% 	S'_{i} &=  S_{i} - G_2^{M_{i}}(S_{i}) \overset{(\ref{eq:n iterations of greedy map is same as reading the first n bits})}{=} \delta_2\left(\gf_2(S_{i})\right) 
% 	= \delta_2\left(\gf_2\left(G_2^{\Sigma_{i}}(S_0) \right)_{1: M_{i}}\right)\\
% 	&\overset{(\ref{eq:n iterations of greedy map is same as shifting n bits})}{=} \delta_2\left(\gf_2(S_0)_{\Sigma_{i}+1:\Sigma_{i}+M_{i}}\right)
% 	 =\delta_2\left(\gf_2(S_0)_{\Sigma_{i}+1:\Sigma_{i+1}}\right)
% 	 \overset{(\ref{eq:definition of the dynamical system})}{=}\delta_2\left(\gf_2(s)_{\Sigma_{i}+1:\Sigma_{i+1}}\right). \label{eq:generalized W_i equivalent to delta of greedy binary}
% \end{align} 
% Therefore,
% \begin{equation}
% 	\sum_{i=0}^n \frac{1}{2^{\Sigma_i}} S'_i \overset{(\ref{eq:generalized W_i equivalent to delta of greedy binary})}{=} \sum_{i=0}^n \frac{1}{2^{\Sigma_i}} \delta_2\left(\gf_2(s)_{\Sigma_{i}+1:\Sigma_{i+1}}\right) \overset{\ref{lem:factorisation of beta expansion through concatenation}}{=} \delta_2\left(\gf_2(s)_{1: \Sigma_{i+1}}\right).\label{eq:sum W i to make x}
% \end{equation}
% Finally,
% \begin{equation}
% 	\delta_{q_n}\left(X_{n+1}\right) \overset{(\ref{eq:intermediate result X n +1})}{=} \sum_{i=0}^n \frac{1}{2^{\Sigma_i}} S'_{i}  - \frac{1}{\chi_n^N}X_{n+1} \overset{(\ref{eq:sum W i to make x})}{=} \delta_2\left(\gf_2(s)_{1: \Sigma_{n+1}}\right) - \frac{1}{\chi_n^N}R_{n+1}.
% \end{equation}
% As $\DD_\beta$ satisfies $(\mathbf{H}')$, by Lemma \ref{lem:generalized d beta is well defined}, $0 \leq R_{n+1} \leq \frac{2}{\beta}$, and as $\chi_n \overset{(\ref{eq:def of chi i})} \geq q_0^n$, then $0 \leq \limi{n} \frac{R_{n+1}}{\chi_n} \leq \limi{n} \frac{2}{\beta q_0^n} = 0$. Moreover, as $\DD_\beta$ satisfies $(\mathbf{H}')$, then also $\Sigma_n \geq N n \log_2(\beta)$, so $\limi{n}\Sigma_n = \infty$. We deduce that
% \begin{equation}
% 	\limi{n} \delta_{q_n}(X_{n+1}) = \limi{n} \delta_2\left(\gf_2(s)_{1: \Sigma_{n+1}}\right) - \limi{n}\frac{1}{\chi_n^N}R_{n+1} = \delta_2(\gf_2(s)) = s,
% \end{equation}
% thereby finishing the proof.
% \end{proof}

\subsection{\texorpdfstring{Algorithmic complexity of the $\beta$-expansion generated by the dynamical system}{}}

We have established that for $\beta \in (1,2)$, and $s \in [0,1]$, $\EE_N(\ssf,\betaf)$ constitutes a valid $\beta$-expansion, assuming that (\ref{eq:final value parameters beta r 1}), (\ref{eq:beta i to generate beta expansion beta r}), (\ref{eq:final value parameters beta r 2}) and  (\ref{eq:s i to generate beta expansion beta r}) hold. In this paragraph, we conclude the proof of (\ref{eq:inequality to be proven}), which establishes a relationship between the algorithmic complexity of the respective prefixes of $\EE_N(\ssf,\betaf)$ and $\gf_2(s)$, respectively.

\begin{lemma}\label{lem:weak inequality binary beta expansion Kolmogorov rational beta r}
	Let $\beta \in (1,2)$ and $s \in [0,1]$. Define $N$, $L$ and $(\Lambda_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 1}), $\betaf = \beta_0\beta_1\ldots$ according to (\ref{eq:beta i to generate beta expansion beta r}), $(\Sigma_i)_{i \in \N_0}$  and (\ref{eq:final value parameters beta r 2}),  and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion beta r}). Then, there exists $\xf \in \Sigma_\beta(s)$, such that
	\begin{equation}
		K[\xf|N n] \leq K[\gf_2(s)|\Sigma_n] +F(K[\gf_2(\betaun)|Nn+L])+ c_\beta, \ \ \text{for all} \ n \in \N.
	\end{equation}
	where $F : t \mapsto t + 2\log_2(t)$, and $c_\beta > 0$ depends only on $\beta$.
\end{lemma}
\begin{proof}
	Let $\beta \in (1,2)$, $s \in [0,1]$. Define $N$, $L$ and $(\Lambda_i)_{i \in \N_0}$ according to (\ref{eq:final value parameters beta r 1}), $\betaf = \beta_0\beta_1\ldots$ according to (\ref{eq:beta i to generate beta expansion beta r}), $(\Sigma_i)_{i \in \N_0}$  and (\ref{eq:final value parameters beta r 2}),  and $\ssf = s_0s_1\ldots $ according to (\ref{eq:s i to generate beta expansion beta r}). By Theorem \ref{thm:convergence rational dynamical system to beta expansion beta r}, $\EE_N(s_0s_1\ldots s_{n-1})$ is an $Nn$-prefix of $\EE_N(\ssf) \in \Sigma_\beta(s)$, for $n \in \N$. The equations of (\ref{eq:R i X i + 1 definition of E N}) can be run on a digital computer because they require only finite precision, and hence $\EE_N$ can be cast into the effective algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$ summarized in Algorithm \ref{alg:conversion binary expansion to beta expansion beta r}. Note that $\varphi(\langle\gf_2(s)_{1:\Sigma_n}, \gf_2(\beta-1)_{1:Nn+L}\rangle) = \EE_N(s_0s_1\ldots s_{n-1},\beta_0\beta_1\ldots \beta_{n-1}) = \EE_N(\ssf,\betaf)_{1:Nn}$, for $n \in \N$. Therefore, by Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity} there exists $c_\varphi > 0$ such that
	\begin{align}
		K[\xf|N n] &\leq K[\langle\gf_2(s)_{1:\Sigma_n}, \gf_2(\beta-1)_{1:Nn+L}\rangle] + c_\varphi,\\
		&\overset{(\ref{eq:simple inequality on pairing of sequences})}{\leq}  K[\gf_2(s)|\Sigma_n] +F(K[\gf_2(\beta-1)|Nn+L]) + C_+ + c_\varphi,
	\end{align}
	for all $n \in \N$. $\varphi$ depends only on $\EE_N$, which itself depends only on $\beta$ as $N = \lceil \log_{\betaprox}(2) \rceil$. Hence, $c_\varphi$ depends only on $\beta$.
	\begin{algorithm}[H]
		\caption{$\beta$-expansion from a binary expansion}\label{alg:conversion binary expansion to beta expansion beta r}
		\begin{algorithmic}[1]
			\Require $n \in \N$, $x \in \{0,1\}^\ast$, $y \in \{0,1\}^\ast$
			\State Check that $|y| \geq Nn+L$, if not raise an error.
			\For{$i = 0, \ldots, n$}
			\State $\beta_i \gets 1 + \sum_{j=1}^{Ni+L} y_{j} 2^{-j}$
			\EndFor
			\For{$i = 0, \ldots, n$}
			\State $\Sigma_i \gets \lceil Ni\log_2(\beta_{i+1}) \rceil - \lfloor \log_2(C_\beta) \rfloor$
			\EndFor
			\State Check that $|x| \geq \Sigma_n$, if not raise an error.
			\For{$i = 0, \ldots, n-1$}
			\State $s_i \gets \frac{\beta_{i+1}^{Ni}}{2^{\Sigma_i}}\delta_2(x_{\Sigma_i+1:\Sigma_{i+1}})$
			\EndFor
			\State \Return $\EE_N(s_0s_1\ldots s_{n-1}, \beta_0\beta_1)$
		\end{algorithmic}
	\end{algorithm}
\end{proof}

% Having established that $\beta \in (1,2)$ and $s \in [0,1]$, $\xf_\beta(s)$ constitutes a valid $\beta$-expansion under condition $(\mathbf{H}')$, it remains to show that the algorithmic complexity of the prefixes of $\xf_\beta(s)$ can inferred from the algorithmic complexity of the prefixes of the greedy expansion $\gf_2(s)$. In this section, we say that $\DD_\beta$ is effective if there exists an effective algorithm which can, on input $n$, output $\Sigma_n$, for all $n \in \N$. We start with an intermediate result, and then conclude on the final result as a corollary. 
% \begin{theorem}\label{lem:generalized weak inequality binary beta expansion Kolmogorov}
% 	Let $\beta \in (1,2)$, $s \in [0,1]$, $\DD_\beta = (L,N,(\Sigma_n))$ be effective, and suppose that there exists $\delta \in \left(0, \frac{2 -\beta}{\beta}\right) \cap \Q$ such that $\DD_\beta$ satisfies \textnormal{(\ref{eq:H delta prime})}. Then, there exists $c > 0$, depending only on $\DD_\beta$, such that
% 	\begin{equation}
% 		K[\xf_\beta(s)|N n] \leq K[\gf_2(s)|\Sigma_n] +F(K[\gf_2(\beta-1)|Nn+L]) + c, \ \ \text{for all} \ n \in \N,
% 	\end{equation}
% 	where $F : t \mapsto t + 2\log_2(t)$.
% \end{theorem}
% \begin{proof}
% 	Let $\beta \in (1,2)$, $s \in [0,1]$, $\DD_\beta = (L,N,(\Sigma_n))$ be effective and suppose that there exists $\delta \in \left(0, \frac{2 -\beta}{\beta}\right) \cap \Q$ such that $\DD_\beta$ satisfies (\ref{eq:H delta prime}).
	
% 	We design an effective algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$ such that
% \begin{equation}
% 	\xf_\beta(s)_{1: N n} = \varphi(\langle \gf_2(s)_{1: \Sigma_n}, \gf_2(\beta-1)_{1: Nn+L}  \rangle), \ \ \text{for all} \ n \in \N.
% \end{equation}
% Let $n \in \N$. Concretely, on input $\langle \gf_2(\beta-1)_{1: Nn+L},  \gf_2(s)_{1: \Sigma_n} \rangle$, $\varphi$ first separates $\gf_2(\beta-1)_{1:  Nn+L}$ from $\gf_2(x)_{1: \Sigma_n}$. $\varphi$ then computes $n$ through $n = \frac{Nn+L - L}{N}$. Further, $\varphi$ uses $\gf_2(\beta-1)_{1:  Nn+L}$ to compute $q_0,\ldots, q_n$, as per $q_i = \delta_2(\gf_2(\beta-1)_{1:  Ni+L})$.
% $\varphi$ then computes $n$ iterations of the dynamical system $\DD_\beta$ on input $s$, and records the successive values $R'_0, \ldots, R'_n$. Finally, it generates $\xf_\beta(s)_{1: N n}$ through the equation
% \begin{equation}
% 	\xf_\beta(s)_{1: N n} :=  \coprod_{i=0}^{n-1} \gf_{q_i}(R'_i)_{1: N}.
% \end{equation}
% Note that as $q_k \in \Q$ for all $0\leq k \leq n$, all the variables involved in the evolution of $\DD_\beta$ are rational numbers, and all the operations underlying this evolution can be run on a digital computer, as they can be reduced to additions and multiplications only. So $\varphi$ is indeed an effective algorithm. By Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists $C > 0$, depending only on $\varphi$, and a fortirori only on $\DD_\beta$, such that, for all $n \in \N$,
% \begin{align}
% 	K[\xf_\beta(x)|N n] &\leq K[\langle \gf_2(s)_{1: \Sigma_n}, \gf_2(\beta-1)_{1: Nn+L}  \rangle] + C\\
% 	&\overset{(\ref{eq:simple inequality on pairing of sequences})}{\leq} K[\gf_2(s)_{1: \Sigma_n}] + F(K[\gf_2(\beta-1)_{1:  Nn+L}]) + C_+ + C.
% \end{align}
% We set $c := C + C_+$, thereby finishing the proof.
% \end{proof}

\begin{corollary}
	Let $\beta \in (1,2)$, $s \in [0,1]$. Then, there exists $\xf\in \Sigma_\beta(s)$ such that
	\begin{equation}\label{eq:generalized algorithmic complexity of beta expansion lower than binary expansion}
		K[\xf|n] \leq  K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] + F(K[\gf_2(\betaun)|n]) + c_\beta, \ \text{for all} \ n \in \N.
	\end{equation}
	where $F : t \mapsto t + 2\log_2(t)$, and $c_\beta > 0$ depends only on $\beta$.
\end{corollary}
\begin{proof}
	\textit{To appear.}
\end{proof}
% \begin{proof}
% 	Let $\beta \in (1,2)$, $s \in [0,1]$. Let $\delta \in (0,\frac{2-\beta}{\beta}) \cap \Q$, and let $\DD_\beta$ such that 
% 	\begin{equation}\label{eq:final conditions of N and Sigma, H delta prime in proof}
% 			\tag{$\mathbf{H}_\delta'$}
% 			\begin{split}
% 			L &= \left\lceil\max\left\{C_{N,\beta} -\log_2\left(\frac{C_{\delta,\beta}}{N^2\beta^N}\right) , \frac{1}{2} \log_2\left(-\log\left(C'_{N,\delta,\beta}\right)\right)\right\}\right\rceil\\
% 			N &= -  \left\lceil\log_\beta\left( \frac{\delta}{2- \beta} \right)\right\rceil, \\
% 			\Sigma_{i} &= \left\lceil Ni\log_2(q_i) - \log_2\left(C_{\delta,\beta} \right)\right\rceil , \ \forall i \in \N.
% 			\end{split}
% 	\end{equation}
% 	Obviously, $\DD_\beta$ satisfies (\ref{eq:H delta prime}), where $\delta \in \Q$, so by Lemma \ref{lem:generalized weak inequality binary beta expansion Kolmogorov}, there exists $c>0$ such that
% 	\begin{equation}
% 		K[\xf_\beta(s)|N n] \leq K[\gf_2(s)|\Sigma_n] +F(K[\gf_2(\beta-1)|Nn+L]) + c, \ \ \text{for all} \ n \in \N.
% 	\end{equation}
% 	Note that by (\ref{eq:simple inequality on concatenation of sequences}), there exists $C>0$ such that
% \begin{equation}\label{eq:generalized before ultimate equation proof kolmogorov}
% 	K[\xf_\beta(s)|n]  \leq K[\gf_2(s)|\Sigma_{\lfloor n/N\rfloor}]+F(K[\gf_2(\beta-1)|N\lfloor n/N\rfloor+L]) + c + C, \ \ \text{for all} \ n \in \N.
% \end{equation}
% Further, remark that
% \begin{equation}
% 	n - N + L \leq N\lfloor n/N\rfloor+L \leq n + L, \ \text{ for all } \ n \in \N.
% \end{equation}
% Then, by Lemma \ref{lem:kolmogorov complexity of closed sequences}, there exists $C' > 0$ such that
% \begin{align}
% 	& K[\gf_2(\beta-1)|N\lfloor n/N\rfloor+L] \leq K[\gf_2(\beta-1)|n] + C', \ \ \text{for all} \ n \in \N,\\
% 	\overset{(a)}{\Rightarrow} & F(K[\gf_2(\beta-1)|N\lfloor n/N\rfloor+L]) \leq F(K[\gf_2(\beta-1)|n]) + C', \ \ \text{for all} \ n \in \N,
% \end{align}
% where (a) is a consequence of $F$ being increasing and subadditive. It follows that 
% \begin{equation}\label{eq:generalized before ultimate equation proof kolmogorov 2}
% 	K[\xf_\beta(s)|n]  \leq K[\gf_2(s)|\Sigma_{\lfloor n/N\rfloor}]+F(K[\gf_2(\beta-1)|n]) + C' + c + C, \ \ \text{for all} \ n \in \N.
% \end{equation}
% Finally, note that
% \begin{align}
% 	\left|\lceil n \log_2(\beta)\rceil - \Sigma_{\lfloor n/N\rfloor}\right| &\leq 2 + \left|n \log_2(\beta) - N\left\lfloor \frac{n}{N}\right\rfloor\log_2(q_{\lfloor n/N \rfloor}) - \log_2\left(C_{\delta,\beta} \right)\right|\\
% 	&\leq 2 + N + \left|n \log_2(\beta) - n\log_2(q_{\lfloor n/N \rfloor}) - \log_2\left(C_{\delta,\beta} \right)\right|\\
% 	&\overset{(a)}{\leq} 2 + N + \left|n\frac{1}{\log(2)} (\beta - q_{\lfloor n/N \rfloor}) - \log_2\left(C_{\delta,\beta} \right)\right|\\
% 	&\leq 2 + N + \left|n\frac{1}{\log(2)} 2^{-L-N{\lfloor n/N \rfloor}} - \log_2\left(C_{\delta,\beta} \right)\right|\\
% 	&\leq 2 + N + \left|\frac{2}{\log(2)} 2^{-L}n2^{-n} - \log_2\left(C_{\delta,\beta} \right)\right|\\
% 	&\overset{(b)}{\leq} 2 + N + \left|\frac{2}{\log(2)} 2^{-L} - \log_2\left(C_{\delta,\beta} \right)\right| =: M\\
% \end{align}
% where (a) follows from $\log : [1, \infty] \to \R$ being 1-Lipschitz, and (b) is by $n2^{-n}\leq 1$ for all $n \in \N$. Then, $\left|\lceil n \log_2(\beta)\rceil - \Sigma_{\lfloor n/N\rfloor}\right| \leq M$ for all $n \in \N$, so by Lemma by Lemma \ref{lem:kolmogorov complexity of closed sequences}, there exists $C'' > 0$ such that
% \begin{equation}\label{eq:generalized before ultimate equation proof kolmogorov 3}
% 	K[\gf_2(s)|\Sigma_{\lfloor n/N\rfloor}] \leq K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] + C'', \ \text{for all} \ n \in \N.
% \end{equation}
% By combining (\ref{eq:before ultimate equation proof kolmogorov}) and (\ref{eq:before ultimate equation proof kolmogorov 2}), one has
% \begin{equation}
% \nonumber
% 	K[\xf_\beta(s)|n] \leq K[\gf_2(s)|\lceil n \log_2(\beta) \rceil] + F(K[\gf_2(\beta-1)|n]) + C'' + C' + C + c, \ \text{for all} \ n \in \N,
% \end{equation}
% thereby finishing the proof by letting $\hat \xf_\beta := \xf_\beta (s)$.
% \end{proof}

We have proven that for every $s \in [0,1]$, there exists a $\beta$-expansion of $s$ which algorithmic complexity of prefixes is upper bounded a very simple manner by a relation involving the algorithmic complexity of the prefixes of the binary expansion of $s$ and the binary expansion of $\beta$, for every $\beta \in (1,2)$. A direct consequence is the following corollary, when $\beta$ is a computable number.
\begin{corollary}
	Let $\beta \in (1,2)$ be a computable number, and $s \in [0,1]$. Then, there exists $\xf \in \Sigma_\beta(s)$ such that
	\begin{equation}\label{eq:computable algorithmic complexity of beta expansion lower than binary expansion}
		K[\xf|n] \leq  K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] + c_\beta, \ \text{for all} \ n \in \N,
	\end{equation}
	where $c_\beta > 0$ depends only on $\beta$.
\end{corollary}
\noindent This achieves the proof of the main Theorem.


==> subfiles/study_all_expansions_kolmogorov_complexity.tex <==
% !TEX root = main.tex

$\N_2 := \{2,3,4,\ldots\}$

\begin{definition}[Multivalued function]\label{def:multivalued_function}
    Let $X,Y$ be two sets. We write $f: X \rightrightarrows Y$ to denote the fact that $f$ is a multivalued function from $X$ to $Y$, i.e., for each $x \in X$, $f(x)$ is a subset of $Y$.
\end{definition}

\begin{definition}[Surrounding multivalued function]\label{def:surrounding_multivalued_function}
    Let $X,Y$ be two sets. We say that a multivalued function $f: X \rightrightarrows Y$ surrounds a function $g : X \to Y$, if
    \begin{equation}
        g(x) \in f(x), \ \forall x \in X.
    \end{equation}
\end{definition}

\begin{doubtfulsec}
\begin{definition}\label{def:finite_multivalued_function}
    Let $X,Y$ be two sets. We say that a multivalued function $f : X \rightrightarrows Y$ is finite if $f(x)$ is a finite set, for every $x \in X$.
\end{definition}
\end{doubtfulsec}

\begin{definition}[Computable multivalued function]\label{def:computable_multivalued_function}
    Let $f: \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ be a finite multivalued function. We say that $f$ is computable if there exists a computable function $g : \{0,1\}^\ast \to \{0,1\}^\ast$ such that 
    \begin{equation}
        g(x) = \coprod_{y \in f(x)} \bar{y}. 
    \end{equation}
\end{definition}

\begin{definition}[Ambiguous multivalued function]\label{def:ambiguous_multivalued_function}
    Let $f: \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ be a multivalued function and $\psi : \N \to \N$. We say that $f$ is $\psi$-ambiguous if 
    \begin{equation}
        \# f(x) \leq \psi(|x|), \ \forall x \in \{0,1\}^\ast.
    \end{equation}
\end{definition}

\begin{theorem}[Ambiguity and complexity]
    Let $f: \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ be a $\psi$-ambiguous computable multivalued function and $x \in \{0,1\}^\ast$. For all $y \in f(x)$,
    \begin{equation}
        K(y) \leq K(x) + \log_2 \psi(|x|) + \constw{x}.
    \end{equation}
\end{theorem}

\begin{theorem}[Multifunctions and complexity]
    Let $f: \{0,1\}^\ast \rightrightarrows \{0,1\}^\ast$ be a computable multivalued function and $x \in \{0,1\}^\ast$. For all $y \in f(x)$,
    \begin{equation}
        K(y) \leq K(x) + \log_2 \#f(x) + \constw{x}.
    \end{equation}
\end{theorem}

\begin{corollary}
    Let $g : \{0,1\}^\ast \to \{0,1\}^\ast$, and suppose that $g$ is surrounded by a $\psi$-ambiguous computable multivalued function. Then, for all $x \in \{0,1\}^\ast$,
    \begin{equation}
        K(g(x)) \leq K(x) + \log_2 \psi(|x|) + \constw{x}.
    \end{equation}
\end{corollary}

\pdfcomment{Stay TO THE POINT: do not make too many undirect definitions}

\begin{definition}
    Let $b_1,b_2 \in (1,\infty)$. The base conversion multifunction is denoted by 
    \begin{equation}
        \begin{array}{cclc}
            C_{b_1,b_2} : & \subseteq \N^\N & \rightrightarrows & \N^\N\\
            & x & \mapsto &  \Sigma_{b_2}(\delta_{b_1}(x)).
        \end{array}
    \end{equation}
\end{definition}

\begin{definition}  Let $b_1,b_2 \in (1,\infty)$, and $f : \N \to \N$ be a nondecreasing function. The prefix base conversion multifunction is denoted by 
    \begin{equation}
        \begin{array}{cclc}
            c_{b_1,b_2}(\cdot | f) : & \subseteq \N^\ast & \rightrightarrows & \N^\ast\\
            & x & \mapsto &  \Sigma_{b_2}(\delta_{b_1}(x\N^\N)) \cap \N^{\leq f(|x|)}.
        \end{array}
    \end{equation}
    We also define $N_{b_1,b_2}(\cdot|f) : \subseteq \N^\ast \to \N$ as
    \begin{equation}
        N_{b_1,b_2}(x|f) := \#c_{b_1,b_2}(x| f), \ \forall x \in \dom(c_{b_1,b_2}(\cdot|f)).
    \end{equation}
\end{definition}

\begin{theorem}
    Let $b_1 \in (1,\infty)$ and $b_2 \in \N_2$. Then,
    \begin{equation}
       \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil \leq N_{b_1,b_2}(x|f) \leq \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil +1.
    \end{equation}
\end{theorem}

\begin{theorem}
    Let $b_1,b_2 \in (1,\infty)$, then 
    \begin{equation}
        \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil \leq N_{b_1,b_2}(x|f) \leq 2^{|x|}.
     \end{equation}
\end{theorem}


I can prove that Garsia numbers have an absolutely continuous Bernoulli convolution with bounded density $\Leftarrow$ we can conclude on there maximal Kolmogorov of their $\beta$-expansion. 





==> subfiles/study_greedy_expansion_kolmogorov_complexity.tex <==
% !TEX root = main.tex


$\N_2 := \{2,3,4,\ldots\}$

POLICY: We treat the case $\base \in (1,2)$.

Story justification for the upcoming definition. It is not possible to convert a prefix of the greedy expansion of a number $s$ to the prefix of the greedy expansion but in another base, except if some very specific conditions hold between the bases (established for integer bases in Brattka, to be investigated for nonintegers). Make the example with base $2$ and $3$. Hence given a prefix the greedy expansion of a number $s$ in base $\base_1$, we can only hope to build a function that gives a list of possible prefixes in base $\base_2$, i.e., such a function takes one element as input, and outputs a set of elements. This exactly falls into the framework introduced previously. as a multivalued function in Brattka

For $\base \in (1,\infty)$, we define the base $\base$ evaluation function $ \ev_\base : \subseteq \N^\N \to [0,1]$ as
\begin{equation}
    \ev_\base(\xf) = \sum_{i=1}^\infty \xf_i \base^{-i},
\end{equation}
for all $\xf \in \dom( \ev_\base) := \digs$. We set $\eval :=  \ev_\base|^{[0,1]}$, i.e., $\eval$ is the evaluation function restricted to those elements of $\digs$ that are a $\base$-expansion of a real number in $[0,1]$. For $f : X \to \N^\N$, $A \subseteq X$ and $n \in \N$, we define
\begin{equation}
    f(A)|_n := \{ \xf|_n : \xf \in f(A)\}.
\end{equation}

\begin{definition} Let $\base_1,\base_2 \in (1,\infty)$, and $f : \N \to \N$ be a nondecreasing function. The prefix base conversion multifunction is denoted by $c_{\base_1,\base_2}(\cdot | f)$ the function that, upon presentation of a prefix of length $n \in \N$ of any expansion in base $\base_1$ as input, outputs the possible corresponding prefixes of length $f(n)$ of the greedy expansion in base $\base_2$. In mathematical symbols, this translates to
    \begin{equation}
        \begin{array}{cclc}
            c_{\base_1,\base_2}(\cdot | f) : & \subseteq \N^\ast & \rightrightarrows & \N^\ast\\
            & x & \mapsto &  \left[\grd[\base_2]\circ\eval[\base_1](x\N^\N)\right]_{1:f(|x|)}.
        \end{array}
    \end{equation}
    Note that $\dom (c_{\base_1,\base_2}(\cdot|f))$ is the set of finite words in $\N^\ast$ that are a prefix of some element of $\dom \eval[\base_1]$.
    % We also define $N_{b_1,b_2}(\cdot|f) : \subseteq \N^\ast \to \N$ as
    % \begin{equation}
    %     N_{b_1,b_2}(x|f) := \#c_{b_1,b_2}(x| f), \ \forall x \in \dom(c_{b_1,b_2}(\cdot|f)).
    % \end{equation}
\end{definition}

We now want to establish an upper bound on $\card (c_{\base_1,\base_2}(x|f))$, for $x \in \dom (c_{\base_1,\base_2}(\cdot|f))$.  Note that $\eval[\base_1](x \N^\N)$ is an interval, of length at most $\frac{\base_1^{-|x|}}{\base_1-1}$. We next establish an upper bound on $\# \grd[\base_2](I)_{1:n}$, where $I \subset [0,1]$ is a closed interval and $n \in \N$. The upper bound will notably depend on $|I|$.

\begin{theorem}
    Let $\base \in (1,\infty)$ and $I \subseteq [0,1]$ be a closed interval. Then,
    \begin{equation}\label{eq:bound number canonical sequences interval}
        \# \gf_b(I)_{1:n} \leq |I|\frac{\lceil b \rceil}{b-1} b^{n} + (\lceil b \rceil -b)\sum_{i=1}^n (G_b^i(\inf I) - G_b^i(\sup I)).
    \end{equation}
\end{theorem}
\begin{proof}
    Let $b \in (1,2)$, $I \subseteq [0,1]$ be a closed interval, and $n \in \N$. First note that for $A,B \subseteq [0,1]$ disjoint,
    \begin{equation}\label{eq:greedy expansions union}
        \gf_b(A )_{1:n} \subseteq \gf_b(A \cup B)_{1:n} \subseteq \gf_b(A)_{1:n} \cup \gf_b(B)_{1:n}.
    \end{equation}
    Next, let us define 
    \begin{align}
        s_n &:= \delta_b(\gf_b(\inf I)_{1:n}),\\
        t_n &:= \delta_b(\gf_b(\sup I)_{1:n}),
    \end{align}
    and $I_n := [s_n,t_n]$. We prove that (a) $\gf_b(I_n)_{1:n} = \gf_b(I)_{1:n}$ and (b) that (\ref{eq:bound number canonical sequences interval}) holds for $I_n$.
    \begin{enumerate}[label=(\alph*)]
        \item Note that $I_n \cup (s_n, \sup I] = [s_n, \inf I) \cup I = [s_n, \sup I]$. We show that $\gf_b([s_n, \sup I])_{1:n} =\gf_b(I_n)_{1:n}$ and that $\gf_b([s_n, \sup I])_{1:n} =\gf_b(I)_{1:n}$, yielding $\gf_b(I_n)_{1:n} =\gf_b(I)_{1:n}$. 
        
        First note that, by \ref{eq:greedy expansions union}, we have
        \begin{align}
            \gf_b(I)_{1:n} &\subseteq \gf_b([s_n, \sup I])_{1:n} \subseteq \gf_b(I)_{1:n} \cup \gf_b([s_n,\inf I))_{1:n}.\\
            \gf_b(I_n)_{1:n} &\subseteq \gf_b([s_n, \sup I])_{1:n} \subseteq \gf_b(I_n)_{1:n} \cup \gf_b((t_n,\sup I])_{1:n}.
        \end{align}
        We prove that (i) $\gf_b([s_n,\inf I))_{1:n} \subseteq \gf_b(I)_{1:n}$ and (ii) $\gf_b(I_n)_{1:n} \subseteq \gf_b((t_n,\sup I])_{1:n}$.

        \begin{enumerate}[label=(\roman*)]
            \item Suppose that there exists $x \in \gf_b((s_n, \inf I])_{1:n} \backslash \ \gf_b(I)_{1:n}$. Note that, in particular, $x \neq \gf_b(s_n)$. As $\inf I - \delta_b(x) < \inf I - s_n \leq b^{-n}$, $x$ is the $n$-prefix of a $b$-expansion of $\inf I$. But since $\delta_b(x) > s_n = \delta_b(\gf_b(\inf I)_{1:n})$, then by Lemma \ref{GR-lem:greedy expansion preserves order}, $x >_L \gf_b(\inf I)_{1:n}$, which is a contradiction.
            \item Suppose that there exists $x \in \gf_b((t_n, \sup I])_{1:n} \backslash \ \gf_b(I_n)_{1:n}$. Note that, in particular, $x \neq \gf_b(s_n)$. As $\sup I - \delta_b(x) < \sup I - t_n \leq b^{-n}$, $x$ is the $n$-prefix of a $b$-expansion of $\sup I$. But since $\delta_b(x) > t_n = \delta_b(\gf_b(\sup I)_{1:n})$, then by Lemma \ref{GR-lem:greedy expansion preserves order}, $x >_L \gf_b(\sup I)_{1:n}$, which is a contradiction.
        \end{enumerate}
        \item We find a law on the number of elements of $\gf_b(I_n)_{1:n}$ based on $\gf_b(I_n)_{1:n-1}$.
    \end{enumerate}
\end{proof}

% \begin{lemma}(Greedy expansion preserves order)\label{lem:greedy expansion preserves order}
%     Let $s,t \in [0,1]$, and $b \in (1,\infty)$. Then,
%     \begin{equation}
%         s < t \iff \gf_b(s) <_L \gf_b(t).
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     Let $s,t \in [0,1]$, and $b \in (1,\infty)$.
%     First note that, obviously, $s \neq t \iff \gf_b(s) \neq \gf_b(t)$. It then suffices to prove that (a) $s < t \Rightarrow \gf_b(s) \leq_L \gf_b(t)$ and (b) $\gf_b(s) <_L \gf_b(t) \Rightarrow s\leq t$. Note that (b) is simply the contraposition of (a), so we only need to prove (a). We proceed by contradiction: suppose that $s < t$, and that $\gf_b(s) >_L \gf_b(t)$, i.e., that there exists $i \in \N$ such that $\gf_b(s)_j = \gf_b(t)_j$, for all $j < i$, and $\gf_b(s)_i > \gf_b(t)_i$. Hence,
%     \begin{equation}
%         t > s \geq \sum_{j=1}^i \gf_b(s)_jb^{-j} > \sum_{j=1}^i \gf_b(t)_jb^{-j} \geq t - b^{-i}.
%     \end{equation}
%     So $\gf_b(s)_{1:i}$ is the $i$-prefix of some $b$-expansion $\xf$ of $t$, satisfying $\xf >_L \gf_b(t)$, which is a contradiction.
% \end{proof}
% \begin{lemma}(Greedy expansion is stable by appending $0$)
%     Let $n \in \N$, and $b \in (1,\infty)$. Then,
%     \begin{equation}
%         \gf_b(\delta_b(x)) = x0^\infty, \ \forall x \in \gf_b([0,1])_{1:n}.
%     \end{equation}
% \end{lemma}
% \begin{proof}
%     Let $n \in \N$, $b \in (1,\infty)$ and $x \in \gf_b([0,1])_{1:n}$. Suppose that $\yf := \gf_b(\delta_b(x)) >_L x0^\infty =: \xf$, i.e., that there exists $i \in \N$ such that $\yf_j = \xf_j$, for all $j < i$, and $1 = \yf_i > \xf_i = 0$.
%     \begin{enumerate}[label=(\alph*)]
%         \item Suppose that $i > n$. Then,
%         \begin{align}
%             \delta_b(\yf) &\leq \delta_b(\yf_{1:n}) + b^{-i}\yf_i\\
%             &= \delta_b(x) + b^{-i}\yf_i\\
%             &> \delta_b(x),
%         \end{align}
%         so $\yf$ is not a $b$-expansion of $\delta_b(x)$, which is a contradiction.
%         \item Suppose that $i \leq n$. Since $x \in \gf_b([0,1])_{1:n}$, there exists $s \in [0,1]$ such that $\gf_b(s)_{1:n} = x$. Note that
%         \begin{equation}
%             s = \delta_b(\gf_b(s)) \geq \delta_b(\gf_b(s)_{1:n}) = \delta_b(x),
%         \end{equation} 
%         and that
%         \begin{equation}
%             \gf_b(s)_{1:i-1} = x_{1:i-1} = \yf_{1:i-1} = \gf_b(\delta_b(x))_{1:i-1}.
%         \end{equation}
%         Hence,
%         \begin{align}
%             G_b^{i-1}(s) &= b^{i-1}(s - \delta_b(\gf_b(s)_{i-1}))\\
%                          &\geq b^{i-1}(\delta_b(x) - \delta_b(\gf_b(s)_{i-1}))\\
%                          &= b^{i-1}(\delta_b(x) - \delta_b(\gf_b(\delta_b(x))_{i-1}))\\
%                          &= G_b^{i-1}(\delta_b(x)).
%         \end{align}
%         However, $\gf_b(\delta_b(x))_i = \yf_i = 1$, so $G_b^{i-1}(\delta_b(x)) > 1/b$, and $\gf_b(s)_i = x_i = 0$, so $G_b^{i-1}(s) \leq 1/b$, which yields a contradiction.
%     \end{enumerate}
% \end{proof}
% \noindent We denote 
% 
% A variant of the right term of the above equation is
% \begin{align}
%     \sum_{i=1}^n (G_b^i(\inf I) - G_b^i(\sup I)) &= \sum_{i=1}^n \left[\beta^i (\inf I - s_i) - \beta^i(\sup I - t_i) \right]\\
%     &= \sum_{i=1}^n \beta^i (t_i - s_i - |I|) 
% \end{align}

\begin{theorem}
    Let $b_1 \in (1,\infty)$ and $b_2 \in \N_2$. Then,
    \begin{equation}
       \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil \leq N_{b_1,b_2}(x|f) \leq \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil +1.
    \end{equation}
\end{theorem}

\begin{theorem}
    Let $b_1,b_2 \in (1,\infty)$, then 
    \begin{equation}
        \left\lceil\frac{(b_2-1)b_2^{f(|x|)}}{b_1^{{|x|}}}\right\rceil \leq N_{b_1,b_2}(x|f) \leq 2^{|x|}.
     \end{equation}
\end{theorem}

1. I can prove that Garsia numbers have an absolutely continuous Bernoulli convolution with bounded density $\Leftarrow$ we can conclude on the maximal Kolmogorov of their $\beta$-expansions. \cite{baker2014approximation}

2. I can prove that for a constructive set of $\beta$ of Hausdorff dimension 1, the greedy $\beta$-expansion has the same complexity as the binary expansion. \cite{schmerling1995symbolic} + \cite{fai2012lengths}

3. We can prove that for all $\beta$, almost all numbers have the same complexity in $\beta$-expansion and in binary expansion. I could, eventually, one day, make a statement about the complexity of the other numbers, but I am not going down this road. That. is. it. (That is work directly from my side)

% \ifthenelse{\equal{\jobname}{main}}{}{
%     \bibliographystyle{IEEEtranS}
%     \bibliography{biblio.bib}
% }


==> subfiles/technical_preliminaries.tex <==
% !TEX root = main.tex

\section{Technical preliminaries}
\label{sec:notations formal result}



In this section, we present preparatory material on $\beta$-expansions, and we split the proof of Theorem \ref{thm:informal equivalence kolmogorov complexity computable} in subcases dealt with in the remaining sections of the paper.
% \subsection{beta-expansions}
\subsection{\texorpdfstring{$\beta$-expansions}{-expansions} and dynamical maps}
\noindent Let $\beta \in (1,2]$. Following \cite{parry1960beta}, we say that $\xf \in \{0,1\}^\omega$ is a $\beta$-expansion of 
$s \in I_\beta := \ibet$ if
\begin{equation}\label{eq:definition beta expansion}
	s = \delta_\beta(\xf),
\end{equation}
where 
\begin{equation}\label{eq:definition of delta beta}
	\begin{array}{lccl}
		\delta_\beta : & \{0,1\}^\omega & \to & I_\beta\\
		& \xf & \mapsto & \displaystyle \sum_{i=1}^{\infty} \xf_i \beta^{-i}.
	\end{array}
\end{equation}
To see that $\delta_\beta$ indeed maps to $I_\beta$, note that $\delta_\beta(0^\infty) = 0$ and $\delta_\beta(1^\infty) = \frac{1}{\beta-1}$. For $x \in \{0,1\}^\ast$, we use the shorthand $\delta_\beta(x):= \sum_{i=1}^{|x|}x_i\beta^{-i}$ instead of the more cumbersome $\delta_\beta(x0^\infty)$. As already mentioned in Section \ref{sec:introduction}, there are, in general, multiple sequences $\xf \in \{0,1\}^\omega$ generating a given $s$ according to (\ref{eq:definition beta expansion}); we denote by $\Sigma_\beta(s) := \delta_\beta^{-1}(\{s\})$ the set of all $\beta$-expansions of $s \in I_\beta$. For instance, as explained in Section \ref{sec:introduction}, for $G = \frac{1 + \sqrt{5}}{2}$ we have $\Card{\Sigma_G(1)} = \infty$. Moreover, for each $\beta \in (1,G)$, the set of $\beta$-expansions for each $s \in I_\beta$ is uncountable, i.e., $\Card{\Sigma_\beta(s)} = 2^{\aleph_0}$ \cite[Theorem 3]{erdos1990characterization}. 

For $s \in I_\beta$, we define the greedy $\beta$-expansion $\gf_\beta(s)$ to be the lexicographically maximal element of $\Sigma_\beta(s)$. As mentioned in Section \ref{sec:introduction}, Algorithm \ref{alg:greedy algorithm beta expansion} computes $\gf_\beta(s)$. We now show that this algorithm can be interpreted as a dynamical system. This interpretation will be crucial to the proof of Theorem \ref{thm:informal equivalence kolmogorov complexity computable}. Inspection of Algorithm \ref{alg:greedy algorithm beta expansion} reveals that the variable ``$r$'' realizes the greedy map $G_\beta : I_\beta \to I_\beta$ \cite[Section 1, p.2]{baker2015induced}:
\begin{equation}\label{eq:greedy map}
	G_\beta (r) = \begin{cases}
		\beta r, \ \ \text{if} \ r < \frac{1}{\beta},\\
		\beta r - 1, \ \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} \ \ \forall r \in I_\beta.
\end{equation}
Further, the variable ``$b$'' in Algorithm \ref{alg:greedy algorithm beta expansion} realizes the following function
\begin{equation}
	d_{\beta}  (r) = \begin{cases}
		0, \ \ \text{if} \ r < \frac{1}{\beta},\\
		1, \ \ \text{if} \ r \geq \frac{1}{\beta}, 
	\end{cases} \ \ \forall r \in I_\beta,
\end{equation}
that generates one bit of the greedy $\beta$-expansion of $r$. Note that $G_\beta(r) = \beta r - d_\beta(r)$, for $r \in I_\beta$. Finally, the greedy $\beta$-expansion is shown to be given by
\begin{equation}\label{eq:greedy beta exp as digit + iterative map}
	\gf_\beta(s) = \coprod_{i=0}^\infty d_{\beta}\left(G_\beta^{i}(s)\right).
\end{equation}
Remark that $G_\beta$ can be interpreted as a bit-shifting and a bit-extraction device. Let $s \in [0,1]$ and denote its greedy $\beta$-expansion by $\xf$. Then, one has 
\begin{equation}
	G_\beta(s) = \beta s - d_\beta(s) = \beta \sum_{i=1}^\infty \xf_i \beta^{-i} - d_\beta(s) = \xf_1 + \sum_{i=2}^\infty \xf_i \beta^{-i+1} - \xf_1 = \sum_{i=1}^\infty \xf_{i+1} \beta^{-i},
\end{equation}
which shows that application of $G_\beta$ simply shifts the sequence $\xf$ by one position to the left. It now follows directly that iterating $G_\beta$ $n$ times effects a left-shift by $n$ positions according to 
\begin{equation}\label{eq:n iterations of greedy map is same as shifting n bits}
	G^n_\beta(s) = \sum_{i=1}^\infty \xf_{i+n} \beta^{-i}.
\end{equation}
Moreover, we can also interpret the greedy map as a bit-extraction device, namely by noting that
\begin{equation}\label{eq:n iterations of greedy map is same as reading the first n bits}
	s - \frac{1}{\beta^n} G^n_\beta(s) = \sum_{i=1}^\infty \xf_i \beta^{-i} - \frac{1}{\beta^n}\sum_{i=1}^\infty \xf_{i+n} \beta^{-i} = \sum_{i=1}^n\xf_i \beta^{-i} = \delta_\beta(\xf_{1: n}).
\end{equation}
We now note that the generation the successive prefixes of the greedy $\beta$-expansion can be cast into the following equation $(E_\Theta)$, depending on the parameter $\Theta = (\beta,R_0) \in (1,2) \times I_\beta$, that describes an iterative process $R_1,R_2,\ldots$, by
\begin{equation}\label{eq:greedy map as system of equations}
		R_{i+1} = \displaystyle G_\beta(R_i),
	\tag{$E_\Theta$}
\end{equation}
for $i \in \N_0$. Setting $R_0 = s \in I_\beta$, we recover
\begin{equation}\label{eq:greedy expansion from evolution of R i}
	\gf_\beta(s) \overset{(\ref{eq:greedy beta exp as digit + iterative map})}{=} \coprod_{i=0}^\infty d_{\beta}\left(R_i\right),
\end{equation}
hence the greedy $\beta$-expansion of $s$ is deduced from the variable $R_i$. The successive values taken by $R_i$ correspond to the evolution of a discrete dynamical system with no inputs. We can further transform the generation of the greedy $\beta$-expansion into a discrete dynamical system with one parameter $\beta \in (1,2)$, always starting on $R_0 = 0$, and presented with an input $\ssf = s_0s_1\ldots \in I_\beta^\omega$, as follows. 
\begin{equation}\label{eq:greedy map as dynamical system}
	\begin{array}{rl}
		R_{i+1} &= \displaystyle G_\beta(R_i + s_i),
	\end{array}
	\tag{$E_{\beta}$}
\end{equation}
for $i \in \N_0$, with $R_0 = 0$. When presented with input $\ssf = s_0s_1 \in I_\beta^\omega$, $E_\beta$ is seen as a mapping $I_\beta^\ast \to \{0,1\}^\ast$ by $E_\beta(\epsilon) := \epsilon$ and
\begin{equation}\label{eq:inferring prefix of greedy expansion from R i E beta}
	E_\beta(s_0s_1\ldots s_{n-1}) := \coprod_{i=0}^{n-1} d_\beta(R_i + s_i), 
\end{equation}
for all $n \in \N$, and as a mapping $ I_\beta^\omega \to \{0,1\}^\omega$ through
\begin{equation}\label{eq:inferring greedy expansion from R i E beta}
	E_\beta(\ssf) := \coprod_{i=0}^{\infty} d_\beta(R_i + s_i).
\end{equation}

Note that by setting $s_0 = s \in I_\beta$ and $s_i = 0$ for $i \in \N$, $E_\beta(\ssf) = \gf_\beta(s)$. Finally, note that we can adapt (\ref{eq:greedy map as dynamical system}) so that it generates the greedy $\beta$-expansion by chunks. Let $N \in \N$, and consider 
\begin{equation}\label{eq:greedy map chunks as dynamical system} \tag{\text{$E^N_\beta$}}
	R_{i+1} = G_\beta^N(R_i + s_i).
\end{equation}
We also generalize the function $d_\beta$ to $d_\beta^N$ that generates $N$ bits of greedy $\beta$-expansion as
\begin{equation}\label{eq:definition multiple digit map}
	d_\beta^N(r) := \coprod_{i=0}^{N-1} d_{\beta}\left(G_\beta^{i}(s)\right) \overset{(\ref{eq:greedy expansion from evolution of R i})}{=} \gf_\beta(r)_{1:N}, \ \text{for} \ r \in I_\beta.
\end{equation}
Note that indeed, $d_\beta^1 = d_\beta$. When presented with input $\ssf = s_0s_1 \in  I_\beta^\omega$, we can see $E^N_\beta$ as a mapping $ I_\beta^\ast \to \{0,1\}^\ast$ by $E^N_\beta(\epsilon) := \epsilon$ and
\begin{equation}\label{eq:inferring prefix of chunks of greedy expansion from R i E beta}
	E^N_\beta(s_0s_1\ldots s_{n-1}) := \coprod_{i=0}^{n-1} d^N_\beta(R_i + s_i), 
\end{equation}
for all $n \in \N$, and as a mapping $I_\beta^\omega \to \{0,1\}^\omega$ through
\begin{equation}\label{eq:inferring chunks of greedy expansion from R i E beta}
	E^N_\beta(\ssf) := \coprod_{i=0}^{\infty} d^N_\beta(R_i + s_i).
\end{equation}
Again, setting $s_0 = s \in I_\beta$ and $s_i = 0$ for $i \in \N$ yields $E^N_\beta(\ssf) = \gf_\beta(s)$. Similar considerations apply to the lazy $\beta$-expansion, but we do not detail it as this is not needed for our proofs.
% One can also define the lazy $\ellf_\beta := \inf_L\left(\Sigma_\beta(s)\right)$. 
% Following \cite[Section 2]{dajani2002greedy} 
% the lazy $\beta${-expansion} can be generated as follows. Analogously to the greedy map $G_\beta$ above, we define the lazy map according to
%  $L_\beta : I_\beta \to I_\beta$ \cite[Section 1]{baker2015induced}:
% \begin{equation}
% 	L_\beta (r) = \begin{cases}
% 		\beta r, \ \ \text{if} \ r \leq \frac{1}{\beta(\beta-1)},\\
% 		\beta r - 1, \ \ \text{if} \ r > \frac{1}{\beta(\beta-1)}, 
% 	\end{cases} \ \ \forall r \in I_\beta.
% \end{equation}
% The bits of the lazy $\beta$-expansion are then computed by the following function
% \begin{equation}
% 	d_{\beta,lazy}  (r) = \begin{cases}
% 		0, \ \ \text{if} \ r \leq \frac{1}{\beta(\beta-1)},\\
% 		1, \ \ \text{if} \ r > \frac{1}{\beta(\beta-1)}, 
% 	\end{cases} \ \ \forall r \in I_\beta.
% \end{equation}
% Finally, the lazy $\beta$-expansion is shown to be given by
% \begin{equation}
% 	\ellf_\beta(s) = \coprod_{i=0}^\infty d_{\beta,lazy}\left(L_\beta^{i}(s)\right).
% \end{equation}



% \subsection{Algorithmic complexity}

% \subsection{Kolmogorov complexity of beta-expansions}
% \label{subsec:Kolmgorov complexity}


% We now proceed in establishing solid ground for the study of algorithmic complexity. Recall the notion of universal effective algorithm introduced in previous section. Following \cite[Definition 3.4]{calude2002information}\cite[Chapter 14.2]{cover1999elements}\cite[Definition 2.1.1]{li2008introduction}, the  algorithmic complexity of a binary sequence $x \in \{0,1\}^\ast$ with respect to a given universal effective algorithm $U : \{0,1\}^\ast \to \{0,1\}^\ast$ is
% \begin{equation}\label{eq:informal definition relative Kolmorogov complexity}
% 	K_U[x] := \min \{ \len u : u \in \{0,1\}^\ast, U(u) = x\}.
% \end{equation}
% Following \cite[Definition 3.4]{calude2002information}, we say that $x^\ast$ is the canonical program for $x$ with respect to $U$ if 
% \begin{equation}
% 	x^\ast := \min \left\{ u \in \{0,1\}^\ast : U(u) = x \right\},
% \end{equation}
% where the $\min$ is taken with respect to the quasi-lexicographical order. Note that $|x^\ast| = K_U[x]$.


%Definition (\ref{eq:informal definition relative Kolmorogov complexity}) is usually referred to as conditional algorithmic complexity, see \cite[Chapter 14.2]{cover1999elements}, where the qualifier ``conditional'' indicates knowledge of $|x|$. 

% Following \cite[Theorem 14.2.1]{cover1999elements}, we now show that the choice of $U$ is somewhat not important. 
% \begin{lemma}
% 	Let $V : \{0,1\}^\ast \to \{0,1\}^\ast$ be another universal effective algorithm. Then, there exists $c > 0$ such that for all $x \in \{0,1\}^\ast$,
% 	\begin{equation}
% 		\left| K_U[x] - K_V[x]\right| \leq c.
% 	\end{equation}
% \end{lemma}
% \begin{proof}
% 	As $U$ is a universal effective algorithm, there exists $p \in \{0,1\}^\ast$ such that 
% 	\begin{equation}
% 		U(\langle p, x \rangle) = V(x), \text{ for all } x \in \{0,1\}^\ast. 
% 	\end{equation}
% Let $x \in \{0,1\}^\ast$, and let $x^\ast \in \{0,1\}^\ast$ be the canonical program for $x$ with respect to $V$. Then, $U(\langle p, x^\ast\rangle) = V(x^\ast) = x$. It follows that $K_U[x] \leq |\langle p, x^\ast \rangle| \leq 2|p| + |x^\ast| + 1 = 2|p|+ 1+ K_V[x]$. We let $c_1 := 2|p| + 1$, and then $K_U[x] \leq K_V[x] + c_1$. Likewise, we can show that there is a constant $c_2 > 0$ such that $K_V[x] \leq K_U[x] + c_2$. The lemma follows by letting $c = \max(c_1,c_2)$.
% \end{proof}
% Then, the definition of algorithmic complexity relatively to a specific universal effective algorithm is invariant up to a positive additive constant. From now on, we fix a universal effective algorithm $\Uref$, and define the (absolute) algorithmic complexity of the binary sequences $x$ as
% \begin{equation}\label{eq:informal definition absolute Kolmorogov complexity}
% 	\begin{array}{lccl}
% 		K[\cdot] : & \{0,1\}^\ast & \to & \N\\ 
% 			& x &	\mapsto & K_{\Uref}[x].
% 	\end{array}
% \end{equation}

% In this paper, we are interested in comparing the algorithmic complexity of binary expansions and $\beta$-expansions. As the expansions are of infinite length and algorithmic complexity is defined for finite binary sequences only, we need an adequate extension of algorithmic complexity to infinitely long sequences. Specifically, following \cite[Definition 10.9]{balcazar2012structural}, we shall consider the algorithmic complexity of $n$-prefixes $\xf_{1: n}$ of such an infinite sequence $\xf$. For simplicity of notations, we shall write
% \begin{equation}
% 	K[\xf|n] := K[\xf_{1: n}], \ \text{ for all } \xf \in \{0,1\}^\omega, \ \text{ and all } n \in \N.
% \end{equation}
% The above definition allows to study the algorithmic complexity of $\beta$-expansions.



\subsection{\texorpdfstring{Algorithmic complexity of binary expansions}{}}

We are now ready to commence our investigation of the algorithmic complexity of $\beta$-expansions, specifically with an eye towards comparison with the behavior of the algorithmic complexity of binary expansions. 

% First, recall that binary expansions are essentially unique, concretely unique up to the 2-ambiguity property discussed in Section \ref{sec:introduction}. On the other hand, $\beta$-expansions are highly non-unique as exemplified in Section \ref{sec:introduction}. The goal of our analysis is to develop an understanding of how this nonuniqueness is reflected in terms of algorithmic complexity. 

We formalize the following statement from \cite[Section IV]{balcazar1997hierarchy}: ``In the cases where $\delta_2$ is not injective, [...]\hspace{0.5mm}the two inverse images [...]\hspace{0.5mm}have essentially (up to a small additive term) the same Kolmogorov complexity''. To our knowledge, the latter assertion is not made formal in the literature. This result allows to make a first simplification to the proof of Theorem \ref{thm:informal equivalence kolmogorov complexity computable}: the variable $\xf$ in (\ref{eq:equivalence kolmogorov complexity binary beta expansions}) can be chosen to be the greedy binary expansion, instead of working with either the greedy or the lazy expansion.
\begin{lemma}\label{lem:greedy and lazy expansion have same K complexity}
	There exists $c > 0$ such that, for every $s \in [0,1]$, the greedy binary expansion $\gf_2(s)$ and the lazy binary expansion $\ellf_2(s)$ satisfy 
\begin{equation}\label{eq:greedy and lazy binary expansions have same algorithmic complexity}
	\left|K[\gf_2(s)|n] - K[\ellf_2(s)|n]\right| \leq c, \ \forall n \in \N.
\end{equation}
\end{lemma}
\begin{proof}
As explained in Section \ref{sec:introduction}, the greedy and lazy binary expansion of a given real number $s \in [0,1]$ differ only when the greedy expansion ends with $0^\infty$; in this case, the lazy expansion ends with $1^\infty$. Such numbers $s$ are said to be ``dyadic''; the set of all dyadic numbers is denoted by $\D$. Now, for $s \notin \D$, one has $\ellf_2(s) = \gf_2(s)$ so that (\ref{eq:greedy and lazy binary expansions have same algorithmic complexity}) holds trivially. When $s \in \D$, the operations underlying (\ref{eq:greedy expansion ending with infinitetail of zeros})-(\ref{eq:lazy expansion ending with infinitetail of ones}), can be cast into an effective algorithm $\varphi$ summarized in Algorithm \ref{alg:generator of greedy expansion fixed input}, such that $\varphi(\gf_2(s)_{1: n}) = \ellf_2(s)_{1: n}$, for all $n \in \N$.
\begin{algorithm}
	\caption{Conversion from a greedy prefix to a lazy prefix}\label{alg:generator of greedy expansion fixed input}
	\begin{algorithmic}[1]
		\Require  $x \in \{0,1\}^\ast$
		\State Find the position $n$ of the last $1$ in $x$ 
		\State $x_n \gets 0$
		\For{$i = n+1, \ldots, |x|$}
		\State $x_i \gets 1$
		\EndFor
		\State \Return $x$
	\end{algorithmic}
	\end{algorithm}

Note that $\varphi$ essentially finds the last bit equal to $1$ of its input $x \in \{0,1\}^\ast$, switches it to $0$, and then switches all the following bits to $1$. Conversely, one can devise an effective algorithm $\psi$ that finds the last $0$ of its input $x \in \{0,1\}^\ast$, switches it to $1$, and then switches all the following bits to $0$. This last algorithm converts a lazy expansion into a greedy expansion, i.e. $\psi(\ellf_2(s)_{1: n}) = \gf_2(s)_{1: n}$ for all $s \in [0,1]$ and all $n \in \N$. By application of Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists two constants $c_\varphi,c_\psi > 0$ such that
\begin{equation}
	\begin{array}{l}
	K[\ellf_2(s) | n] \leq K[\gf_2(s)|n] + c_\varphi,\\
	K[\gf_2(s)|n] \leq K[\ellf_2(s)|n] + c_\psi,
	\end{array} \ \forall n \in \N, \ \text{and} \ \forall s \in \D.
\end{equation}
Setting $c := \max(c_\varphi, c_\psi)$ finishes the proof.
\end{proof}

Thanks to Lemma \ref{lem:greedy and lazy expansion have same K complexity}, Theorem \ref{thm:informal equivalence kolmogorov complexity computable} can be restated as follows. For all $s \in [0,1]$ and all computable $\beta \in (1,2]$, there exist $\xf \in \Sigma_\beta(s)$ and $c > 0$ such that
\begin{equation}\label{eq:equivalence algorithmic complexity beta expansion binary expansion}
	\left|K[\xf|n] - K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] \right| \leq c, \ \ \forall n \in \N.
\end{equation}
This result constitutes a vast extension of \cite[Theorem 3]{staiger2002kolmogorov}, which establishes an equivalent fact for $q$-ary expansions, where $q \in \N_2$.

\subsection{\texorpdfstring{Related work on $q$-ary expansions}{}}

Fix $q \in \N_2$. A $q$-ary expansion of a given $s \in [0,1]$ is an infinite $q$-ary sequence $\xf \in A_q^\omega$ satisfying
\begin{equation}
	s = \sum_{i=1}^\infty \xf_i q^{-i} =: \delta_q(\xf).
\end{equation}
For $x \in A_q^\ast$, we use the shorthand $\delta_q(x)$ to denote $\delta_q(x0^\infty)$. It was shown in \cite[Section 7.2]{calude2002information} that $q$-ary expansions also exhibit a $2$-ambiguity property; specifically for $\delta_q(\xf)$ irrational, $\delta_q(\xf) = \delta_q(\xf')$ implies $\xf = \xf'$, whereas for rational $\delta_q(\xf)$, there can be two different $q$-ary sequences that generate it. We define the greedy $q$-ary expansion $\gf_q(s)$ of a given $s \in [0,1]$ to be the lexicographically larger $q$-ary expansion of $s$. 

We first extend the notion of algorithmic complexity to $q$-ary sequences. Note that as each $b \in A_q$ can be encoded with a binary sequence of length $\lceil \log_2(q) \rceil$, then each $x \in A_q^\ast$ can be encoded by a binary sequence of length $|x| \lceil \log_2(q) \rceil$, that we denote $x^{(2)}$. For $x \in A_q^\ast$, we set $K[x] := K[x^{(2)}]$, and for $\xf \in A_q^\omega$, we let $K[\xf|n] := K[(\xf_{1:n})^{(2)}]$. 
\begin{theorem}\cite[Theorem 3]{staiger2002kolmogorov}\label{thm:staiger invariance}
	For all $q \in \N_2$ and  all $s \in [0,1]$, there exists $c > 0$ such that
\begin{equation}\label{eq:equivalence Kolmogorov complexity q ary expansions}
	\left| K\left[\gf_q(s)|n\right] - K\left[\gf_2(s)|\lceil n\log_2(q) \rceil\right]\right| \leq c, \ \ \text{for all} \ n \in \N, \ s \in [0,1].
\end{equation}
\end{theorem}
\begin{proof} We present the proof of the inequality
\begin{equation}
	 K\left[\gf_q(s)|n\right] \leq K\left[\gf_2(s)|\lceil n\log_2(q) \rceil\right] + c, \ \ \text{for all} \ n \in \N, \ s \in [0,1],
\end{equation}
and the converse inequality is analogously proven. The above inequality will be proved by showing that there exists an effective algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$ and $b_n \in \{0,1\}$, such that 
\begin{equation}
	\varphi(b_n \, \gf_2(s)_{1:\lceil n\log_2(q) \rceil}) = \gf_q(s)_{1:n}, \ \text{for all} \ n \in \N.
\end{equation} 
We make three observations, that allow to construct $\varphi$.
\begin{enumerate}[label = (\alph*)]
	\item \label{item:observation spacings between finite expansions} For $n \in \N$, let $S_n(q) := \{ \delta_q(x) : x \in A_q^n\}$. Then, for all $n \in \N$, $S_n(q) = \{ m q^{-n} : m \in \{0, \ldots, q^n - 1\}\}$, and $\delta_q$ is bijective from $A_q^n$ to $S_n(q)$. Below we displayed $S_n(q)$ for $n = 3$ and $q = 3$.
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}[scale = 10]
			\draw (0,0) -- (1,0);
			\draw (0,0) -- (1,0);
			\draw (0,-0.02) -- (0,0.02);
			\draw (1,-0.02) -- (1,0.02);
			\node[below] at (0,-0.015){$0$};
			\node[below] at (1,-0.015){$1$};
			\foreach \x in {0, ..., 26}
			{\draw[red] (\x/27,-0.01) -- (\x/27,0.01);}
		\end{tikzpicture}
		\caption{Each red line corresponds to one element $t$ in $S_3$, which in turn corresponds to exactly one element $x$ in $A_3^3$, being the preimage of $t$ by $\delta_3$.}
		\label{fig:spacings between finite q ary expansions}
	\end{figure}
		This observation essentially says that $S_n(q)$ is made of elements that are isolated and $q^{-n}$ apart. The 2-ambiguity of $q$-ary expansions crucially relies on this property.
	\item \label{item:observation greedy prefix is the immediate predecessor}For $s \in [0,1]$, $n \in \N$, $g_q(s)_{1:n}$ is exactly the preimage by $\delta_q$ of the number $t \in S_n$ that is the immediate predecessor of $s$. Below we displayed this number $t$ for $n = 3$, $q = 3$ and $s = 0.745$.
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}[scale = 10]
			\draw (0,0) -- (1,0);
			\draw (0,0) -- (1,0);
			\draw (0,-0.02) -- (0,0.02);
			\draw (1,-0.02) -- (1,0.02);
			\draw[blue] (0.745,-0.02) -- (0.745,0.02);
			\node[below] at (0,-0.015){$0$};
			\node[below] at (1,-0.015){$1$};
			\node[below] at (0.745,-0.015){$s$};
			\draw[->] (0.73,0.03) -- (0.74,0.012);
			\node[above] at (0.73,0.025){$t$};
			\foreach \x in {0, ..., 26}
			{\draw[red] (\x/27,-0.01) -- (\x/27,0.01);}
		\end{tikzpicture}
		\caption{Here $t = \delta_3(\gf_3(s)_{1:3})$.}
	\end{figure}
	\item \label{item:observation binaru exp is close to the real number}Let $m \in \N$, and $x \in \{0,1\}^m$. $x$ can be the $m$-prefix of the greedy binary expansion of any number in $[\delta_2(x), \delta_2(x) + 2^{-m})$.
	\begin{figure}[H]
		\centering
		\begin{tikzpicture}[scale = 10]
			\draw (0,0) -- (1,0);
			\draw (0,0) -- (1,0);
			\draw (0,-0.02) -- (0,0.02);
			\draw (1,-0.02) -- (1,0.02);
			\draw[blue] (0.625,-0.02) -- (0.625,0.02);
			\draw[blue] (0.75,-0.02) -- (0.75,0.02);
			\draw[blue, thick] (0.625,0) -- (0.75,0);
			\node[below] at (0,-0.015){$0$};
			\node[below] at (1,-0.015){$1$};
			\node[below] at (0.625,-0.012){\tiny $\delta_2(x)$};
			\node[below] at (0.75,-0.008){\tiny $\delta_2(x) + 2^{-3}$};
		\end{tikzpicture}
		\caption{Here we displayed the range of real numbers that admit $x = 0.101$ as prefix of their greedy binary expansion.}
	\end{figure}
\end{enumerate}
By combining the above three observations, we deduce that for $n,m \in \N$, and $x \in \{0,1\}^m$, there are less than $\lceil 2^{-m}/q^{-n} \rceil + 1$ elements in $A_q^n$ that correspond to the $n$-prefix of the greedy $q$-ary expansion of one of the real numbers whose greedy binary expansion starts with $x$.  The set of $n$-prefixes of greedy $q$-ary expansions associated with $x$ is denoted $A_q^n(x)$. Below, we displayed this result for $n = m = 3$ and $x = 0.101$.
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[scale = 10]
		\draw (0,0) -- (1,0);
		\draw (0,0) -- (1,0);
		\draw (0,-0.02) -- (0,0.02);
		\draw (1,-0.02) -- (1,0.02);
		\node[below] at (0,-0.015){$0$};
		\node[below] at (1,-0.015){$1$};
		\foreach \x in {0, ..., 26}
		{\draw[red] (\x/27,-0.01) -- (\x/27,0.01);}
		\draw[blue] (0.625,-0.02) -- (0.625,0.02);
		\draw[blue] (0.75,-0.02) -- (0.75,0.02);
		\draw[blue, thick] (0.625,0) -- (0.75,0);
		\draw[->] (0.68,0.06) -- (0.74,0.012);
		\draw[->] (0.68,0.06) -- (0.704,0.012);
		\draw[->] (0.68,0.06) -- (0.668,0.012);
		\draw[->] (0.68,0.06) -- (0.632,0.012);
		\draw[->] (0.68,0.06) -- (0.594,0.012);
		\node[above] at (0.68,0.055){\footnotesize Image of $A_3^3(x)$ by $\delta_q$.};
		\node[below] at (0.625,-0.012){\tiny $\delta_2(x)$};
		\node[below] at (0.75,-0.008){\tiny $\delta_2(x) + 2^{-3}$};
	\end{tikzpicture}
	\caption{In blue, we represented the set $I(x)$ of real numbers for which $x$ is a prefix of their greedy binary expansion. In red are all the numbers that are the image of elements of $A_3^3$ through $\delta_3$. The red elements designated by an arrow are elements in $A_3^3$ that are a prefix of the greedy ternary expansion of at least one real number in $I(x)$. We observe that there are 5 such elements, which is in accordance with the above formula $\lceil 2^{-3}/3^{-3} \rceil + 1 = 5$.}
\end{figure}

Now, let $s \in [0,1]$ and $n,m \in \N$. By the above discussion, $\gf_q(s)_{1:n} \in A_q^n(\gf_2(s)_{1:m})$. Therefore, one just needs $\gf_2(s)_{1:m}$ and the position $b_n \in \{0, \ldots, \lceil 2^{-m}/q^{-n} \rceil \}$ of $\gf_q(s)_{1:n}$ in the lexicographical enumeration of $A_q^n(\gf_2(s)_{1:m})$ to deduce $\gf_q(s)_{1:n}$. Remark that in the particular case $m = \lceil n \log_2(q)\rceil$, we have $b_n \in \{0, 1\}$. This concludes the construction the algorithm $\varphi$, as we have derived a method to deduce $\gf_q(s)_{1:n}$ from $b_n \, \gf_2(s)_{1:\lceil n \log_2(q)\rceil}$, for all $n \in \N$ and all $s \in [0,1]$.

Now, from Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists $C > 0$ such that
\begin{equation}\label{eq:g q g 2 and binary pos}
	K[\gf_q(s)_{1:n}] \leq K[b_n \, \gf_2(s)_{1:\lceil n \log_2(q)\rceil}] + C.
\end{equation}
Now, this is easy to conceive two effective algorithms $\varphi_0$ and $\varphi_1$ such that $\varphi_0(x) = 0x$ and $\varphi_1(x) = 1x$, for all $x \in \{0,1\}$, and hence by Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, there exists $c_0,c_1$ such that 
\begin{equation}
	K[0x] \leq x + c_0, \ \text{and} \ K[1x] \leq x + c_1, \ \text{for all} \ x \in \{0,1\}^\ast.
\end{equation}
Injecting in (\ref{eq:g q g 2 and binary pos}) gives
\begin{align}%\label{eq:g q g 2 and binary pos 2}
	K[\gf_q(s)_{1:n}] &\leq K[\gf_2(s)_{1:\lceil n \log_2(q)\rceil}] + C + c_{b_n}\\
	&\leq K[\gf_2(s)_{1:\lceil n \log_2(q)\rceil}] + C + \max \{c_0, c_1\}.
\end{align}
Setting $c := C + \max \{c_0, c_1\}$ finishes the proof.
\end{proof}

% The proof relies on the following critical observation, which is a premisse to the 2-ambiguity property of $q$-ary expansion.

% \begin{proof}
% Suppose we know the first $\lceil n \log_2(q) \rceil$ bits of $\gf_2(s)$. Note that 
% \begin{equation}
% 	0 \leq s - \delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil}) <  2^{- \lceil n \log_2(q) \rceil} \leq  q^{-n}
% \end{equation}
% and
% \begin{equation}
% 	0 \leq s - \delta_q(\gf_q(s)_{1:n}) < q^{-n},
% \end{equation}
% which implies that 
% \begin{equation}
% 	|\delta_q(\gf_q(s)_{1:n}) - \delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil})| < q^{-n}.
% \end{equation}
% Then, $\gf_q(s)_{1:n}$ is one of the $q$-ary sequences $x$ of length $n$ that satisfy
% \begin{equation}
% 	|\delta_q(x) - \delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil})| < q^{-n},
% \end{equation}
% i.e.,
% \begin{equation}
% 	\gf_q(s)_{1:n} \in \delta_q^{-1}(S_n \cap I) \cap A_q^n,
% \end{equation}
% where $I = (\delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil})- q^{-n},\delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil}) + q^{-n})$. As $\max I - \min I < 2q^{-n}$, there are at most two elements in $S_n \cap I$. Since $\delta_q : A_q^n \to S_n$ is bijective, there are at most 2 elements in $\delta_q(S_n \cap I) \cap A_q^n$, one of which being $\gf_q(s)_{1:n}$. Hence, given $\delta_2(\gf_2(s)_{1:\lceil n \log_2(q) \rceil})$, and one bit to decide which sequence to chose from $\delta_q(S_n \cap I)$, one can compute $\gf_q(s)_{1:n}$ through an effective algorithm. This is summarized in Algorithm \ref{alg:conversion base 2 base q}. 
% \begin{algorithm}
% 	\caption{Conversion from the greedy binary expansion to the greedy $q$-ary expansion}\label{alg:conversion base 2 base q}
% 	\begin{algorithmic}[1]
% 		\Require $x \in \{0,1\}^\ast, b \in \{0,1\}, q \in \N$
% 		\State $n \gets \lfloor |x|  / \log_2(q) \rfloor$
% 		\State Find all the sequences $x \in A_q^n$ that satisfy $|\delta_q(x) - \delta_2(x)| < q^{-n}$.
% 		\State As there are at most two such sequences, denote them $x$ and $x'$, where $x <_L x'$.
% 		\If{$b =0$}
% 		\State \Return $x^{(2)}$
% 		\Else
% 		\State \Return $x'^{(2)}$
% 		\EndIf
% 	\end{algorithmic}
% \end{algorithm}

% We denote the above algorithm $\varphi : \{0,1\}^\ast \to \{0,1\}^\ast$. Following the above discussion, there exists $b \in \{0,1\}$ such that
% \begin{equation}
% 	(\gf_q(s)_{1:n})^{(2)} = \varphi(\langle \gf_2(s)_{1:\lceil n \log_2(q) \rceil}, \langle b, q\rangle \rangle).
% \end{equation}
% By Lemma \ref{lem:if two sequences are connected through an algorithm, they have same kolmogorov complexity}, one concludes that there exists $c_0 >0$ such that
% \begin{align}
% 	K[\gf_q(s)|n] &\leq  K[\langle \gf_2(s)_{1:\lceil n \log_2(q) \rceil}, \langle b, q\rangle \rangle] + c_0\\
% 	& \overset{(a)}{\leq} K[\gf_2(s)|\lceil n \log_2(q) \rceil] + 2K[\langle b, q\rangle] + C_+ + c_1,
% \end{align}
% where $C_+ > 0$, and (a) follows from (\ref{eq:simple inequality on pairing of sequences}). We let $c := 2K[\langle b, q\rangle] + C_+ + c_1$, and we have
% \begin{equation}
% 	K[\gf_q(s)|n] \leq K[\gf_2(s)|\lceil n \log_2(q) \rceil] + c.
% \end{equation}
% The converse inequality can be established similarly, thereby finishing the proof.
% \end{proof}

We now proceed to extend the proof technique presented above to $\beta$-expansions, and to show its limitations.

\subsection{\texorpdfstring{Algorithmic complexity of $\beta$-expansions}{}}

% For $\beta \in (1,2)$, the above proof technique presented in the last section cannot be generalized to $\beta$-expansions in order to establish (\ref{eq:equivalence algorithmic complexity beta expansion binary expansion}). 

One can generalize the methodology presented in the last section to establish the following statement, which detailed proof is presented in Appendix \ref{app:greedy binary expansion is a minimizer of Kolmogorov complexity}.
\begin{theorem}\label{thm:binary expansion minimizes kolmogorov complexity}
	There exists $c > 0$ such that
	\begin{equation}
			K\left[\gf_2(s)|\lceil n\log_2(\beta)\rceil\right] \leq K\left[\xf|n\right] + c, 
	\end{equation}
	for all $n \in \N$, $ \xf \in \Sigma_\beta(s)$, and $s \in [0,1]$.
\end{theorem}
For $s \in [0,1]$, $n \mapsto K\left[\gf_2(s)|\lceil n\log_2(\beta)\rceil\right]$ is then seen to be a lower bound for the algorithmic complexity of the $\beta$-expansions of $s$. To establish (\ref{eq:equivalence algorithmic complexity beta expansion binary expansion}), one needs to prove that at least one $\beta$-expansion reaches this lower bound. We hence need to prove the following inequality. For computable $\beta \in (1,2)$, there exists $c > 0$, such that for all $s \in [0,1]$, there exists $\xf \in \Sigma_\beta(s)$ satisfying
\begin{equation}\label{eq:inequality to be proven}
	K\left[\xf|n\right] \leq K\left[\gf_2(s)|\lceil n\log_2(\beta)\rceil\right] + c, \ \ \text{for all} \ n \in \N.
\end{equation}
It would be tempting to adapt the proof of Theorem \ref{thm:staiger invariance} to establish the above result with $\xf = \gf_\beta(s)$. However, this is not possible for the simple reason that the observation \ref{item:observation spacings between finite expansions} examplified by Figure \ref{fig:spacings between finite q ary expansions} does not hold anymore: the elements of the set $S_n(\beta) = \{\delta_\beta(x) : x \in \{0,1\}^n\}$ are not $\simeq \beta^{-n}$ apart. As an example, Figure \ref{fig:spacings between finite beta ary expansions} represents the set $S_n(\beta)$, for $\beta = 1.6$ and $n = 4$.
\begin{figure}[H]
	\centering
	\begin{tikzpicture}[scale = 7]
		\draw (0,0) -- (1.67,0);
		\draw (0,-0.02) -- (0,0.02);
		\draw (1.67,-0.02) -- (1.67,0.02);
		\node[below] at (0,-0.015){$0$};
		\node[below] at (1.67,-0.015){$\frac{1}{\beta-1} = \frac{5}{3}$};
		\foreach \xun in {0, 1}{
			\foreach \xdeux in {0,1} {
				\foreach \xtrois in {0,1} {
					\foreach \xquatre in {0,1} {
						\foreach \beta in {1.6}{
							\draw[red] (\xun*1/\beta + \xdeux*1/\beta^2 + \xtrois*1/\beta^3 + \xquatre*1/\beta^4,-0.01) -- (\xun*1/\beta + \xdeux*1/\beta^2 + \xtrois*1/\beta^3 + \xquatre*1/\beta^4,0.01);
						}
					}
				}
			}
		}
		\draw[->] (0.35,-0.1) -- (0.386,-0.013);
		\draw[->] (0.44,-0.1) -- (0.403,-0.013);
		\node[below] at (0.33,-0.1){\tiny $t_1$};
		\node[below] at (0.46,-0.1){\tiny $t_2$};
	\end{tikzpicture}
	\caption{Here $t_2 - t_1 \simeq 0.06$, while $\beta^{-4} = 0.15$.}
	\label{fig:spacings between finite beta ary expansions}
\end{figure}
To use the same proof technique as above, we would need that the spacings between elements of $S_n(\beta)$ scale as $\beta^{-n}$. However, it is shown that there exists values of $\beta$ for which this is not the case \cite[Theorem 2.2]{benjamini2008spacings}. The best result one can get with the above proof technique is the following. 
\begin{theorem}\label{thm:upper bound kolmogorov complexity beta expansions}
	For Lebesgue-almost all $\beta \in (1,\sqrt{2})$, if $\beta$ is computable, there exists $c >0$ such that for all $s \in [0,1]$, and all $\xf \in \Sigma_\beta(s)$,
\begin{equation} \label{eq:upper bound Kolmogorov complexity beta expansions}
	K[\xf|n] \leq K[\gf_2(s)|\lceil n \log_2(\beta)\rceil] + n \log_2 \left(\frac{2}{\beta}\right) + c, \ \text{for all} \ n \in \N.
\end{equation}
\end{theorem}
\noindent The term $n\log_2\left(\frac{2}{\beta}\right)$ is an upper bound of the cardinality of $A_\beta^n(\gf_2(s)_{\lceil n \log_2(\beta)\rceil})$, where $A_\beta^n(x)$ is defined analogously to $A_q^n(x)$ in the proof of Theorem \ref{thm:staiger invariance}, for $x \in \{0,1\}^\ast$. The establishment of this upper bound involves using the Bernoulli convolution, which is the asymptotic distribution of the elements of the set $S_n(\beta)$ when $n$ goes to $\infty$. For an in-depth study of Bernoulli convolutions, we refer to \cite{peres2000sixty}. More specifically, the proof technique used for establishing the upper bound is inspired from the proof of \cite[Lemma 3.4]{kempton2013counting}. The technical details involve that the Bernoulli convolution has to be abslutely continuous and bounded, which is the case for Lebesgue-almost $\beta \in (1,\sqrt{2})$ \cite[Corollary 1]{solomyak1995random}. For $s \in [0,1]$, $n \mapsto K\left[\gf_2(s)|\lceil n\log_2(\beta)\rceil\right] + n\log_2\left(\frac{2}{\beta}\right)$ is then seen to be an upper bound for the algorithmic complexity of the $\beta$-expansions of $s$, holding however only for some specific values of $\beta$: $\beta$ must lay in a certain full-measure subset of $(1,\sqrt{2})$, and be computable. To the best of our knowledge, there is no proof that these two conditions are not mutually exclusive. The full proof is presented in Appendix \ref{app:greedy binary expansion is a minimizer of Kolmogorov complexity}.

To conclude on (\ref{eq:equivalence algorithmic complexity beta expansion binary expansion}), one needs to get rid of the term $n\log_2\left(\frac{2}{\beta}\right)$ in (\ref{eq:upper bound Kolmogorov complexity beta expansions}) for some $\xf \in \Sigma_\beta(s)$. To the best of our knowledge, this is not possible to adapt the arguments of the proof of Theorem \ref{thm:staiger invariance}. We opted instead for a drastic change of methodology.


